Lorentz Transformation and General Covariance Principle

I tell about different mathematical tool that is important in general relativity. The text of the book includes definition of geometrical object, concept of reference frame, geometry of metric-affinne manifold. Using this concept I learn few physical applications: dynamics and Lorentz transformation in gravitational fields, Doppler shift. A reference frame in event space is a smooth field of orthonormal bases. Every reference frame is equipped by anholonomic coordinates. Using anholonomic coordinates allows to find out relative speed of two observers and appropriate Lorentz transformation. Synchronization of a reference frame is an anholonomic time coordinate. Simple calculations show how synchronization influences time measurement in the vicinity of the Earth. Measurement of Doppler shift from the star orbiting the black hole helps to determine mass of the black hole. We call a manifold with torsion and nonmetricity the metric\hyph affine manifold. The nonmetricity leads to a difference between the auto parallel line and the extreme line, and to a change in the expression of the Frenet transport and moving basis. The torsion leads to a change in the Killing equation. We also need to add a similar equation for the connection. The analysis of the Frenet transport leads to the concept of the Cartan transport and an introduction of the connection compatible with the metric tensor. The dynamics of a particle follows to the Cartan transport. We need additional physical constraints to make a nonmetricity observable. Learning how torsion influences on tidal force reveals similarity between tidal equation for geodesic and the Killing equation of second type.

==> Abstract.0803.3276.English.tex <==
%auto-ignore
\begin{abstract}
I tell about different mathematical tool that is important in general relativity.
The text of the book includes definition of geometric object, concept of reference frame, geometry
of metric\hyph affinne manifold. Using this concept I learn few physical
applications: dynamics and Lorentz transformation in gravitational fields,
Doppler shift.

A reference frame in event space is a smooth field of orthonormal bases.
Every reference frame is equipped by anholonomic coordinates.
Using anholonomic coordinates allows to find out relative speed
of two observers and appropriate Lorentz transformation.

Synchronization of a reference frame is an anholonomic time coordinate.
Simple calculations show how synchronization influences time measurement in
the vicinity of the Earth.
Measurement of Doppler shift from the star orbiting the black hole helps
to determine mass of the black hole. According observations of Sgr A,
if non orbiting observer estimates age of S2 about 10 Myr,
this star is 0.297 Myr younger.

We call a manifold with torsion and nonmetricity the metric\hyph affine manifold.
The nonmetricity leads to a difference between the auto parallel line and the extreme line,
and to a change in the expression of the Frenet transport and moving basis.
The torsion leads to a change in the Killing equation. We also need to add a similar equation
for the connection.

The analysis of the Frenet transport leads to the concept of the Cartan transport
and an introduction of the connection compatible with the metric tensor.
The dynamics of a particle follows to the Cartan transport.
We need additional physical constraints to make
a nonmetricity observable.

Learning how torsion influences on tidal force reveals
similarity between tidal equation for geodesic and the Killing equation of second type.
The relationship between tidal acceleration, curvature and torsion gives an opportunity
to measure torsion.
\end{abstract}


==> Abstract.0803.3276.Russian.tex <==
%auto-ignore
\begin{abstract}
Я рассказываю о различных математических инструментах, которые важны в
общей теории относительности.
Текст книги включает определение геометрического объекта, концепцию системы отсчёта, геометрию
метрико\hyph аффинного многообразия. Опираясь на эти понятия я изучаю несколько физических
приложений: динамика и преобразование Лоренца в гравитационном поле,
эффект Допплера.

Система отсчёта в пространстве событий - это непрерывное поле ортонормированных базисов.
Каждая система отсчёта снабжена неголономными координатами.
Использование неголономных координат позволяет найти относительную скорость
двух наблюдателей и соответствующее преобразование Лоренца.

Синхронизация системы отсчёта - это неголономная координата времени.
Простые рассчёты показывают, как синхронизация влияет на измерение времени в
окрестности Земли.
Измерение эффекта Допплера от звезды, вращающейся вокруг чёрной дыры помогает
определить массу чёрной дыры. Согласно наблюдениям Sgr A, если
неподвижный наблюдатель оценивает возраст S2 порядка 10 Myr,
то эта звезда моложе на 0.297 Myr.

Мы будем называть многообразие с кручением и
неметричностью метрико\hyph аффинным многообразием.
Неметричность приводит к различию между автопараллельными
и экстремальными кривыми
и к изменению в выражении переноса Френе и подвижного базиса.
Кручение приводит к изменению в уравнении Киллинга.
Нам нужно также добавить аналогичное уравнение для связности.

Анализ переноса Френе ведёт к концепции переноса Картана
и введению связности, совместимой с метрическим тензором.
Динамика частицы приводит к переносу Картана.
Необходимы дополнительные физические условия, чтобы сделать
неметричность наблюдаемой.

Изучение, как кручение влияет на приливную силу обнаруживает
сходство между приливным уравнением для геодезической и уравнением Киллинга второго типа.
Связь между приливным ускорением, кривизной и кручением даёт возможность
измерить кручение.
\end{abstract}


==> Affine.Russian.tex <==
%auto-ignore
\input{Affine.Eq}
\ifx\PrintBook\undefined
\else
\chapter{Геометрия метрико-аффинного многообразия}
\fi

\section{Кривая экстремальной длины}
\labelSection{Line with extreme length}

Существует два разных определения геодезической
в римановом многообразии.
Одно из них опирается на параллельный перенос.
Мы будем называть соответствующую
\AddIndex{кривую автопараллельной}{auto parallel line}.
Другое определение опирается на длину траектории.
Мы будем называть соответствующую
\AddIndex{кривую экстремальной}{extreme line}.
В метрико\hyph аффинном многообразии эти линии имеют различные
уравнения \citeBib{torsion}.
Уравнение автопараллельной кривой не меняется.
Однако, уравнение
экстремальной кривой меняется.\,\footnote{Чтобы вывести
уравнение \EqRef{xtremeLine},
я следую идеям, которые Рашевский \citeBib{Rashevsky}
использовал для Риманова многообразия.}

\begin{theorem}
Пусть $x^i = x^i(t,\alpha)$ - кривая, зависящая от параметра $\alpha$,
с фиксированными точками при $t = t_1$ и
$t = t_2$, и мы определяем её длину как
\ShowEq{Line Length}
Тогда 
%\begin{widetext}
\ShowEq{Var Line Length}
%\end{widetext}
где $\delta x^k$ - изменение длины, когда $\alpha$ меняется.
\end{theorem}
\begin{proof}
Имеем
$$\frac {ds} {dt} = \sqrt{g_{ij} \frac {dx^i} {dt} \frac {dx^j} {dt}}$$
и
\ShowEq{Var Line Length, 1}
Мы можем оценить знаменатель дроби в равенстве
\EqRef{Var Line Length, 1}
\ShowEq{Var Line Length, 2}
Из равенств
\EqRef{Var Line Length, 1},
\EqRef{Var Line Length, 2}
следует, что
\ShowEq{Var Line Length, 3}
Первое слагаемое равно $0$, так как точки, где $t = t_1$ и $t = t_2$, зафиксированы.
Следовательно, мы доказали утверждение теоремы.
\end{proof}

\begin{theorem}
\labelTheorem{xtremeLine}
Экстремальная кривая удовлетворяет уравнению
\begin{equation}
\EqLabel{xtremeLine}
\frac {D\frac {dx^l} {ds}} {ds} =
\frac 1 2 g^{il} \left(g_{kj;i} - g_{ik;j}
- g_{ij;k}\right) \frac{dx^k}{ds} \frac{dx^j}{ds}
\end{equation}
\end{theorem}
\begin{proof}
Чтобы найти линию экстремальной длины,
мы воспользуемся функционалом
\EqRef{Line Length}.
Так как $\delta s = 0$, то
$$
\frac 1 2 \left(g_{kj;i} -
g_{ij;k} -
g_{ik;j}\right) \frac {dx^k} {ds} \frac {dx^j} {ds} ds
- g_{ij} D\frac {dx^j} {ds} = 0$$
следует из \EqRef{Var Line Length}.
\end{proof}

\begin{theorem}
Параллельный перенос вдоль экстремальной кривой
сохраняет длину касательного вектора.
\end{theorem}
\begin{proof}
Пусть $$v^i=\frac {dx^i}{ds}$$ касательный вектор к экстремальной кривой.
Из теоремы \RefTheorem{xtremeLine} следует, что
$$\frac {Dv^l} {ds} =
g^{il} \frac 1 2 \left(g_{kj;i} - g_{ik;j}
- g_{ij;k}\right) v^k v^j
$$
и
\ShowEq{Parallel transport holds length, 1}
Следовательно длина вектора $v^i$ не меняется вдоль экстремальной кривой.
\end{proof}

\section{Перенос Френе}
\labelSection{Frenet Transport}

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
Все уравнения, которые мы выводили до сих пор, различны,
однако они имеют нечто общее в своей структуре.
Все эти уравнения выражают движение вдоль кривой и в их правой части
мы можем видеть кривизну этой кривой.

\else
Из уравнения
\EqRef{xtremeLine}
следует, что экстремальная кривая имеет кривизну $0$.
\fi
По определению, кривизна кривой равна
\[\xi(s) = \left| \frac {D\frac {dx^l} {ds}} {ds} \right|\]
Следовательно, мы можем определить единичный вектор $e_1$ такой, что
\[\frac {D\frac {dx^l} {ds}} {ds} = \xi e^l_1\]

Знание переноса базиса вдоль кривой очень важно,
так как это позволяет нам изучать как изменяется пространство\Hyph время,
когда наблюдатель совершает движение.
Наша задача - найти уравнения, подобные переносу Френе в
римановом пространстве. Мы строим сопутствующий базис $\nu^i_k$ таким же
образом, как мы это делаем в римановом пространстве.

Векторы
\[\xi^i(t)=\frac{dx^i(t)}{dt}, \ \ \ \frac {D\xi^i} {dt},
\ \ \ ...\ \ \ \frac {D^{n-1}\xi^i} {dt^{n-1}}\]
вообще говоря, линейно независимы. Мы называем плоскость, построенную
на базе первых $p$ векторов, $p$-ой соприкасающейся плоскостью $R_p$.
Эта плоскость не зависит от выбора параметра $t$.

Наша следующая задача - построить ортогональный базис, который
покажет нам, как кривая изменяется.
Мы берём вектор $\nu^i_1\in R_1$ так, что он касателен к кривой.
Мы берём вектор $\nu^i_p\in R_p$, $p>1$ так, что $\nu^i_p$
ортогонален $R_{p-1}$. Если исходная кривая не изотропна,
то каждый $\nu^i_p$ также не изотропен и мы можем взять единичный вектор
в том же направлении. Мы называем этот базис сопутствующим.

\begin{theorem}
\labelTheorem{FrenetTransfer}
\AddIndex{Перенос Френе}{Frenet transport} в метрико-аффинном многообразии имеет вид
\begin{equation}
\begin{split}
\frac {D\nu^i_p} {dt}
= \frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_p - \\
- \epsilon_p \epsilon_{p-1} \xi_{p-1} \nu^i_{p-1} + \xi_p \nu^i_{p+1}
\end{split}
\EqLabel{Frenet}
\end{equation}
\[\epsilon_k = sign(g_{pq} \nu^p_k \nu^q_k)\]
Здесь $\nu^a_k$ - вектор базиса, движущегося вдоль кривой,
\[\epsilon_k = sign(g_{pq} \nu^p_k \nu^q_k)\]
\end{theorem}
\begin{proof}
Мы определяем векторы $\nu^a_k$ таким образом, что
\begin{equation}
\frac {D\nu^i_p} {dt}
= \frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_p
+ a^q_p \nu^i_q
\EqLabel{Frenet_1}
\end{equation}
где $a_p^q = 0$, когда $q > p+1$.
Теперь мы можем определить коэффициенты $a^q_p$.
Если мы возьмём производную уравнения
\[
g_{ij} \nu^i_p \nu^j_p = const
\]
и подставим \EqRef{Frenet_1}, мы получим уравнение
\ShowEq{Frenet 2}

$a_p^q = 0$, когда $q > p+1$ по определению.
Следовательно $a_p^q = 0$, когда $q < p+1$.
Полагая $\xi_p = a^{p+1}_p$, мы получим
\[
a^p_{p+1} = - \epsilon_p \epsilon_{p+1} \xi_p 
\]
Когда $q = p$, мы получим
\[
a_{p,p} = 0
\]
Мы получим \EqRef{Frenet}, когда подставим $a^q_p$ в \EqRef{Frenet_1}.
\end{proof}

\section{Связность Картана}
\labelSection{Cartan Transport}

Теоремы \RefTheorem{xtremeLine} и \RefTheorem{FrenetTransfer}
утверждают, что
движение вдоль кривой порождает преобразование вектора, дополнительное
к параллельному переносу.
Это преобразование очень важно
и мы будем называть его \AddIndex{переносом Картана}{Cartan transport}.
Мы определим \AddIndex{символ Картана}{Cartan symbol}
\ShowEq{Cartan symbol}
и \AddIndex{связность Картана}{Cartan connection}
\ShowEq{overbrace Gamma i kl}
Пользуясь связностью Картана, мы можем записать форму связности в виде
\ShowEq{Cartan connection form}
Соответственно, мы определим
\AddIndex{производную Картана}{Cartan derivative}
\ShowEq{overbrace nabla_l}
\ShowEq{overbrace D}

\begin{theorem}
\labelTheorem{LengthTangentVector}
Перенос Картана вдоль экстремальной
кривой сохраняет длину касательного вектора.
\end{theorem}
\begin{proof}
Пусть $$v^i=\frac {dx^i}{ds}$$ - касательный вектор к экстремальной кривой.
Из теоремы \RefTheorem{xtremeLine} следует, что
$$\frac {Dv^l} {ds} =
\frac 1 2 g^{il} \left(g_{kj;i} - g_{ik;j}
- g_{ij;k}\right) v^k v^j
$$
и
\ShowEq{Length of Tangent Vector}
Следовательно длина вектора $v^i$ не меняется вдоль экстремальной кривой.
\end{proof}

Мы распространим перенос Картана на любой геометрический объект подобно тому, как мы это
делаем для параллельного переноса.

\begin{theorem}
\labelTheorem{g ij;l=0}
\ShowEq{g ij;l=0}
\end{theorem}
\begin{proof}
\ShowEq{g ij;l=0 proof}
\end{proof}

Связность Картана $\overbrace{\Gamma^i_{kl}}$
отличается от связности $\Gamma^i_{kl}$
на дополнительное слагаемое, которое является симметричным тензором.
Для любой связности мы определяем стандартным образом производную и кривизну.
Утверждения геометрии и физики
имеют одну и ту же форму, независимо от того использую ли я связность $\Gamma^i_{kl}$ или связность Картана.
Чтобы это показать, мы можем обобщить понятие связности Картана
и изучать связность, определённую равенством
\ShowEq{conection overline}
\ShowEq{conection overline =}
где $A$ - это $0$, или символ Картана или любой другой
симметричный тензор.
Соответственно мы определяем производную
\ShowEq{overline nabla_l, definition 1}
\ShowEq{overline nabla_l, definition 2}
\ShowEq{overline nabla_l}
\ShowEq{overline D}
и кривизну
\ShowEq{GLn curvature_overline}
\ShowEq{GLn curvature_overline =}
Эта связность имеет тоже кручение
\begin{equation}
T^a_{cb} =
\overline{\Gamma^a_{bc}}-\overline{\Gamma^a_{cb}}
\EqLabel{Torsion coordinates_overline}
\end{equation}

С этой точки зрения теорема \RefTheorem{LengthTangentVector} означает,
что экстремальная кривая является геодезической
для связности Картана.

\begin{theorem}
\labelTheorem{curvature_overline}
Кривизна связности \EqRef{conection overline =} имеет вид
\begin{equation}
\overline{R^a_{bde}}=R^a_{bde}
+A^a_{be;d}-A^a_{bd;e}+A^a_{cd}A^c_{be}-A^a_{ce}A^c_{bd}+S^p_{de}A^a_{bp}
\label{curvature_overline}
\end{equation}
где $R^a_{bde}$ - кривизна связности $\Gamma^i_{kl}$
\end{theorem}
\begin{proof}
\begin{align*}
\overline{R^a_{bde}}&=\overline{\Gamma^a_{be,d}}-\overline{\Gamma^a_{bd,e}}
+\overline{\Gamma^a_{cd}}\ \overline{\Gamma^c_{be}}-\overline{\Gamma^a_{ce}}\ \overline{\Gamma^c_{bd}}\\
&=\Gamma^a_{be,d}+A^a_{be,d}-\Gamma^a_{bd,e}-A^a_{bd,e}\\
&+(\Gamma^a_{cd}+A^a_{cd})(\Gamma^c_{be}+A^c_{be})-(\Gamma^a_{ce}+A^a_{ce})(\Gamma^c_{bd}+A^c_{bd})\\
&=\Gamma^a_{be,d}+A^a_{be,d}-\Gamma^a_{bd,e}-A^a_{bd,e}\\
&+\Gamma^a_{cd}\Gamma^c_{be}+\Gamma^a_{cd}A^c_{be}+A^a_{cd}\Gamma^c_{be}+A^a_{cd}A^c_{be}\\
&-\Gamma^a_{ce}\Gamma^c_{bd}-A^a_{ce}\Gamma^c_{bd}-\Gamma^a_{ce}A^c_{bd}-A^a_{ce}A^c_{bd}\\
&=R^a_{bde}+A^a_{be,d}-A^a_{bd,e}\\
&+\Gamma^a_{cd}A^c_{be}+A^a_{cd}\Gamma^c_{be}+A^a_{cd}A^c_{be}\\
&-A^a_{ce}\Gamma^c_{bd}-\Gamma^a_{ce}A^c_{bd}-A^a_{ce}A^c_{bd}\\
&=R^a_{bde}\\
&+A^a_{be;d}-\underline{\Gamma^a_{pd}A^p_{be}}_2+\underline{\Gamma^p_{bd}A^a_{pe}}_4+\underline{\Gamma^p_{ed}A^a_{bp}}_{1:S}\\
&-A^a_{bd;e}+\underline{\Gamma^a_{pe}A^p_{bd}}_3-\underline{\Gamma^p_{be}A^a_{pd}}_5-\underline{\Gamma^p_{de}A^a_{bp}}_1\\
&+\underline{\Gamma^a_{cd}A^c_{be}}_2+\underline{\Gamma^c_{be}A^a_{cd}}_5+A^a_{cd}A^c_{be}\\
&-\underline{\Gamma^c_{bd}A^a_{ce}}_4-\underline{\Gamma^a_{ce}A^c_{bd}}_3-A^a_{ce}A^c_{bd}
\end{align*}
\end{proof}

\begin{corollary}
\AddIndex{Кривизна Картана}{Cartan curvature} имеет вид
\ShowEq{Cartan curvature}
\ShowEq{Cartan curvature =}
\end{corollary}

\section{Производная Ли}
\labelSection{Lie Derivative}

Векторное поле $\xi^k$ на многообразии порождает инфинитезимальное преобразование
\ShowEq{infinitesimal displacement}
которое ведёт к \AddIndex{производной Ли}{Lie derivative}.
Производная Ли говорит нам, как объект изменяется,
когда мы движемся вдоль векторного поля.

Из равенства
\EqRef{infinitesimal displacement}
следует, что
\ShowEq{infinitesimal displacement, derivative}
Из равенства
\EqRef{infinitesimal displacement}
следует также, что
\ShowEq{infinitesimal displacement, 1}
\ShowEq{infinitesimal displacement, 1, derivative}

\begin{theorem}
\AddIndex{Производная Ли метрики}{Lie derivative of metric} имеет вид
\ShowEq{Lie derivative of metric}
\ShowEq{Lie derivative of metric, def}
\end{theorem}
\begin{proof}
Мы начнём с преобразования \EqRef{infinitesimal displacement}.
Тогда
\[g_{ab}(x')=g_{ab}(x)+g_{ab,c}\epsilon \xi^c\]
Равенство
\begin{align*}
g'_{ab}(x')&=\frac{\partial x^c}{\partial x'^a} \frac{\partial x^d}{\partial x'^b}g_{cd}(x)\\
&=g_{ab}-\epsilon \xi^c_{,a}g_{cb}-\epsilon \xi^c_{,b}g_{ac}
\end{align*}
следует из равенства
\EqRef{infinitesimal displacement, 1, derivative}.
Согласно определению производной Ли, мы имеем
\ShowEq{Lie derivative of metric, 1}
\ShowEq{Lie derivative of metric, 2}
\EqRef{Lie derivative of metric, def} следует из
\EqRef{Lie derivative of metric, 2} и \EqRef{Torsion coordinates}.
\end{proof}

\begin{theorem}
\AddIndex{Производная Ли связности}{Lie derivative of connection} имеет вид
\ShowEq{Lie derivative of connection}
\ShowEq{Lie derivative of connection, def}
\end{theorem}
\begin{proof}
Мы начнём с преобразования \EqRef{infinitesimal displacement}.
Тогда
\ShowEq{Lie derivative of connection,1}
Равенство
\ShowEq{Lie derivative of connection,2}
следует из равенств
\EqRef{infinitesimal displacement, derivative},
\EqRef{infinitesimal displacement, 1, derivative}.
По определению
\ShowEq{Lie derivative of connection 2}
\ShowEq{Lie derivative of connection,3}
Так как
\ShowEq{Lie derivative of connection,41}
является тензором, то
\ShowEq{Lie derivative of connection 3}
Равенство
\ShowEq{Lie derivative of connection,4}
следует из равенства
\EqRef{Lie derivative of connection 3}.
Мы подставим \EqRef{Lie derivative of connection,4} и \EqRef{Lie derivative of connection,3}
в \EqRef{Lie derivative of connection,2} и получим
\ShowEq{Lie derivative of connection,5}
Согласно определению производной Ли, мы имеем,
пользуясь \EqRef{Lie derivative of connection,1} и \EqRef{Lie derivative of connection,5},
\ShowEq{Lie derivative of connection,6}
Из \EqRef{Lie derivative of connection,6}
и \EqRef{Torsion coordinates} следует, что
\ShowEq{Lie derivative of connection,7}
Из \EqRef{Lie derivative of connection,7} и \EqRef{GLn curvature} следует, что
\ShowEq{Lie derivative of connection,8}
Из \EqRef{Lie derivative of connection,8} и \EqRef{Bianchi 1} следует, что
\ShowEq{Lie derivative of connection,9}
Мы подставим \EqRef{commutator second derivative of vector} в \EqRef{Lie derivative of connection,9}
\ShowEq{Lie derivative of connection,10}
\EqRef{Lie derivative of connection, def}
следует из \EqRef{Lie derivative of connection,10}.
\end{proof}
\begin{corollary}
Производная Ли связности в римановом пространстве имеет вид
\begin{equation}
\EqLabel{Lie derivative of connection in Rieman space}
\mathcal{L}_\xi\Gamma^a_{bc}=-R^a_{cbp} \xi^p+\xi^a_{;cb}\\
\end{equation}
\end{corollary}
\begin{proof}
\EqRef{Lie derivative of connection in Rieman space} следует
из \EqRef{Lie derivative of connection, def}, когда $T^a_{bc}=0$
\end{proof}

\section{Тождество Бианки}
\labelSection{Bianchi Identity}

\begin{theorem}
 Первое тождество Бианки для пространства с кручением имеет вид
\ShowEq{Bianchi 1}
\end{theorem}
\begin{proof}
Дифференциал равенства \EqRef{Torsion 1} имеет вид
\ShowEq{Bianchi 1, 1}
Две формы равны, когда их коэффициенты равны. Следовательно, из
\EqRef{Bianchi 1, 1}
следует, что
\ShowEq{Bianchi 1, 2}
Мы выразим производные, пользуясь ковариантными производными,
и изменим порядок слагаемых
\ShowEq{Bianchi 1, 3}
Равенство
\ShowEq{Bianchi 1, 4}
следует из равенства
\EqRef{Bianchi 1, 3}.
\EqRef{Bianchi 1} следует из \EqRef{Bianchi 1, 4}.
\end{proof}

%If мы получим derivative of form (\ref{eq: Torsion})
%мы will получим first Bianchi identity for space with кручение \citeBib{Neeman}
%\[D T^a = \Omega^a_c \wedge \theta^c\]
%из \EqRef{Torsion} и \EqRef{Bianchi 1,1}

Если мы возьмём производную формы \EqRef{Curvature},
мы увидим, что второе тождество Бианки не
зависит от кручения. 

\section{Вектор Киллинга}
\labelSection{Killing Vector}

Инвариантность метрического тензора $g$ при инфинитезимальном координатном преобразовании
\EqRef{infinitesimal displacement}
приводит к \AddIndex{уравнению Киллинга}{Killing equation}.

\begin{theorem}
Уравнение Киллинга в метрико\hyph аффинном многообразии имеет вид
\ShowEq{Killing equation 1}
\end{theorem}
\begin{proof}
Инвариантность метрического тензора $g$ означает, что его производная Ли равна $0$
\begin{equation}
\mathcal{L}_\xi g_{ab}=0
\EqLabel{Killing equation 1,1}
\end{equation}
\EqRef{Killing equation 1} folows из \EqRef{Killing equation 1,1} и
\EqRef{Lie derivative of metric, def}.
\end{proof}

%However it looks like for the metric\hyph affine manifold the Killing equation is not
%a sufficient condition for homogeneity of event space. Мы need to write a similar condition
%for the connection as well.

\begin{theorem}
Условие инвариантности связности в метрико\hyph аффинном многообразии имеет вид
\ShowEq{Killing equation 2}
\end{theorem}
\begin{proof}
Так как связность инвариантна при инфинитезимальном преобразовании, мы имеем
\ShowEq{Killing equation 2,1}
\EqRef{Killing equation 2} следует из
\EqRef{Killing equation 2,1} и \EqRef{Lie derivative of connection, def}.
\end{proof}

Мы называем уравнение \EqRef{Killing equation 2}
\AddIndex{уравнением Киллинга второго рода}{Killing equation second type}
и вектор $\xi^a$
\AddIndex{вектором Киллинга второго рода}{Killing vector second type}.

\begin{theorem}
Вектором Киллинга второго рода удовлетворяет уравнению
\ShowEq{Killing equation 2, corollary}
\end{theorem}
\begin{proof}
Из \EqRef{Killing equation 2}
и \EqRef{commutator second derivative of vector}
следует, что
\ShowEq{Killing equation 2,4}
\EqRef{Killing equation 2, corollary} следует из \EqRef{Killing equation 2,4}.
\end{proof}

\begin{corollary}
Уравнением Киллинга второго рода в римановом пространстве является тождеством.
Связность в римановом пространстве инвариантна при
любом инфинитезимальном преобразовании \EqRef{infinitesimal displacement}.
\end{corollary}
\begin{proof}
Прежде всего, кручение равно 0. Остальное является следствием первого тождества Бианки.
\end{proof}


==> Basis.Russian.tex <==
%auto-ignore

\input{Basis.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Многообразие базисов}
\labelChapter{Basis Manifold}
\fi

\section{Базис в векторном пространстве}
\labelSection{Basis in Vector Space}

\begin{definition}
\labelDefinition{vector space over field}
Пусть $D$ - поле.
Абелевая группа \symb{V}{V}1 называется
\AddIndex{векторным пространством}{vector space} над полем $D$,
если определено произведение\,\footnote{
Так как произведение в поле $D$ коммутативно,
для нас не имеет значения
записываем мы произведение в виде $av$ или $va$.
Я выбрал запись $va$ так как хочу пользоваться
матричным представлением вектора.
}
\ShowEq{f:A->B}{*}{V\times D}V
\ShowEq{f:A->B}{*}{D\times V}V
которое удовлетворяет соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон коммутативности}{comutative law}
\labelItem{comutative law, vector space}
\ShowEq{comutative law}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, vector space}
\DrawEq{associative law, right module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, vector space}
\ShowEq{distributive law, right module}
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, vector space}
\ShowEq{unitarity law, right A-module}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{set of vectors generated by set of vectors, vector space}
Пусть $V$ - векторное пространство.
Множество векторов, порождённое множеством векторов
\ShowEq{vi V},
имеет вид\,\footnote{
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}
\ShowEq{w=sum vi, vector space}
\end{theorem}

\begin{proof}
Мы должны доказать следующие утверждения:
\ShowEq{vector space generated by set of vectors}

\begin{itemize}
\item
Для произвольного
\ShowEq{vk in v}
положим
\ShowEq{ci=dik}D
Тогда
\ShowEq{vk=sum vi, right module}
Утверждение
\RefItem{vector space, vk in Jv}
следует из
\EqRef{w=sum vi, vector space},
\EqRef{vk=sum vi, right module}.
\item
Утверждение
\RefItem{vector space over D, cvk in Jv}
являются следствием определения
\RefDefinition{vector space over field}
и утверждения
\RefItem{vector space, vk in Jv}.
\item
Так как $V$ является абелевой группой,
то утверждение
\RefItem{vector space over D, sum cvk in Jv}
следует из утверждения
\RefItem{vector space over D, cvk in Jv}
и определения
\RefDefinition{vector space over field}.
\item
Пусть
\ShowEq{w12 in Jv over D}
Так как $V$ является абелевой группой,
то вектор $w_1+w_2$ порождён множеством векторов $v$.
Согласно равенству
\EqRef{w=sum vi, vector space},
существуют $D$\Hyph числа
\ShowEq{gi12}w
такие, что
\DrawEq[w]{w12= right}{module}
где множества
\DrawEq[w]{|ci12 ne 0|}{right module}
конечны.
Так как $V$ является абелевой группой,
то из равенства
\eqRef{w12= right}{module}
следует, что
\DrawEq[w]{w1+w2= right}{module}
Равенство
\DrawEq[w]{w1+w2= 1 right}{module}
является следствием равенств
\EqRef{distributive law, right module, 2},
\eqRef{w1+w2= right}{module}.
Из равенства
\eqRef{|ci12 ne 0|}{right module}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}w
конечно.
Следовательно, утверждение
\RefItem{vector space over D, v,w in Jv=>v+w in Jv}
верно.
\item
Пусть
\ShowEq{w in Jv over D}
Согласно определению
\RefDefinition{vector space over field},
для любого $D$\Hyph числа $a$,
вектор $wa$ порождён множеством векторов $v$.
Согласно равенству
\EqRef{w=sum vi, vector space},
существуют $D$\Hyph числа
\ShowEq{set au vi}w
такие, что
\ShowEq{w= right module}
где
\DrawEq{|wi ne 0|}{vector space}
Из равенства
\EqRef{w= right module}
следует, что
\ShowEq{aw= right module}
Из утверждения
\eqRef{|wi ne 0|}{vector space}
следует, что
множество
\ShowEq{right module, |awi ne 0|}
конечно.
Следовательно, утверждение
\RefItem{vector space over D, v in Jv=>av in Jv}
верно.
\end{itemize}
\end{proof}

\def\SideWS{right }%
\def\SideNS{right}%
\ShowDefinition{linear combination of vectors}

Представим множество $D$\Hyph чисел
\ShowEq{set au vi}w
в виде матрицы
\ShowEq{column vector w=wi}w
Представим множество векторов
\ShowEq{set vi}
в виде матрицы
\ShowEq{row vector w=wi}vn
Тогда мы можем записать линейную комбинацию векторов
\ShowEq{w=wi vi\SideNS}
в виде
\ShowEq{w=vw over D}

\begin{theorem}
\labelTheorem{linearly depends on rest of vectors, vector space}
Если уравнение
\ShowEq{\SideWS wi vi=0}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0},
то вектор $v_{\gij}$
линейно зависит от остальных векторов $v$.
\end{theorem}

\ShowProof{linearly depends on rest of vectors}

Очевидно, что для любого множества векторов $v_{\gii}$,
\ShowEq{right 0=0vi over D}

\begin{definition}
\labelDefinition{linearly independent vectors}
Множество векторов\,\footnote{
Я следую определению в
\citeBib{Serge Lang}, страница 100.}
\ShowEq{set vi}
векторного пространства $V$
\AddIndex{линейно независимо}{linearly independent set},
если $w=0$ следует из уравнения
\ShowEq{\SideWS wi vi=0}
В противном случае, множество векторов
\ShowEq{set vi}
\AddIndex{линейно зависимо}{linearly dependent set}.
\qed
\end{definition}

Определения
\RefDefinition{generating set of vector space},
\RefDefinition{basis of vector space}
являются следствием теоремы
\RefTheorem{set of vectors generated by set of vectors, vector space}.

\begin{definition}
\labelDefinition{generating set of vector space}
$J(v)$
называется
векторным подпространством, порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
векторного подпространства $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
векторного пространства $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
\qed
\end{definition}

\begin{definition}
\labelDefinition{basis of vector space}
Если множество $X\subset V$ является множеством образующих
векторного пространства $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих векторного пространства $V$.
Если существует минимальное множество $X$, порождающее
векторное пространство $V$, то такое множество $X$ называется
\AddIndex{базисом}{basis} векторного пространства $V$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{basis of vector space}
Множество векторов
\ShowEq{basis for module over algebra}
является базисом векторного пространства
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, vector space}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, vector space}
Вектор $e_{\gii}$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
\end{theorem}

\begin{proof}
Согласно утверждению
\RefItem{vector is linear combination of set, vector space},
теореме
\RefTheorem{set of vectors generated by set of vectors, vector space}
и определению
\RefDefinition{\SideWS linear combination of vectors},
множество $\Basis e$ порождает векторное пространство $V$
(определение
\RefDefinition{generating set of vector space}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, vector space},
множество $\Basis e$ является минимальным множеством,
порождающим векторное пространство $V$.
Согласно определению
\RefDefinition{basis of vector space},
множество $\Basis e$ является базисом  векторного пространства $V$.
\end{proof}

\begin{theorem}
\labelTheorem{field, vector space}
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом векторного пространства}{basis, vector space}
$V$, если векторы $e_{\gii}$ линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{theorem}

\begin{proof}
Пусть множество векторов
\ShowEq{ei, i in I}
линейно зависимо. Тогда в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}.
Согласно теореме
\RefTheorem{linearly depends on rest of vectors, vector space},
вектор $e_{\gij}$
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\RefDefinition{basis of vector space},
множество векторов
\ShowEq{ei, i in I}
не является базисом векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{ei, i in I}
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{ei, i in I},
то множество векторов $v$,
\ShowEq{ei, i in I}
не является линейно независимым.
\end{proof}

Из теоремы
\RefTheorem{field, vector space}
следует, что $\Basis e$ -
это максимальное множество линейно независимых векторов.
В том случае, когда мы хотим явно указать, что это базис
векторного пространства $V$, мы будем пользоваться обозначением
\ShowEq{basis in V}

\begin{definition}
\labelDefinition{coordinates of vector, vector space}
Пусть $\Basis e$ - базис векторного пространства $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve vector space}{}
относительно базиса $\Basis e$.
$D$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
\qed
\end{definition}

Пусть $\Basis e$ - базис векторного пространства $V$.
Представим множество векторов
\ShowEq{set ei}
в виде матрицы
\ShowEq{row vector basis e}
Представим множество координат
\ShowEq{set au v1n}v
вектора $\Vector v$ относительно базиса $\Basis e$
в виде матрицы
\ShowEq{column vector w=wi}v
Матрица $v$
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
Тогда мы можем записать вектор $\Vector v$
в виде произведения матриц
\DrawEq [v]{vv=vev}{}

\begin{theorem}
\labelTheorem{coordinates of vector of vector space}
Координаты вектора $v\in V$ относительно базиса $\Basis e$
векторного пространства $V$
определены однозначно.
\end{theorem}

\begin{proof}
Пусть вектор $\Vector v$ имеет разложения
\DrawEq[1]{vv=evi}{1}
\DrawEq[2]{vv=evi}{2}
относительно базиса $\Basis e$.
Равенство
\ShowEq{ev (1-2)}
является следствием равенств
\eqRef{vv=evi}{1},
\eqRef{vv=evi}{2}.
Утверждение
\ShowEq{vi1=vi2}
является следствием равенства
\EqRef{ev (1-2)}
и теоремы
\RefTheorem{field, vector space}.
\end{proof}

\begin{theorem}
\labelTheorem{coordinates of linear composition}
Представим множество координат векторов
\ShowEq{row vector w=wi}vm
в виде матрицы
\ShowEq{row vector coordinates}
Тогда координаты линейной комбинации
\ShowEq{vi ci}
векторов $v$ можно представить в виде произведения матриц
\ShowEq{vc=vm cm}
\end{theorem}

\begin{proof}
Теорема является следствием теоремы
\RefTheorem{coordinates of vector of vector space}.
\end{proof}

\begin{theorem}
\labelTheorem{coordinate matrix of basis is not singular}
Пусть $\Basis e$, $\Basis f$ - базисы векторного пространства $V$.
Координатная матрица
\ShowEq{coordinate matrix nn}e
базиса $\Basis e$ относительно базиса $\Basis f$
является невырожденной матрицей.
\end{theorem}

\begin{proof}
Согласно определению
\RefDefinition{linearly independent vectors}
и теоремам
\RefTheorem{field, vector space},
\RefTheorem{coordinates of linear composition},
система линейных уравнений
\ShowEq{matrix of basis *c=0}
имеет единственное решение.
Следовательно, матрица $e$
является невырожденной матрицей.
\end{proof}

\section{Линейное преобразование векторного пространства}

\begin{definition}
\labelDefinition{linear transformation of vector space}
Пусть $V$ - векторное пространство.
Отображение
\ShowEq{f:A->B}fVV
называется линейным преобразованием векторного пространства $V$, если
\ShowEq{f linear map}
для любых векторов $v$, $w\in V$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{linear transformation of vector space}
Пусть
$\Basis e$ -
базис векторного пространства $V$.
Тогда линейное преобразование
\ShowEq{f:A->B}{\Vector f}VV
имеет представление
\ShowEq{f:A->A vector space}
\DrawEq[wfv]{w=f v matrix}1
относительно базиса $\Basis e$. Здесь
\begin{itemize}
\item $v$ - координатная матрица вектора
$\Vector v$
относительно базиса
\ShowEq{basis e}{}{}
\DrawEq [v]{vv=vev}v
\item $w$ - координатная матрица вектора
\ShowEq{vw=vf(vv)}
относительно базиса
\ShowEq{basis e}{}{}
\DrawEq [w]{vv=vev}w
\item $f$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) vector space}
относительно базиса
\ShowEq{basis e}{}.
Мы будем называть матрицу $f$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector f$ относительно базиса
\ShowEq{basis e}{}.
\end{itemize}
\end{theorem}

\begin{proof}
Так кaк отображение
$\Vector f$
является линейным отображением, то равенство
\ShowEq{vw=f(e1)vv}
является следствием равенств
\EqRef{f linear map},
\eqRef{vv=vev}v,
\EqRef{vw=vf(vv)}.
Вектор
\ShowEq{vf(e1)}
имеет разложение
\ShowEq{vf(e1)=}
относительно базиса $\Basis e$.
Комбинируя \EqRef{vw=f(e1)vv}
и \EqRef{vf(e1)=}, мы получаем
\ShowEq{w=e f v}
\ShowEq{e w=e f v matrix}
Равенство
\eqRef{w=f v matrix}1
следует из сравнения
\eqRef{vv=vev}w
и \EqRef{w=e f v}.
\end{proof}

\begin{theorem}
\labelTheorem{non-singular linear transformation}
Матрица $f$ линейного преобразования $\Vector f$
невырождена
тогда и только тогда, когда
линейное преобразование $\Vector f$ отображает
базис векторного пространства $V$ в базис.
\end{theorem}

\begin{proof}
Пусть
\ShowEq{Bases egh}
- базисы векторного пространства $V$.
Пусть линейное преобразование $\Vector f$
отображает базис $\Basis e$ в базис $\Basis g$.
Пусть
\ShowEq{coordinate matrix nn}e
координатная матрица базиса $\Basis e$ относительно базиса $\Basis h$.
Пусть
\ShowEq{coordinate matrix nn}g
координатная матрица базиса $\Basis g$ относительно базиса $\Basis h$.
Пусть
\ShowEq{coordinate matrix nn}f
координатная матрица отображения $\Vector f$ относительно базиса $\Basis h$.
Тогда равенство
\ShowEq{product g=fe}
является следствием теоремы
\RefTheorem{linear transformation of vector space}.
Согласно теореме
\RefTheorem{coordinate matrix of basis is not singular}
матрицы $e$ и $g$ не вырождены.
Следовательно, матрица $f$ тоже не вырождена.

С другой стороны, пусть координатная матрица $f$ отображения $\Vector f$
является невырожденной матрицей.
Так как координатная матрица $e$ базиса $\Basis e$ - невырожденная матрица,
то из равенства
\EqRef{product g=fe}
следует, что матрица $g$ также является невырожденной матрицей.
Следовательно, матрица $g$ является
координатной матрицей базиса $\Basis g$
и отображение $\Vector f$ отображает базис в базис.
\end{proof}

\begin{theorem}
Множество невырожденных матриц
\ShowEq{GV}
порождает группу.
Мы обычно будем называть группу $G(V)$
\AddIndex{группой симметрии}{symmetry group}.
Группа $G(V)$
порождает левостороннее линейное представление
в векторном пространстве $V$.
\end{theorem}

\begin{proof}
Согласно теореме
\RefTheorem{linear transformation of vector space},
линейные преобразования
\ShowEq{f:A->B}{\Vector f}VV
\ShowEq{f:A->B}{\Vector g}VV
имеют вид
\DrawEq[wfv]{w=f v matrix}{wfv}
\DrawEq[ugw]{w=f v matrix}{ugw}
Равенство
\ShowEq{u=gfv}
является следствием равенств
\eqRef{w=f v matrix}{wfv},
\eqRef{w=f v matrix}{ugw}.
Теорема является следствием равенства
\EqRef{u=gfv}.
Представление является левосторонним
согласно закону произведения матриц.
\end{proof}

Согласно теореме
\RefTheorem{linear transformation of vector space},
мы будем отождествлять элемент $g$ группы $G(V)$
с соответствующим преобразованием представления
и записывать его действие на вектор $v\in V$ в виде $gv$.
Эта точка зрения позволяет определить два типа координат
для элемента $g$ группы $G(V)$. Мы можем либо пользоваться координатами,
определёнными на группе, либо определить координаты как
элементы матрицы соответствующего преобразования.
Первая форма координат более эффективна, когда мы изучаем
свойства группы $G(V)$. Вторая форма координат
содержит избыточную информацию,
но бывает более удобна,
когда мы изучаем представление группы $G(V)$.
Мы будем называть вторую форму координат
\AddIndex{координатами представления}{coordinates of representation}.

В зависимости от рассматриваемых свойств векторного пространства,
мы можем рассматривать группу $G\subseteq G(V)$,
преобразования которой сохраняют рассматриваемые свойства.
Рассматриваемая группа $G$ называется группой симметрии
векторного пространства $V$.

Из теоремы
\RefTheorem{non-singular linear transformation}
следует, что мы можем продлить линейное преобразование
векторного пространства $V$ на множество базисов.
Таким образом, мы можем распространить левостороннее представление группы симметрии
на множество базисов.
Мы будем
записывать действие элемента $g$ группы $G$ на базис $\Basis{e}$ в виде
\ShowEq{active transformation}
Тем не менее, не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Таким образом, множество базисов
можно представить как объединение орбит группы $G$.

Свойства базиса зависят от группы симметрии.
Мы можем выбрать базисы $\Basis{e}$, векторы которых находятся
в отношении, которое инвариантно относительно группы симметрии.
В этом случае все базисы из орбиты
\ShowEq{bases from orbit ge}
имеют векторы, которые удовлетворяют одному и тому же отношению.
Такой базис мы будем называть
\AddIndex{$G$\Hyph базисом}{G-basis}.
В каждом конкретном случае мы должны доказать существование
базиса с искомыми свойствами. Если подобного типа базиса
не существует, мы можем выбрать произвольный базис.

\begin{definition}
\labelDefinition{basis manifold of vector space}
Мы будем называть орбиту $G\Basis{e}$
выбранного базиса $\Basis{e}$
\AddIndex{многообразием базисов
\ShowEq{basis manifold of vector space}
векторного пространства}{basis manifold of vector space}
$V$.
 \qed
 \end{definition}

\begin{theorem}
\labelTheorem{basis manifold of vector space}
Представление группы $G$ на многообразии базисов
однотранзитивно.
\end{theorem}
\begin{proof}
Согласно определению \RefDefinition{basis manifold of vector space}
любые два базиса связаны по крайней мере одним преобразованием
представления. Для доказательства теоремы достаточно показать,
что это преобразование определено однозначно.

Допустим элементы $g_1$, $g_2$ группы $G$ и базис $\Basis{e}$ таковы, что
\ShowEq{two transformations on basis manifold, 1}
Из \EqRef{two transformations on basis manifold, 1} следует
\ShowEq{two transformations on basis manifold, 2}
Так как любой вектор имеет единственное разложение
относительно базиса $\Basis{e}$, то из
\EqRef{two transformations on basis manifold, 2} следует,
что
\ShowEq{two transformations on basis manifold, 3}
является тождественным преобразованием
векторного пространства $V$. Так как представление
группы $G$ эффективно на векторном пространстве $V$,
то $g_1=g_2$.
Отсюда следует утверждение теоремы.
\end{proof}

Из теоремы \RefTheorem{basis manifold of vector space} следует,
что многообразие базисов $\mathcal{B}(V)$ является однородным пространством группы $G$.
Мы построили левостороннее однотранзитивное линейное
представление группы $G$ на многообразии базисов.
Мы будем называть это представление
\AddIndex{активным представлением}{active representation},
а соответствующее преобразование на многообразие базисов
\AddIndex{активным преобразованием}{active transformation}
(\citeBib{Korn})
потому, что линейное преобразование векторного пространства породило
преобразование многообразия базисов.

Согласно теореме \RefTheorem{single transitive representation of group},
так как многообразие базисов $\mathcal{B}(V)$ -
однородное пространство группы $G$,
мы можем определить на $\mathcal{B}(V)$
две формы координат, определённые на группе $G$.
В обоих случаях координаты базиса $\Basis{e}$ - это
координаты гомоморфизма, отображающего заданный базис $\Basis{e}_0$ в
базис $\Basis{e}$.
Координаты представления называются
\AddIndex{стандартными координатами базиса}
{standard coordinates of basis}.
Нетрудно показать, что стандартные координаты
\ShowEq{standard coordinates of basis}
базиса $\Basis{e}$ при заданном значении $k$ являются
координатами вектора
\ShowEq{vector of basis}
относительно заданного базиса $\Basis{e}_0$.

Базис $\Basis{e}$ порождает координаты на $V$.
В различных типах пространства это может быть сделано различным образом.
В аффинном пространстве, если вершина базиса является точкой $A$, то
точка $B$ имеет те же координаты, что и вектор $\overset{\longrightarrow}{AB}$
относительно базиса $\Basis{e}$.
В общем случае мы вводим координаты вектора как координаты
относительно выбранного базиса.
Использование только $G$\Hyph пространства означает использование специальных координаты на $\mathcal{A}_n$.
Для того, чтобы отличать их, мы будем называть их
\AddIndex{$G$\Hyph координатами}{G-coordinates}.
Мы также будем называть пространство $V$ с такими координатами
\AddIndex{$G$\Hyph пространством}{GSpace}.

Согласно теореме \RefTheorem{two representations of group}, на многообразии базисов существует другое
представление, перестановочное с активным.
Как мы видим из замечания \ref{remark: one representation of group}
преобразование этого
представления отличается от активного преобразования и не может быть сведено к
преобразованию пространства $V$.
Чтобы подчеркнуть различие, это преобразование называется
\AddIndex{пассивным преобразованием}{passive transformation}
векторного пространства $V$,
а представление называется
\AddIndex{пассивным представлением}{passive representation}.
Мы будем записывать пассивное преобразование базиса $\Basis{e}$,
порождённое элементом $g\in G$, в виде
\ShowEq{passive transformation}

\section{Базис в аффинном пространстве}

Мы отождествляем векторы аффинного пространства
\ShowEq{An}
с парой точек $\overset{\longrightarrow}{AB}$.
Все векторы, которые имеют общее начало $A$ порождают векторное пространство,
которое мы будем называть касательным векторным пространством $T_A\mathcal{A}_n$.

Топология, которую $\mathcal{A}_n$ наследует из отображения $\mathcal{A}_n\rightarrow R^n$,
позволяет нам изучать непрерывные преобразования пространства $\mathcal{A}_n$
и их производные. Более точно, производная
преобразования $f$ отображает векторное пространство $T_A\mathcal{A}_n$ в $T_{f(A)}\mathcal{A}_n$.
Если $f$ линейно, то его производная одна и та же в каждой точке.
Вводя координаты $A^1,...,A^n$ точки $A\in\mathcal{A}_n$, мы можем записать
линейное преобразование как
\begin{align}
A'^i&=P^i_j A^j + R^i &\det P\ne 0
\EqLabel{AffineTransformation}
\end{align}
Производная этого преобразования определена матрицей $\|P^i_j\|$
и не зависит от точки $A$. Вектор
$(R^1,...,R^n)$ выражает смещение в аффинном пространстве.
Множество преобразований \EqRef{AffineTransformation} - это группа Ли,
которую мы обозначим
\ShowEq{affine transformation group}
и будем называть
\AddIndex{группой аффинных преобразований}{affine transformation group}.

\begin{definition}
\AddIndex{Аффинный базис}{Affine Basis}
\ShowEq{Affine Basis}
- это множество
линейно независимых векторов $\Vector e_i=\overset{\longrightarrow}{OA_i}=(e^1_i,...,e^n_i)$
с общей начальной точкой $O=(O^1,...,O^n)$. \qed
\end{definition}

\begin{definition}
\AddIndex{Многообразие базисов
\ShowEq{Basis Manifold, Affine Space}
аффинного пространства}{Basis Manifold, Affine Space} %\index{manifold of}
- это множество базисов этого пространства.
\qed
\end{definition}

Мы будем называть активное преобразование
\AddIndex{аффинным преобразованием}{affine transformation}.
Мы будем называть пассивное преобразование
\AddIndex{квазиаффинным преобразованием}{quasi affine transformation}.

Если мы не заботимся о начальной точке вектора, мы получим несколько отличный
тип пространства, которое мы будем называть центро-аффинным пространством
\symb{\mathcal{CA}_n}{CAn}1.
В центро-аффинном пространстве мы можем идентифицировать все
касательные пространства и обозначить их $T\mathcal{CA}_n$.
Если мы предположим, что начальная точка
вектора - это начало $O$ координатной системы в пространстве,
то мы можем отождествить любую
точку $A\in\mathcal{CA}_n$ с вектором $a=\overset{\longrightarrow}{OA}$. Это ведёт
к идентификации $\mathcal{CA}_n$ и $T\mathcal{CA}_n$.
Теперь преобразование - это просто отображение
\begin{align*}
a'^i&=P^i_j a^j & \det P\ne 0
\end{align*}
и такие преобразования порождают группу Ли $GL_n$.

\begin{definition}
\AddIndex{Центро-аффинный базис}{Central Affine Basis}
\ShowEq{Central Affine Basis}
- это множество
линейно независимых векторов $\Vector e_i=(e^1_i,...,e^n_i)$.
\qed
\end{definition}

\begin{definition}
\AddIndex{Многообразие базисов
\ShowEq{BCAn}
центро-аффинного пространства}{Basis Manifold, Central Affine Space}
- это множество базисов этого пространства. \qed
\end{definition}

\section{Базис в евклидовом пространстве}
\labelSubsection{EuclideSpace}

Когда мы определяем метрику в центро-аффинном пространстве, мы
получаем новую геометрию потому, что
мы можем измерять расстояние и длину вектора. Если метрика
положительно определена, мы будем называть пространство евклидовым
\ShowEq{Euclid space}
в противном случае мы будем называть пространство псевдоевклидовым
\ShowEq{pseudo Euclid space}

Преобразования, которые сохраняют длину,
образуют группу Ли $SO(n)$ для евклидова пространства и группу Ли $SO(n,m)$ для
псевдоэвклидова пространства, где $n$ и $m$ числа положительных
и отрицательных слагаемых в метрике.

\begin{definition}
\AddIndex{Ортонормированный базис}{Orthonornal Basis}
\ShowEq{Orthonornal Basis}
- это множество
линейно независимых векторов $\Vector e_i=(e^1_i,...,e^n_i)$ таких, что длина
каждого вектора равна $1$ и различные векторы ортогональны.
\qed
\end{definition}

Существование ортогонального базиса доказывается с помощью
процесса ортогонализации Грама--Шмидта.

\begin{definition}
\AddIndex{Многообразие базисов
\ShowEq{BEn}
евклидова пространства}{Basis Manifold, Euclid Space}
- это множество ортонормированных базисов этого пространства.
\qed
\end{definition}

Мы будем называть активное преобразование
\AddIndex{движением}{movement transformation}.
Мы будем называть пассивное преобразование
\AddIndex{квазидвижением}{quasi movement}.

\section{Геометрический объект}
\labelSection{Geometric Object of Vector Space}

Активное преобразование изменяет базисы и векторы согласовано
и координаты вектора относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат вектора относительно базиса.

Допустим пассивное преобразование $a\in G$, заданное матрицей
$(a^i_j)$, отображает
базис $\Basis{e}=<e_i>\in\mathcal{B}(V)$
в базис $\Basis{e}'=<e'_i>\in\mathcal{B}(V)$
\ShowEq{passive transformation of vector space}
Допустим вектор $v\in V$ имеет разложение
\ShowEq{vector expansion in vector space, basis f}
относительно базиса $\Basis{e}$ и имеет разложение
\ShowEq{vector expansion in vector space, basis fprim}
относительно базиса $\Basis{e}'$.
Из \EqRef{passive transformation of vector space}
и \EqRef{vector expansion in vector space, basis fprim} следует, что
\ShowEq{vector expansion in vector space, basis f, 1}
Сравнивая \EqRef{vector expansion in vector space, basis f}
и \EqRef{vector expansion in vector space, basis f, 1} получаем, что
\ShowEq{coordinate transformation, 1}
Так как $a^i_j$ - невырожденная матрица, то
из \EqRef{coordinate transformation, 1} следует
\DrawEq['{}a]{passive coordinate transformation}1
Преобразование координат \eqRef{passive coordinate transformation}1
не зависит от вектора $v$ или базиса $\Basis{e}$, а
определенно исключительно координатами вектора $v$
относительно базиса $\Basis{e}$.

Если мы фиксируем базис $\Basis{e}$, то множество координат
\ShowEq{coordinates in vector space}
относительно этого базиса порождает векторное пространство
\ShowEq{coordinate vector space}
изоморфное векторному пространству $V$.
Это векторное пространство называется
\AddIndex{координатным векторным пространством}{coordinate vector space},
а изоморфизм
\AddIndex{координатным изоморфизмом}{coordinate isomorphism}.
Мы будем обозначать
\ShowEq{image of vector e_k, coordinate vector space}
образ вектора $e_k\in\Basis{e}$ при этом изоморфизме.

\begin{theorem}
\labelTheorem{coordinate transformations form representation, vector space}
Преобразования координат \eqRef{passive coordinate transformation}1
порождают левостороннее эффективное линейное
представление группы $G$, называемое
\AddIndex{контравариантным представлением}{contravariant representation}.
\end{theorem}
\begin{proof}
Допустим мы имеем два последовательных пассивных преобразования
$a\in G$ и $b\in G$. Преобразование координат
\DrawEq['{}a]{passive coordinate transformation}a
соответствует пассивному преобразованию $a$.
Преобразование координат
\DrawEq[{''}'b]{passive coordinate transformation}b
соответствует пассивному преобразованию $b$. Произведение
преобразований координат \eqRef{passive coordinate transformation}a
и \eqRef{passive coordinate transformation}b имеет вид
\ShowEq{coordinate transformation, ba}
и является координатным преобразованием,
соответствующим пассивному преобразованию $ab$.
Это доказывает, что преобразования координат
порождают контравариантное правостороннее линейное
представление группы $G$.

Если координатное преобразование не изменяет векторы $\delta_k$,
то ему соответствует единица группы $G$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}

Предположим,
что гомоморфизм группы $G$ в
группу пассивных преобразований
векторного пространства $W$ согласован с группой симметрий
векторного пространства $V$.
Это означает, что пассивному преобразованию $a\in G$ векторного пространства $V$
соответствует пассивное преобразование $A(a)$ векторного пространства $W$
\ShowEq{passive transformation of vector space W}
Тогда координатное преобразование в $W$ принимает вид
\ShowEq{coordinate transformation, W}

\begin{definition}
\labelDefinition{geometric object, coordinate representation}
Мы будем называть орбиту
\ShowEq{geometric object, coordinate vector space}
\ShowEq{geometric object, coordinate vector space, show}
\AddIndex{геометрическим объектом в координатном представлении}
{geometric object, coordinate vector space},
определённым в векторном пространстве $V$.
Для любого базиса
$\Basis{e}'_V=\Basis{e}_Va$
соответствующая точка \EqRef{coordinate transformation, W} орбиты  определяет
\AddIndex{координаты геометрического объекта}
{coordinates of geometric object, coordinate vector space}
относительно базиса $\Basis{e}'_V$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{geometric object}
Мы будем
называть орбиту
\ShowEq{geometric object, vector space}
\ShowEq{geometric object, vector space, show}
\AddIndex{геометрическим объектом}{geometric object, vector space},
определённым в векторном пространстве $V$.
Для любого базиса
$\Basis{e}'_V=\Basis{e}_Va$
соответствующая точка \EqRef{coordinate transformation, W} орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometric object, vector space}
относительно базиса $\Basis{e}'_V$
и соответствующий вектор
\ShowEq{representative of geometric object}{}
называется
\AddIndex{представителем геометрического объекта}
{representative of geometric object, vector space}
в базисе $\Basis{e}'_V$.
\qed
\end{definition}

Мы будем также говорить, что $w$ - это
\AddIndex{геометрический объект типа $A$}
{geometric object of type A, vector space}

Так как геометрический объект - это орбита представления,
то согласно теореме \RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Определение \RefDefinition{geometric object, coordinate representation}
строит геометрический объект в координатном пространстве.
Определение \RefDefinition{geometric object} предполагает,
что мы выбрали базис в векторном пространстве $W$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.

\begin{theorem}
(\AddIndex{принцип инвариантности}{invariance principle}).
\labelTheorem{invariance principle}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis{e}'_V$.
\end{theorem}
\begin{proof}
Для того, чтобы представитель геометрического объекта был определён,
мы должны выбрать базис $\Basis{e}_V$,
базис
$\Basis{e}_W=(e_{W\alpha})$
и координаты геометрического объекта
$w^\alpha$. Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{representative of geometric object}{}
Базис $\Basis{e}'_V$ связан с базисом
$\Basis{e}_V$ пассивным преобразованием $a\in G$.
Согласно построению это порождает пассивное преобразование
\EqRef{passive transformation of vector space W}
и координатное преобразование
\EqRef{coordinate transformation, W}. Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}

\begin{definition}
\labelDefinition{sum of geometric objects}
Пусть
\ShowEq{representative of geometric object}1
\ShowEq{representative of geometric object}2
геометрические объекты одного и того же типа,
определённым в векторном пространстве $V$.
Геометрический объект
\ShowEq{sum of geometric objects}
называется \AddIndex{суммой
\ShowEq{sum of geometric objects 1}
геометрических объектов}{sum of geometric objects, vector space}
$\Vector w_1$ и $\Vector w_2$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{product of geometric object and constant}
Пусть
\ShowEq{representative of geometric object}1
геометрический объект,
определённый в векторном пространстве $V$ над полем $F$.
Геометрический объект
\ShowEq{product of geometric object and constant}
называется \AddIndex{произведением
\ShowEq{product of geometric object and constant 1}
геометрического объекта $w_1$ и константы $k\in F$}
{product of geometric object and constant, vector space}.
\qed
\end{definition}

\begin{theorem}
Геометрические объекты типа $A$,
определённые в векторном пространстве $V$ над полем $F$,
образуют векторное пространство над полем $F$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из непосредственной проверки
свойств векторного пространства.
\end{proof}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\BiblioItem{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}%

\BiblioItem{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}%

\BiblioItem{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\BiblioItem{MVector}
{
Александр Клейн,
Линейное отображение D-алгебры,\\
eprint \href{http://arxiv.org/abs/MVector}{arXiv:MVector} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Теория представлений универсальной алгебры,\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{1812.03397}
{
Ivan Kyrchei,
Linear differential systems over the quaternion skew field,\\
eprint \href{http://arxiv.org/abs/1812.03397}{arXiv:1812.03397} (2018)
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{1510.02224}
{
Kit Ian Kou, Yong-Hui Xia.
Linear Quaternion Differential Equations: Basic Theory and Fundamental Results.\\
eprint \href{http://arxiv.org/abs/1510.02224}{arXiv:1510.02224} (2017)
}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,\\
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Gen.Relativity.Russian.tex <==
%auto-ignore

\input{Gen.Relativity.Eq}

\ifx\PrintBook\Defined
\chapter{Приложения в общей теории относительности}
\fi

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
\section{Синхронизация системы отсчёта}
\labelSection{Synchronization of Reference Frame}

Так как наблюдатель пользуется ортогональным базисом для измерения в каждой точке,
мы можем ожидать, что он также пользуется неголономными координатами.
Мы так же видим, что координата времени вдоль локальной системы отсчёта
является собственным временем наблюдателя.
Так как система отсчёта состоит из локальных систем отсчёта,
мы ожидаем, что их собственные времена синхронизированы.

Мы определяем \AddIndex{синхронизацию системы отсчёта}{synchronization of reference frame}
как неголономную координату времени.

Так как синхронизация - это неголономная координата, это порождает
новые физические явления,
которые мы должны иметь в виду, когда работаем с сильными гравитационными полями
или выполняем точные измерения. Ниже я опишу одно из этих явлений.
\fi

\section{Неголономные координаты в гравитационном поле центрального тела}
\labelSection{Anholonomic Coordinates in Central Body Gravitational Field}

Мы будем изучать наблюдателя, вращающегося вокруг центрального тела.
Результаты оценочны и хороши, когда эксцентриситет около $0$,
так как мы будем изучать круговую орбиту.
Тем не менее, основная цель этой оценки - показать, что мы имеем
измеримое действие неголономности.

Мы пользуемся метрикой Шварцшильда для центрального тела
\ShowEq{Schwarzschild metric}
$$r_g = \frac {2 G m} {c^2}$$
$G$ - гравитационная константа, $m$ - масса центрального тела,
$c$ - скорость света.

Эта метрика имеет связность
\ShowEq{Schwarzschild metric, Connection}

Неголономный базис имеет вид
\ShowEq{Schwarzschild metric 1}
Объект неголономности имеет вид
\DrawEq{Schwarzschild metric 2}{note19}
Из равенства
\eqRef{Schwarzschild metric 2}{note19}
следует, что
для изучения влияния неголономности на синхронизацию системы отсчёта
мы должны рассмотреть радиальное движение.

Пусть Джон путешествует в радиальном направлении.
Начальная точка траектории удалена от центра гравитации на расстоянии $R_1$
(точка $A$).
Когда Джон удалился на расстояние $R_2$ от центра гравитации (точка $B$),
он делает остановку и возвращается в исходное положение.
Его друг Джеймс остаётся в точке $A$
и ждёт возвращения Джона.

Мы предполагаем, что все часы в системе отсчёта Джеймса синхронизированы.
Джон понимает, что показание его часов отличается от показаний часов
в системе отсчёта Джеймса.
Поэтому Джон периодически проверяет показание часов в системе отсчёта Джеймса.
Когда Джон вновь встречает Джеймса, они сверяют свои результаты измерения времени.

Пусть $v$ - скорость, с которой движется Джон в системе отсчёта Джеймса.
Пусть
\ShowEq{experiment, step 1}
начальное движение мяча.
Равенство
\ShowEq{experiment, t1=dR/v}
является следствием
\EqRef{experiment, step 1}.
Равенство
\ShowEq{experiment, d1t=}
является следствием равенства
\ShowEq{experiment, dt=int}
а так же равенств
\EqRef{experiment, step 1},
\EqRef{experiment, t1=dR/v}.

Нужно сперва взять неопределённый интеграл
(я пользуюсь заменой переменной
\ShowEq{experiment, r=R1+vt})
\ShowEq{experiment, d1t= indefinite}
Пусть
\ShowEq{experiment, u2=r/r}
Тогда
\ShowEq{experiment, r=..u2}
\ShowEq{experiment, dr=..du}
Равенство
\ShowEq{experiment, d1t= indefinite 1}
является следствием равенств
\EqRef{experiment, d1t= indefinite},
\EqRef{experiment, r=..u2},
\EqRef{experiment, dr=..du}.
Пусть
\ShowEq{experiment, u2/u2=abcd}
Система уравнений
\ShowEq{experiment, u2/u2 abcd=}
являются следствием равенства
\EqRef{experiment, u2/u2=abcd}.
Система уравнений
\ShowEq{experiment, u2/u2 abcd= 1}
является следствием системы уравнений
\EqRef{experiment, u2/u2 abcd=}.
Равенство
\ShowEq{experiment, u2/u2 abcd= 2}
является следствием системы уравнений
\EqRef{experiment, u2/u2 abcd= 1}.
Равенство
\ShowEq{experiment, d1t= indefinite 2}
является следствием равенств
\EqRef{experiment, d1t= indefinite 1},
\EqRef{experiment, u2/u2=abcd},
\EqRef{experiment, u2/u2 abcd= 2}.

Если $x^0$ меняется от $0$ до $t_1$,
то $r$ меняется от $R_1$ до $R_2$
и $u$ меняется от
\ShowEq{experiment, u=u1}1
до
\ShowEq{experiment, u=u1}2
Так как время движения в обоих направлениях одно и тоже, то мы получим
\ShowEq{experiment, d1t+d2t}

Осталось посчитать время, как долго Джеймс ждал возвращение Джона.
Равенство
\ShowEq{experiment, d3t=}
является следствием равенства
\EqRef{experiment, dt=int}.

Для анализа результатов эксперимента,
я предположу, что вместо того, чтобы Джон путешествовал
из точки $A$ в точку $B$ и обратно,
Джеймс отправит пучок света ($v=c=2.998e10$ см/сек) в точку $B$, где установлено зеркало,
которое вернёт пучок света обратно в точку $A$.
Пусть точка $A$ находится на поверхности Земли
($R_1=6.371e8$ сантиметров, расстояние от центра Земли)
и точка $B$ находится на поверхности Луны
($R_2=3.84e10$ сантиметров).\,\footnote{
Результаты расчёта являются оценкой,
так как в рассчёте я не учитываю гравитационное поле Луны.
}
Время, которое измерил Джеймс, равно $2.5192061357$ секунд.
Время, которое измерил луч света, равно $2.5192002762$ секунд.
Так как фаза волны светового пучка зависит от локального времени
в системе отсчёта Джеймса, то
Джеймс может использовать интерференцию
исходного луча света и вернувшегося луча света,
чтобы наблюдать отклонение интерференции
от ожидаемой картины.

\section{Эффект Допплера в гравитационном поле центрального тела}

Я хочу показать ещё один способ
рассчёта эффекта Допплера. Эффект Допплера в гравитационном поле является
хорошо изученным явлением, однако метод, который я покажу полезен, чтобы
лучше понять физику гравитационного поля.

Мы можем описать движение фотона в гравитационном поле,
пользуясь его волновым вектором $k^i$. Длина этого вектора равна 0;
$\frac {k^i} {dx^i} = const$; траектория является
геодезической, и следовательно, координаты этого вектора удовлетворяют
дифференциальному уравнению
\begin{equation}
dk^i = -\Gamma^i_{kl}k^k dx^l
\EqLabel{Transport}
\end{equation}

Мы ищем частоту $\omega$ света
и $k^0$ пропорционально $\omega$.
Рассмотрим радиальное движение фотона. В этом случае волновой вектор имеет вид 
$k=(k^0,k^1,0,0)$.
В центральном поле с метрикой
\EqRef{Schwarzschild metric} мы можем выбрать
\[k^0=\frac \omega c \sqrt{\frac r {r-r_g}}\]
\[k^1=\omega \sqrt{\frac {r-r_g} r}\]
\[dt=\frac {k^0} {k^1} dr= \frac 1 c \frac r {r-r_g}dr\]
Тогла уравнение \EqRef{Transport} принимает вил
\[dk^0=-\Gamma^0_{10}(k^1 dt + k^0 dr)\]
\[d\left(\frac\omega c \sqrt{\frac r {r-r_g}}\right)=
-\frac{r_g \omega} {2r(r-r_g)}\left(\sqrt{\frac {r-r_g} r}\frac r {r-r_g}
+\sqrt{\frac r {r-r_g}}\right)\frac {dr} c\]
\[d\omega \sqrt{\frac r {r-r_g}}-\omega\frac 1 2 \sqrt{\frac {r-r_g}r}
\frac {r_gdr} {(r-r_g)^2}
=-\frac {r_g\omega dr} {r(r-r_g)}\sqrt{\frac r {r-r_g}}\]
\[\frac  {d\omega} \omega
=-\frac {r_g} {2r(r-r_g)}dr\]
\[\ln  \omega
=\frac 1 2 \ln \frac r {r-r_g} + \ln C\]
Если мы определим $\omega = \omega_0$, когда $r=\infty$, мы получим окончательно 
\[\omega
=\omega_0\sqrt{\frac r {r-r_g}}\]

\ePrints{0803.3276}
\ifx\Semafor\ValueOff
\section{Задержка времени в гравитационном поле центрального тела}
\labelSection{Time Delay in Central Body Gravitational Field}

Мы изучим вращение вокруг центрального тела.
Результаты являются только оценкой и хороши, когда эксцентриситет около $0$,
так как мы изучаем круговые орбиты.
Основная задача этой оценки - показать, что мы имеем измеримый эффект негологомности.

Давайте сравним измерения двух наблюдателей. Первый наблюдатель
зафиксировал своё положение в гравитационном поле
$$t=\frac s  c \sqrt{\frac r {r-r_g}}$$ $$r=const, \phi=const, \theta=const$$
Второй наблюдатель вращается вокруг центра поля с постоянной скоростью
$$t=s \sqrt{\frac r {(r-r_g) c^2 - \alpha^2 r^3}}$$
$$\phi=\alpha\ s \sqrt{\frac r {(r-r_g) c^2 - \alpha^2 r^3}}$$
$$r=const,\theta=const$$
Мы выберем натуральный параметр для обоих наблюдателей.

Второй наблюдатель начинает своё путешествие,
когда $s=0$, и завершает его, когда возвращается к той же точке пространства.
Так как $\phi$ - циклическая координата, второй наблюдатель завершает своё путешествие,
когда $\phi=2\pi$. В этой точке мы имеем
$$s_2=\frac{2\pi} \alpha \sqrt{\frac{(r-r_g) c^2 - \alpha^2 r^3} r}$$
$$t=T=\frac{2\pi} \alpha$$
Значение натурального параметра первого наблюдателя в этой точке
$$s_1=\frac{2\pi} \alpha c\sqrt{\frac{r-r_g} r}$$
Разница между их собственными временами
$$
\Delta s = s_1 - s_2
=\frac{2\pi} \alpha
\left(c\sqrt{\frac{r-r_g} r}-\sqrt{\frac{(r-r_g) c^2 - \alpha^2 r^3} r}\right)
$$
Мы определили разницу в сантиметрах. Чтобы получить разницу в секундах,
мы должны делить обе части на c.
$$\Delta t = \frac{2\pi} \alpha
\left(\sqrt{\frac{r-r_g} r}-\sqrt{\frac{r-r_g} r - \frac{\alpha^2 r^2} {c^2}}\right)$$

Перейдём к конкретным данным.

Масса Солнца равна $1.989_{10}33$ г, Земля вращается вокруг Солнца на
расстоянии $1.495985_{10}13$ см от его центра напротяжение $365.257$ дней.
В этом случае мы получим
$\Delta t = 0.155750625445089$ сек. Меркурий вращается вокруг Солнца на
расстоянии $5.791_{10}12$ см от его центра напротяжение $58.6462$ дней.
В этом случае мы получим
$\Delta t = 0.145358734930827$ сек.

Масса Земли равна $5.977_{10}27$ г. Космический корабль,
который вращается вокруг Земли на
расстоянии $6.916_{10}8$ см от его центра напротяжение $95.6$ мин
имеет $\Delta t = 1.8318_{10}-6$ сек.
Луна вращается вокруг Земли на
расстоянии $3.84_{10}10$ см от его центра напротяжение $27.32$ дней.
В этом случае мы получим
$\Delta t = 1.372_{10}-5$ сек.

Для лучшего представления я поместил эти данные в
таблицы \ref{table: Effect of Anholonomic Coordinates, Sun},
\ref{table: Effect of Anholonomic Coordinates, Earth},
и \ref{table: Effect of Anholonomic Coordinates, Sgr A}.

Так как часы первого наблюдателя в момент встречи показывают большее
значение, он оценивает возраст второго наблюдателя
старше реального. Так, если взять параметры орбиты S2 из \citeBib{Ghez},
то мы получим, что за 10 Myr S2 будет моложе на .297 Myr по сравнению
с оценкой неподвижного наблюдателя.

\begin{table}[ht]
\caption{Солнце - центральное тело, масса - $1.989_{10}33$ г}
\label{table: Effect of Anholonomic Coordinates, Sun}
\noindent\[
\begin{tabular}{|c|c|c|}
\hline
спутник&Земля&Меркурий\\
\hline
расстояние, см&$1.495985_{10}13$&$5.791_{10}12$\\
\hline
период вращения, дней&$365.257$&$58.6462$\\
\hline
задержка времени, сек&$0.15575$&$0.14536$\\
\hline
\end{tabular}
\]
\end{table}

\begin{table}[ht]
\caption{Земля - центральное тело, масса - $5.977_{10}27$ г}
\label{table: Effect of Anholonomic Coordinates, Earth}
\noindent\[
\begin{tabular}{|c|c|c|}
\hline
спутник&космический корабль&Луна\\
\hline
расстояние, см&$6.916_{10}8$&$3.84_{10}10$\\
\hline
период вращения&$95.6$ mins&$27.32$ дней\\
\hline
задержка времени, сек&$1.8318_{10}-6$&$1.372_{10}-5$\\
\hline
\end{tabular}
\]
\end{table}

\begin{table}[ht]
\caption{Sgr A - центральное тело, S2 - спутник}
\label{table: Effect of Anholonomic Coordinates, Sgr A}
\noindent\[
\begin{tabular}{|c|c|c|}
\hline
масса, $M_\odot$&$4.1_{10}6$&$3.7_{10}6$\\
\hline
расстояние, см&$1.4692_{10}16$&$1.1565_{10}16$\\
\hline
период вращения, лет&$15.2$&$15.2$\\
\hline
задержка времени, мин&$164.7295$&$153.8326$\\
\hline
\end{tabular}
\]
\end{table}
\fi

\section{Преобразование Лоренца в орбитальном направлении}
\labelSection{Lorentz Transformation in Orbital Direction}

Причина задержки времени, которую мы оценили выше, находится в преобразовании Лоренца
между стационарным и вращающимся наблюдателями.
Это значит, что мы имеем вращение в плоскости $(e_{(0)}, e_{(2)})$.
Базисные вектора для стационарного наблюдателя - это
\[e_{(0)}=(\frac 1 c \sqrt{\frac r {r-a}}, 0, 0, 0)\]
\[e_{(2)}=(0, 0, \frac 1 r, 0)\]
Мы предположим, что для вращающегося наблюдателя изменение $\phi$ и $t$
пропорциональны и
\[d\phi=\omega dt\]
Единичный вектор скорости в этом случае должен быть пропорционален вектору
\begin{equation}
(1, 0, \omega, 0)
\label{NewVectorE2}
\end{equation}
Длина этого вектора
\begin{equation}
L^2=\frac {r-a} r c^2 - r^2 \omega^2
\label{LengthNewVectorE2}
\end{equation}
Мы видим в этом выражении очень знакомый узор и ожидаем, что линейная
скорость вращающегося наблюдателя $V = \omega r$.

Тем не менее, мы должны помнить, что мы выполняем измерение в гравитационном
поле и координаты являются лишь ярлыками для разметки точек в пространстве\Hyph времени.
Это значит, что нам нужен корректный метод для измерения скорости.

Если объект движется от точки $(t, \phi)$ к точке $(t+dt, \phi+d\phi)$
мы должны измерить пространственные и временные интервалы между этими точками.
Мы предположим, что в обеих точках имеются наблюдатели $A$ и $B$.
Наблюдатель $A$ посылает одновременно световой сигнал $B$ и мяч, который имеет
угловую скорость $\omega$. Каждый раз, когда
наблюдатель $B$ получает какую-то информацию, он посылает световой сигнал
обратно $A$.

Когда $A$ получает первый сигнал, он может оценить расстояние до $B$.
Когда $A$ получает второй сигнал, он может оценить, как долго двигался мяч до $B$.

Время путешествия света в обоих направлениях одно и тоже.
Траектория света определена уравнением $ds^2=0$.
В данном случае мы имеем
\[\frac {r-r_g} r c^2 dt^2 - r^2 d\phi^2 = 0\]
Когда свет возвращается к наблюдателю $A$, изменение $t$ равно
\[dt=2 \sqrt{\frac r {r-r_g}} c^{-1}r d\phi\]
Собственное время первого наблюдателя равно
\[ds^2= \frac {r-r_g} r c^2 4 \frac r {r-r_g}c^{-2}r^2 d\phi^2\]
Следовательно, пространственное расстояние
\[L=r d\phi\]
Когда объект, движущийся с угловой скорость $\omega$, прибывает в $B$,
изменение $t$ равно $\frac {d\phi} \omega$.
Собственное время в этой точке равно 
\[ds^2 = \frac {r - r_g} r c^2 d\phi^2 \omega^{-2}\]
\[T = \sqrt{\frac {r - r_g} r} \omega^{-1} d\phi\]
Следовательно, наблюдатель $A$ измеряет скорость
\[V=\frac L T = \sqrt{\frac r {r - r_g}} r\omega\]

Мы можем использовать скорость $V$ как параметр преобразования Лоренца.
Тогда длина
\eqref{LengthNewVectorE2} вектора \eqref{NewVectorE2} равна
\[L=\sqrt{\frac {r-r_g} r \left(c^2 - \frac r {r-r_g}r^2 \omega^2\right)}=
\sqrt{\frac {r-r_g} r} c\sqrt{\left(1 - \frac {V^2}{c^2}\right)}\]
Следовательно, временной орт движущегося наблюдателя
\[e'_{(0)}=\left(\frac 1 L, 0, \frac \omega L, 0\right)\]
\[e'_{(0)}=\left(\sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0,
\omega \sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0\right)\]
Пространственный орт $e'_{(2)}=(A,0,B,0)$ ортогонален $e'_{(0)}$ и имеет длину $-1$. Следовательно,
\begin{equation}
\frac {r-r_g} r c^2\frac 1 L A - r^2 \frac \omega L B = 0
\label{NewVectorE0_1}
\end{equation}
\begin{equation}
\frac {r-r_g} r c^2 A^2 - r^2 B^2 = -1
\label{NewVectorE0_2}
\end{equation}
Мы можем выразить $A$ из \eqref{NewVectorE0_1}
\[A = c^{-2}\frac r{r-r_g} r^2 \omega B\]
и подставить в \eqref{NewVectorE0_2}
\[ c^{-2}\frac r{r-r_g} r^4 \omega^2 B^2 - r^2 B^2 = -1\]
\[\frac {V^2}{c^2} r^2 B^2 - r^2 B^2 = -1\]
Окончательно пространственный орт в направлении движения
\[e'_{(2)}=\left(c^{-2}\frac r{r-r_g} r \omega \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}},
0,\frac 1 r \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}},0\right)\]
\[e'_{(2)}=\left(c^{-2}\sqrt{\frac r{r-r_g}} \frac V {\sqrt{1 - \frac {V^2}{c^2}}},
0,\frac 1 r \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}},0\right)\]

Следовательно, мы получим преобразование
\begin{equation}
\begin{split}
{e'}_{(0)}=\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac V  c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(2)}
\\
{e'}_{(2)}=\frac V c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(2)}
\end{split}
\label{Lorentz}
\end{equation}
Если стационарный наблюдатель посылает свет в радиальном направлении,
вращающийся наблюдатель наблюдает эффект Допплера
$$
\omega'=\frac \omega {\sqrt{1 - \frac {V^2} {c^2}}}
$$
Мы должны добавить эффект Допплера для гравитационного поля,
если движущийся наблюдатель получает радиальную волну, которая пришла из
бесконечности. В этом случае эффект Допплера примет форму
$$
\omega'=\sqrt{\frac r {r-r_g}}\frac \omega {\sqrt{ 1 - \frac {V^2} {c^2}}}
$$

Мы приводим оценку для динамики звезды S2, которая вращается вокруг Sgr A
в таблицах \ref{table:DShift1S2} и \ref{table:DShift2S2}.
Таблицы основаны на двух различных оценках для массы Sgr A.

\begin{sloppypar}
Если мы возьмём массу Sgr $4.1_{10}6 M_\odot$ \citeBib{Ghez}, то
в перицентре (расстояние $1.868_{10}15$ см) S2 имеет скорость $738767495.4$ см/сек
и эффект Допплера равен $\omega'/\omega=1.000628$. В этом случае мы измеряем длину $2.16474 \mu m$
для волны, излучаемой с длиной $2.1661 \mu m$ (Br $\gamma$).
В апоцентре (расстояние $2.769_{10}16cm$) S2 имеет скорость $49839993.28cm/s$
и эффект Допплера равен $\omega'/\omega=1.0000232$. Мы измеряем длину $2.166049 \mu m$
для той же самой волны.
Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$13.098$\AA.
\end{otherlanguage}

Если мы возьмём массу Sgr $3.7_{10}6 M_\odot$ \citeBib{Schodel}, то
в перицентре (расстояние $1.805_{10}15cm$) S2 имеет скорость $713915922.3cm/s$
и эффект Допплера равен $\omega'/\omega=1.000587$. В этом случае мы измеряем длину $2.16483 \mu m$
для волны, излучаемой с длиной $2.1661 \mu m$ (Br $\gamma$).
В апоцентре (расстояние $2.676_{10}16cm$) S2 имеет скорость $48163414.05cm/s$
и эффект Допплера равен $\omega'/\omega=1.00002171$. Мы измеряем длину $2.1666052 \mu m$
для той же самой волны.
Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$12.232$\AA.
\end{otherlanguage}
\end{sloppypar}

\begin{table}[ht]
\caption{эффект Допплера на Земле для волны, излучаемой с S2;
масса Sgr A равна $4.1_{10}6 M_\odot$ \citeBib{Ghez}}
\label{table:DShift1S2}
\begin{tabular}{|c|c|c|}
\hline
&перицентр&апоцентр\\
\hline
расстояние см&$1.868_{10}15$&$2.769_{10}16$\\
\hline
скорость см/s&$738767495.4$&$49839993.28$\\
\hline
$\omega'/\omega$&$1.000628$&$1.0000232$\\
\hline
излучаемая волна $(Br\ \gamma)\ \mu m$& $2.1661$&$2.1661$\\
\hline
наблюдаемая волна $\mu m$&$2.16474$ &$2.166049$\\
\hline
\end{tabular}

Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$13.098$\AA.
\end{otherlanguage}
\end{table}

\begin{table}[ht]
\caption{эффект Допплера на Земле для волны, излучаемой с S2;
масса Sgr A равна $3.7_{10}6 M_\odot$ \citeBib{Schodel}}
\label{table:DShift2S2}
\begin{tabular}{|c|c|c|}
\hline
&перицентр&апоцентр\\
\hline
расстояние см&$1.805_{10}15$&$2.676_{10}16$\\
\hline
скорость см/s&$713915922.3$&$48163414.05$\\
\hline
$\omega'/\omega$&$1.000587$&$1.00002171$\\
\hline
излучаемая волна $(Br\ \gamma)\ \mu m$& $2.1661$&$2.1661$\\
\hline
наблюдаемая волна $\mu m$&$2.16483$ &$2.1666052$\\
\hline
\end{tabular}

Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$12.232$\AA.
\end{otherlanguage}
\end{table}

Разность между двумя измерениями длины волны в перицентре равна
\begin{otherlanguage}{english}
$0.9$\AA.
\end{otherlanguage}
Анализируя эти данные, мы приходим к заключению, что
использование эффекта Допплера может помочь улучшить оценку
массы Sgr A.

\section{Преобразование Лоренца в радиальном направлении}

Мы видим, что преобразование Лоренца в орбитальном направлении имеет знакомый вид.
Очень интересно увидеть, какой вид это преобразование имеет в радиальном направлении.
Мы начнём с процедуры измерения скорости и будем пользоваться координатной скоростью $v$
\begin{equation}
dr=vdt
\EqLabel{RadialSpeed}
\end{equation}
Время путешествия света в обоих направлениях одно и тоже.
Траектория света определена уравнением $ds^2=0$.
\[\frac {r-r_g} r c^2 dt^2 - \frac r {r-r_g} dr^2 = 0\]
Когда свет возвращается к наблюдателю $A$, изменение $t$ равно
\[dt=2 \frac r {r-r_g} c^{-1} dr\]
Собственное время наблюдателя $A$ равно
\ShowEq{proper time, observer A, Radial Direction}
Следовательно, пространственное расстояние равно
\[L=\sqrt{\frac r {r-r_g}} dr\]
Когда объект, движущийся со скоростью \EqRef{RadialSpeed}, прибывает в $B$
изменение $t$ равно $\frac {dr} v$.
Собственное время наблюдателя $A$ в этой точке 
\[ds^2 = \frac {r - r_g} r c^2 dr^2 v^{-2}\]
\[T = \sqrt{\frac {r - r_g} r} v^{-1} dr\]
Следовательно, наблюдатель $A$ измеряет скорость
\begin{align*}
V&=\frac L T =
=\frac{\sqrt{\frac r {r-r_g}} dr}{\sqrt{\frac {r - r_g} r} v^{-1} dr}=\\
&=\frac r {r-r_g} v
\end{align*}

Теперь мы готовы найти преобразование Лоренца.
Базисные вектора для стационарного наблюдателя - это
\[e_{(0)}=\left(\frac 1 c \sqrt{\frac r {r-r_g}}, 0, 0, 0\right)\]
\[e_{(1)}=\left(0,  \sqrt{\frac {r-r_g} r},0, 0\right)\]

Единичный вектор скорости должен быть пропорционален вектору
\begin{equation}
(1, v, 0, 0)
\EqLabel{NewRadialVectorE1}
\end{equation}
Длина этого вектора
\begin{equation}
\begin{split}
L^2&=\frac {r-r_g} r c^2 - \frac r {r-r_g} v^2=\\
&=\frac {r-r_g} r c^2\left(1 - \frac {V^2}{c^2}\right)
\EqLabel{LengthNewRadialVectorE1}
\end{split}
\end{equation}
Следовательно, временной орт движущегося наблюдателя
\begin{align*}
e'_{(0)}&=\left(\frac 1 L,  \frac v L,0, 0\right)=\\
&=\left(\sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 
v \sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0,0\right)\\
&=\left(\sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 
\frac V c \sqrt{\frac {r-r_g} r}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0,0\right)
\end{align*}
Пространственный орт $e'_{(1)}=(A,B,0,0)$ ортогонален $e'_{(0)}$ и имеет длину $-1$. Следовательно,
\begin{equation}
\frac {r-r_g} r c^2\frac 1 L A - \frac r {r-r_g} \frac v L B = 0
\label{NewRadialVectorE0_1}
\end{equation}
\begin{equation}
\frac {r-r_g} r c^2 A^2 - \frac r {r-r_g} B^2 = -1
\label{NewRadialVectorE0_2}
\end{equation}
Мы можем выразить $A$ из \eqref{NewRadialVectorE0_1}
\[A = c^{-2}\frac {r^2}{(r-r_g)^2} v B = c^{-2}\frac r{r-r_g} V B\]
и подставить в \eqref{NewRadialVectorE0_2}
\[\frac {r-r_g} r c^2 c^{-4}\frac {r^2}{(r-r_g)^2} V^2 B^2 - \frac r {r-r_g} B^2 = -1\]
\[\frac r{r-r_g} B^2\left(1- \frac{V^2}{c^2} \right) = 1\]
\[ B^2 = \frac{r-r_g} r\frac 1{1- \frac{V^2}{c^2} }\]
\[ B = \sqrt{\frac{r-r_g} r}\frac 1{\sqrt{1- \frac{V^2}{c^2}} }\]
\begin{align*}
A &= c^{-2}\frac r{r-r_g} V \sqrt{\frac{r-r_g} r}\frac 1{\sqrt{1- \frac{V^2}{c^2}} }\\
&= c^{-2} V \sqrt{\frac r{r-r_g}}\frac 1{\sqrt{1- \frac{V^2}{c^2}} }
\end{align*}
Окончательно пространственный орт в направлении движения
\[e'_{(1)}=\left(c^{-2} V \sqrt{\frac r{r-r_g}}\frac 1{\sqrt{1- \frac{V^2}{c^2}} },
\sqrt{\frac{r-r_g} r}\frac 1{\sqrt{1- \frac{V^2}{c^2}} },0,0\right)\]

Следовательно, мы подучаем преобразование в знакомой форме
\begin{equation}
\begin{split}
{e'}_{(0)}=\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac V  c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(1)}
\\
{e'}_{(1)}=\frac V c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(1)}
\end{split}
\label{RadialLorentz}
\end{equation}

\section{Эффект Допплера в пространстве Фридмана}
\labelSection{Doppler Shift in Friedman Space}

Мы рассмотрим другой пример в пространстве Фридмана. Метрика
пространства имеет вид
$$ds^2 = a^2 (dt^2
- d\chi^2 - \sin^2\chi (d\theta^2 - \sin^2 \theta d\phi^2))
$$
для закрытой модели и
$$ds^2 = a^2 (dt^2
- d\chi^2 - \sinh^2\chi (d\theta^2 - \sin^2 \theta d\phi^2))
$$
для открытой модели. Связность пространства
($\alpha$, $\beta$ принимают значения 1, 2, 3)
\[\Gamma^0_{00}=\frac {\dot{a}} a\]
\[\Gamma^0_{\alpha\alpha}=-\frac {\dot{a}} {a^2}g_{\alpha\alpha}\]
\[\Gamma^\alpha_{0\beta}=\frac {\dot{a}} a\delta^\alpha_\beta\]

Поскольку пространства однородно, для нас не имеет значение
направление распространения света.
В этом случае
\[dk^0=-\Gamma^0_{ij}k^i k^j\]
Так как $k$ - изотропный вектор, касательный к его траектории, мы имеем
\[dx^\alpha=\frac {k^\alpha} {k^0}dt\]
Так как $k^0=\frac \omega a$, то
\[d\frac \omega a=-\frac {da} {a^2}\omega+\frac {da} {\omega a}g_{\alpha\alpha}k^\alpha k^\alpha=
-2\frac {da} {a^2}\omega\]
\[ad\omega+\omega da=0\]
\[a\omega=const\]
Следовательно, когда $a$ растёт,
$\omega$ становится меньше и длина волны растёт. 

$a$ растёт, когда свет путешествует сквозь пространство\Hyph время,
и это приводит к красному смещению.
Причиной наблюдаемого красного смещения
является не разбегание галактик,
а изменение геометрии.

Рассмотрим теперь как красное смещение меняется во времени,
если начальная и конечная точки не движутся.
Для простоты я буду изменять только $\chi$. $\chi_1$ - начальное значение
и $\chi_2$ - конечное значение. Так как на траектории
света $dt=d\chi$, мы имеем
\[\chi = \chi_1 + t - t_1\ \ \ \ t_2 = \chi_2 - \chi_1 + t_1\]
Следовательно $a(t_1) \omega_1 = a(t_2) \omega_2$.
Смещение Допплера имеет вид
\[K(t_1) =\frac {\omega_2} {\omega_1} = \frac {a(t_1)} {a(t_2)}\]
Если начальное время изменяется
\ShowEq{t'1=t1+dt}
t'1 = t1 + dt,
то
\ShowEq{K(t1+dt)=}
Производная $K$ по времени имеет вид    
\[\dot{K} = \frac {\dot{a}_1 a_2 - a_1 \dot{a}_2} {a_2^2}\]

Для замкнутого пространства $a = \cosh t$. Тогда $\dot{a} = \sinh t$. 
\[\dot{K} = \frac{\sinh t_1 \cosh t_2 - \sinh t_2 \cosh t_1} {\cosh^2 t_2}
= \frac{\sinh(t_1 - t_2)} {\cosh^2 t_2}\] 
$K$ уменьшается, когда $t_1$ увеличивается. 

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
\section{Преобразование Лоренца в пространстве Фридмана}
\labelSection{Lorentz Transformation in Friedman Space}

Чтобы изучить преобразование Лоренца в пространстве Фридмана,
я хочу воспользоваться метрикой в форме
\[ds^2=c^2 dt^2 -a^2(d\chi^2 + b^2(d\theta^2 - \sin^2 \theta d\phi^2))\]
У меня есть два наблюдателя. Один не движется и имеет скорость $(1,0,0,0)$,
а другой движется вдоль $\chi$ и его скорость
имеет вид $C=(1,v,0,0)$, и мы положим $V=a v$.

Метрика диагональна и координаты $\theta, \phi$ не меняются.
У нас возникает преобразование в плоскости $t, \chi$.

Единичная скорость первого наблюдателя имеет вид
\[e_0 = (\frac 1 c , 0, 0, 0)\]
и вектор, ортогональный ей, имеет вид
\[e_1 = (0, \frac 1 a , 0, 0)\]

Длина вектора $C$ имеет вид
\[L=\sqrt{c^2 - a^2 v^2} = c \sqrt{1 - \frac{V^2} {c^2}}\]
Следовательно, единичный вектор скорости второго наблюдателя имеет вид
\[e'_0=(\frac 1 L, \frac v L, 0, 0)\]
Мы ищем вектор
\[e'_1=(A, B, 0, 0)\]
который ортогонален вектору $e'_0$. Для этого мы имеем
\begin{equation}
c^2 A^2 - a^2 B^2 = -1
\EqLabel{length of vector, e1, 1}
\end{equation}
\begin{equation}
c^2 A \frac 1 L - a^2 B \frac v L = 0
\EqLabel{length of vector, e1, 2}
\end{equation}
Мы получим из уравнения \EqRef{length of vector, e1, 2}
\begin{equation}
A = \frac {a^2} {c^2} v B
\EqLabel{length of vector, e1, 3}
\end{equation}
Мы подставим \EqRef{length of vector, e1, 3}
в \EqRef{length of vector, e1, 1} и получим
\[B^2 (\frac {a^4} {c^2} v^2 - a^2) = -1\] 
\[B = \frac 1 {a \sqrt{1 - \frac {V^2} {c^2}}}\]
Следовательно базис второго наблюдателя имеет вид
\[e'_0=(\frac 1 {c \sqrt{1 - \frac{V^2} {c^2}}}, \frac V {c a\sqrt{1 - \frac{V^2} {c^2}}}, 0, 0)\]
\[e'_1=( \frac V {c^2 \sqrt{1 - \frac {V^2} {c^2}}},
\frac 1 {a \sqrt{1 - \frac {V^2} {c^2}}}, 0, 0)\]
Теперь мы можем выразить $e'$ через $e$
\[e'_0= \frac 1 {\sqrt{1 - \frac {V^2} {c^2}}} e_0
+ \frac V c \frac 1 {\sqrt{1 - \frac{V^2} {c^2}}} e_1\]
\[e'_1= \frac V c \frac 1 {\sqrt{1 - \frac{V^2} {c^2}}} e_0
+ \frac 1 {\sqrt{1 - \frac{V^2} {c^2}}} e_1\] 
\fi


==> Geom.Object.Russian.tex <==
%auto-ignore

\ePrints{0803.3276}
\ifx\Semafor\ValueOff

\ifx\PrintBook\Defined
\chapter{Геометрический объект}
\fi

\section{Метрико-аффинное многообразие}
\labelSection{Metric-affine Manifold}

В случае связности
\EqRef{GLn connection form}
мы определим \AddIndex{форму кручение}{torsion form}
\begin{equation}
T^a = d^2 x^a + \omega^a_b \wedge dx^b
\EqLabel{Torsion}
\end{equation}
Из \EqRef{GLn connection form} следует
\begin{equation}
\omega^a_b \wedge dx^b=(\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
\EqLabel{wedge connection}
\end{equation}
Подставляя \EqRef{wedge connection} и \EqRef{anholonomity} в \EqRef{Torsion}
мы получим
\begin{equation}
T^a=T^a_{cb}dx^c\wedge dx^b =
-c^a_{cb}dx^c\wedge dx^b + (\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
\EqLabel{Torsion 1}
\end{equation}
где мы определили \AddIndex{тензор кручения}{torsion tensor}
\begin{equation}
T^a_{cb} =
\Gamma^a_{bc}-\Gamma^a_{cb}-c^a_{cb}
\EqLabel{Torsion coordinates}
\end{equation}

Коммутатор вторых производных имеет вид
\begin{equation}
u^\alpha_{;kl}-u^\alpha_{;lk}
=R^\alpha_{\beta lk}u^\beta
-T^p_{lk}u^\alpha_{;p}
\EqLabel{commutator second derivative}
\end{equation}
Из \EqRef{commutator second derivative} следует, что
\begin{equation}
\EqLabel{commutator second derivative of vector}
\xi^a_{;cb}-\xi^a_{;bc}
=R^a_{d bc}\xi^d
-T^p_{bc}\xi^a_{;p}
\end{equation}

В римановом пространстве мы имеем метрический тензор $g_{ij}$ и связность $\Gamma^k_{ij}$.
Одно из свойств риманова пространства - это симметрия связности и равенство нулю ковариантной производной
метрики. Это порождает тесную связь между метрикой и связностью.
Однако  связность не обязательно симметрична
и ковариантная производная метрического тензора может быть отлична от 0.
В последнем случае мы вводим \AddIndex{неметричность}{nonmetricity}
\begin{equation}
Q^{ij}_k=g^{ij}_{;k}=g^{ij}_{,k}+\Gamma^i_{pk}g^{pj}+\Gamma^j_{pk}g^{ip}
\EqLabel{Nonmetricity}
\end{equation}

Так как производная метрического тензора не равна 0, мы не можем поднимать или опускать индекс
тензора внутри производной как мы это делаем в обычном римановом пространстве.
Теперь эта операция принимает следующий вид
\[a^i_{;k} = g^{ij} a_{j;k} + g^{ij}_{;k} a_j\]
Это равенство для метрического тензора принимает следующий вид
\[g^{ab}_{;k} = - g^{ai} g^{bj} g_{ij;k}\]

\begin{definition}
\labelDefinition{metric-affine manifold}
Мы будем называть многообразие с кручением
и неметричностью
\AddIndex{метрико\Hyph аффинным многообразием}{metric-affine manifold} \citeBib{Mielke}.
\qed  
\end{definition}

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Неметричность значительно изменяет закон движения в пространстве
времени ортогонального базиса.
Однакко изучение параллельного переноса в пространстве с неметричностью
позволяет нам
ввести перенос Картана
и связность, совместимую с метрическим тензором
(раздел \RefSection[0405.028]{Cartan Transport}). Перенос Картана
сохраняет базис ортонормированным и это делает его важным инструментом,
так как наблюдатель использует ортонормированный базис как инструмент измерения.
Мы будем предполагать, что неметричность пространства
времени равна $0$.
\else

Если мы изучаем подмногообразие $V_n$ многообразия $V_{n+m}$, мы видим, что имерсия порождает
связность $\Gamma^\alpha_{\beta\gamma}$, которая связана со связностью в многообразии соотношением
\[
\Gamma^\alpha_{\beta\gamma} e^l_\alpha =
\Gamma^l_{mk} e^m_\beta e^k_\gamma + \frac {\partial e^l_\beta} {\partial u^\gamma}
\]
Следовательно, не существует непрерывного вложения
пространства с кручением в риманово пространство.
\fi
\fi

\section{Геометрический смысл кручения}

\ShowEq{note: sum of vectors 2}vw

\ShowEq{note: sum of vectors 3}

\ShowEq{note: sum of vectors 4}

\ShowEq{note: sum of vectors 5}

\ShowLemma{increase of coordinate along geodesic}
\ShowProof{increase of coordinate along geodesic}

\ShowTheorem{parallelogram is not closed}
\ShowProof{parallelogram is not closed}

\ePrints{GJSFRA.13.1.39,0803.3276}
\ifx\Semafor\ValueOff
\section{Соотношение между связностью и метрикой}

Сейчас мы хотим найти, как мы можем выразить связность, если известны
метрика и кручение. Согласно определению
\[-Q_{kij}=g_{ij;k}=g_{ij,k}-\Gamma^p_{ik}g_{pj}-\Gamma^p_{jk}g_{pi}\]
\[-Q_{kij}=g_{ij,k}-\Gamma^p_{ik}g_{pj}-\Gamma^p_{kj}g_{pi}-S^p_{jk}g_{pi}\]
Перенесём производную $g$ и кручение в левую часть.
\ShowEq{Connection1}
Меняя порядок индексов, мы запишем ещё два уравнения
\ShowEq{Connection2}
\ShowEq{Connection3}
Если мы вычтем равенство \EqRef{Connection1} из суммы равенств
\EqRef{Connection2} и \EqRef{Connection1}, то мы получим
\ShowEq{Connection4}
Окончательно мы получаем
\ShowEq{Connection5}
\fi


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%966%C%cr собственная строка
   {\CR собственная строка}%
   {cr eigenrow}%
\Index%964%C%cr собственное значение
   {\CR собственное значени}%
   {cr eigenvalue}%
\Index%947%C%cr собственный столбец
   {\CR собственный столбец}%
   {cr eigencolumn}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%965%R%rc собственная строка
   {\RC собственная строка}%
   {rc eigenrow}%
\Index%963%R%rc собственное значение
   {\RC собственное значение}%
   {rc eigenvalue}%
\Index%946%R%rc собственный столбец
   {\RC собственный столбец}%
   {rc eigencolumn}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%913%Б%базис абелевой группы
   {базис абелевой группы}%
   {basis of Abelian group}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate representation}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%701%К%квазибазис диаграммы представлений
   {квазибазис диаграммы представлений}%
   {quasibasis of diagram of representations}%
\Index%535%К%квазибазис представления
   {квазибазис представления}%
   {quasibasis of representation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация столбцов
   {левая линейная комбинация столбцов}%
   {left linear combination of columns}%
\Index%954%Л%левая линейная комбинация строк
   {левая линейная комбинация строк}%
   {left linear combination of rows}%
\Index%959%Л%левое A subs векторное пространство
   {левое $A_*$\Hyph векторное пространство}%
   {left A subs vector space}%
\Index%958%Л%левое A sups векторное пространство
   {левое $A^*$\Hyph векторное пространство}%
   {left A sups vector space}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное *G представление
   {пассивное \sT{G}представление}%
   {passive *G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%912%П%подмодуль, порождённым множеством
   {подмодуль, порождённым множеством}%
   {submodule generated by set}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация столбцов
   {правая линейная комбинация столбцов}%
   {right linear combination of columns}%
\Index%956%П%правая линейная комбинация строк
   {правая линейная комбинация строк}%
   {right linear combination of rows}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%960%П%правое A sups векторное пространство
   {правое $A^*$\Hyph векторное пространство}%
   {right A sups vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%384%П%принцип инвариантности
   {принцип инвариантности}%
   {invariance principle}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Newton.Russian.tex <==
%auto-ignore
\def\texNewton{}
\ifx\PrintBook\Defined
\chapter{Метрико-аффинная гравитация}
\fi

\section{Закон Ньютона: скалярный потенциал}
\labelSection{Newton Laws: Scalar Potential}

Знание динамики точечной частицы важно для нас,
так как мы можем изучать как частица взаимодействует с внешними полями,
так же как свойства самой частицы.

Чтобы изучить движение точечной частицы, мы можем использовать потенциал определённых полей.
Потенциал может быть скалярным или векторным.

В случае скалярного потенциала мы положим, что точечная частица
имеет массу покоя $m$ и мы пользуемся функцией Лагранжа в следующем виде
\[L = - m c ds - U dx^0\]о
где $U$ - \AddIndex{скалярный потенциал}{scalar potential}
или \AddIndex{потенциальная энергия}{potential energy}.

\begin{theorem}
\labelTheorem{First Newton law}
(\AddIndex{Первый закон Ньютона}{First Newton law})
Если $U = 0$ (следовательно, мы рассматриваем свободное движение),
то тело выбирает траекторию с экстремальной длиной.
\end{theorem}

\begin{theorem}
(\AddIndex{Второй закон Ньютона}{Second Newton law})
Траекторию точечной частицы удовлетворяет дифференциальному уравнению
\begin{equation}
\frac {\overbrace{D}u^l} {ds} =
\frac {u^0} {m c} F^l
\EqLabel{Newton}
\end{equation}
\[u^j = \frac {dx^l} {ds}\]
где мы определяем силу
\begin{equation}
F^l = g^{il} \frac{\partial U}{\partial x^i}
\EqLabel{potential force}
\end{equation}
\end{theorem}
\begin{proof}

Пользуясь \EqRef{Var Line Length},
мы можем записать вариацию лагранжиана в виде
$$\frac 1 2 m c \left(g_{kl;i} - g_{ik;l}
- g_{il;k}\right) u^k u^j ds
- m c g_{ij} Du^j
+ \frac {\partial U} {\partial x^i} dx^0 = 0$$
Отсюда следует утверждение теоремы.
\end{proof}

\section{Закон Ньютона: векторный потенциал}
В разделе \RefSection{Newton Laws: Scalar Potential}
мы изучили динамику скалярного потенциала.
Однако в электродинамике мы рассматриваем \AddIndex{векторный потенциал}
{vector potential} $A^k$.
В этом случае действие имеет вид
\[
S = \int^{t_2}_{t_1} \left( - m c ds - \frac e c A_l dx^l \right)
\]
\[
A_c = g_{cd} A^d
\]

\begin{theorem}
Траектория частицы, движущейся в векторном поле, удовлетворяет дифференциальному уравнению
\[
\frac {\overbrace{D}u^j} {ds} =
\frac e {m c^2} g^{ij} F_{li} u^l
\]
\[u^j = \frac {dx^l} {ds}\]
где мы определяем \AddIndex{тензор напряжённости поля}
{field-strength tensor}
\[F_{dc} = A_{d;c} - A_{c;d} + S^p_{dc} A_p
 = \overbrace{\nabla_c}A_d - \overbrace{\nabla_d}A_c + S^p_{dc} A_p\]
\end{theorem}
\begin{proof}

Пользуясь \EqRef{Var Line Length}, мы можем записать вариацию действия в виде
%\begin{widetext}
\[
\delta S =\]
\[=\int^{t_2}_{t_1} \left( - m c \left(
\frac 1 2 \left( g_{kj;i}
- g_{ij;k} - g_{ik;j} \right) u^k u^j ds
- g_{ij} D u^j\right) \delta x^i
- \frac e c \left(\delta A_l dx^l + A_l \delta dx^l \right)
\right)
\]
%\end{widetext}
Мы можем оценить второе слагаемое
\[
- \frac e c \left(A_{l,k} dx^l \delta x^k + A_l d\delta x^l \right) =
\]
\[
=- \frac e c \left(A_{l;k} dx^l \delta x^k
+ \Gamma^p_{lk} A_p dx^l \delta x^k
+ A_l d\delta x^l \right) =
\]
%\begin{widetext}
\[
=- \frac e c \left(A_{k;l} dx^l \delta x^k +
\left(A_{l;k} - A_{k;l}\right)dx^l \delta x^k+
S^p_{lk} A_p dx^l \delta x^k + \Gamma^p_{kl} A_p dx^l \delta x^k
+ A_l d\delta x^l \right) =
\]
\[
=- \frac e c \left(DA_k \delta x^k + A_k D\delta x^k +
\left(A_{l;k} - A_{k;l}\right)dx^l \delta x^k
+ S^p_{lk} A_p dx^l \delta x^k \right) =
\]
%\end{widetext}
\[
=- \frac e c \left(\underline{d\left(A_k \delta x^k\right)} +
\left( A_{l;k} - A_{k;l}
+ S^p_{lk} A_p \right) dx^l \delta x^k\right)
\]
Интеграл подчёркнутого слагаемого равен $0$,
так как точки, когда $t = t_1$ и $t = t_2$, фиксированы.
Следовательно,
\[
- m c \left(
\frac 1 2 \left( g_{kj;i}
- g_{ij;k} - g_{ik;j} \right) u^k u^j ds
- g_{ij} D u^j\right)-
\frac e c F_{li} dx^l = 0
\]
Отсюда следует утверждение теоремы.
\end{proof}

Из этой теоремы следует
зависимость тензора напряжённости поля от производной метрики.
Это изменяет форму уравнения Эйнштейна и импульс гравитацинного поля
появляется в случае векторного поля.

\begin{theorem}
Тензор напряжённости поля не изменяется, когда векторный потенциал изменяется
согласно правилу
\[A'_j=A_j+\partial_j\Lambda\]
где $\Lambda$ - произвольная функция $x$.
\end{theorem}
\begin{proof}
Изменение в тензоре напряжённости поля имеет вид
\[(\partial_d\Lambda){}_{;c} - (\partial_c\Lambda){}_{;d} + S^p_{dc} \partial_p\Lambda =\]
\[\partial_{cd}\Lambda - \Gamma^p_{dc} \partial_p\Lambda
- \partial_{dc}\Lambda+\Gamma^p_{cd} \partial_p\Lambda + S^p_{dc}\partial_p\Lambda =0\]
Это доказывает теорему.
\end{proof}





==> Preface.0803.3276.English.tex <==
%auto-ignore

\ePrints{0803.3276,4827-2437}
\ifx\Semafor\ValueOn
\chapter{Introduction}
\section{About This Book}
\labelSection{About This Book}

Since Einstein introduced general relativity,
the close relation between geometry
and physics became a reality
(\citeBib{Einstein: Geometry and Experience}).
At the same time,
quantum mechanics introduced new concepts that
contradicted a tradition established during centuries.
This meant that we need new geometric concepts that will become part
of the language of quantum mechanics.

When I learned
general relativity and quantum mechanics I felt that language of
quantum mechanics is not adequate to phenomenon that it observes.
I mean the geometry.
This book starts from learning of geometric object, turns to
reference frame in physics, then suddenly changes its course
to learn metric affine manifolds.

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
I dedicated chapter \RefChapter{Space and Time in Physics}
to small essay that I wrote when I was young.\,\footnote{
Unfortunately some references are lost. If somebody recognize
\label{footnote: Space and Time in Physics}
familiar text, I will appreciate if he let me know exactly reference.}
In this essay I tried to analyze nature of definitions of space and time.
\fi
\fi

\ePrints{0405.027,0803.3276,GJSFRA.13.1.39,4827-2437}
\ifx\Semafor\ValueOn
\section{Geometric Object and Invariance Principle}

\ePrints{0803.3276,4827-2437}
\ifx\Semafor\ValueOn
Sections \RefSection{Basis in Vector Space}
and \RefSection{Geometric Object of Vector Space}
was written under the great influence of the book \citeBib{Rashevsky}.
The studying of a homogenous space of a group of symmetry of a vector space
leads us to the definition of a basis of this space. A basis  manifold is a set of
bases of particular vector space and is an example of a homogenous space.
As it is shown in \citeBib{Rashevsky} it gives ability to define
concepts of invariance and of geometric object.

We introduce two types of transformation of a basis manifold:
active and passive transformations. The difference between them is
that the passive transformation can be expressed as a transformation of
an original space.

This definition can be extended on an arbitrary manifold. However in
this case we generalize the definition of a basis and introduce a reference
frame. In case of an event space of general relativity it leads us to
a natural definition of a reference frame and the Lorentz transformation.
A reference frame in event space is a smooth field of orthonormal basis.
\fi

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
The invariance principle considered in the
theorem \xRef[0412.391]{theorem: invariance principle}
is limited by vector spaces and we can use it only
in frame of the special relativity. Our task is
to describe structures which allow to extend
the invariance principle to general relativity.
\fi

A measurement of a spatial interval and a time length
is one of the major tasks of general relativity.
This is a physical process that allows the study
of geometry in a certain area of spacetime.
From a geometric point of view,
the observer uses an orthonormal basis in a tangent plane as his measurement tool
because an orthonormal basis leads to the simplest local geometry.
When the observer moves from point to point he brings
his measurement tool with him.

Notion of a geometric object is closely related with
physical values measured in space time.
The invariance principle allows expressing physical laws
independently from the selection of a basis.
On the other hand if we want
to examine a relationship obtained in the test, we need to select
measurement tool. In our case this is basis. Choosing
the basis we can define coordinates of the geometric object
corresponding to studied physical value.
Hence we can define the measured value.

Every reference frame is equipped by anholonomic coordinates.
\ePrints{4827-2437}
\ifx\Semafor\ValueOn
In the paper
\citeBib{GJSFRA.13.1.39},
I discussed importance of anholonomic coordinates in physics calculations.
\else
For instance, synchronization of a reference frame is an anholonomic time coordinate.
Simple calculations show how synchronization influences time measurement in
the vicinity of the Earth.
Measurement of Doppler shift from the star orbiting the black hole helps
to determine mass of the black hole.

The section
\RefSection{Lorentz Transformation in Orbital Direction}
shows importance of calculations in orthogonal
basis. Coordinates that we use in event space
are just labels
and calculations that we make in coordinates may appear
not reliable. For instance in papers \citeBib{Tartaglia,Tomozawa}
authors determine coordinate speed of light. This leads to
not reliable answer and as consequence of this to
the difference of speed of light in different directions.
\fi
\fi

\ePrints{0405.027,0407.092,0803.3276,GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Paper \citeBib{Ranada} drew my attention. To explain anomalous acceleration of Pioneer 10
and Pioneer 11 (\citeBib{Anderson02}) Antonio Ranada incorporated the old Einstein's view on nature of
gravitational field and considered Einstein's idea about variability of speed of light.
When Einstein started to study the gravitational field he tried to
keep the Minkowski geometry, therefore he assumed that scale of
space and time does not change. As result he had to accept the idea that speed of light should
vary in gravitational field. When Grossman introduced Riemann geometry to Einstein, Einstein
realized that the initial idea was wrong and Riemann geometry solves his problem better.
Einstein never returned to idea about variable speed of
light.

Indeed, three values: scale of length and time and speed of light are correlated in present
theory and we cannot change one without changing another.
The presence of gravitational field changes this relation. We have two choices. We keep
a priory given geometry (here, Minkowski geometry) and we accept that the speed of light
changes from point to point. The Riemann geometry gives us another option. Geometry becomes
the result of observation and the measurement tool may change from point to point. In this case
we can keep the speed of light constant. Geometry becomes a background which depends on
physical processes. Physical laws become background independent.
\fi

\ePrints{0405.027,0803.3276}
\ifx\Semafor\ValueOn
There are few papers dedicated to a variable speed of light theory
\citeBib{Magueijo,Bassett}. Their theory is based on idea that metric tensor
may be invariant with respect to dilatation. This idea is not new.
As soon as Einstein published general relativity
Weil introduced his idea to make theory invariant relative
conformal transformation. However Einstein was firmly opposed to
this idea because it broke dependence between distance
and proper time. You can find detailed analysis in \citeBib{Straumann}.

We have strong relation between the speed of light
and units of length and time in special and general relativity.
When we develop new theory and discover that speed of light is different
we should ask ourselves about the reason. Did we make accurate measurement?
Do we have alternative way to exchange information and synchronize reference
frame? Did transformations between reference frames change
and do they create group?

In some models photon may have small rest mass \citeBib{Lammerzahl}.
In this case speed of light is different from maximal speed and may
depend on direction. Recent experiment \citeBib{0305117}
put limitation on parameters of these models.
\fi

\ePrints{0405.028,0803.3276,GJSFRA.13.1.39,4827-2437}
\ifx\Semafor\ValueOn
\ePrints{4827-2437}
\ifx\Semafor\ValueOff
\section{Torsion Tensor in General Relativity}

Close relationship between the metric tensor and the connection is
the basis of the Riemann geometry.
At the same time, connection and metric as any geometric object are objects of measurement.
When Hilbert derived Einstein equation, he introduced the lagrangian where
the metric tensor and the connection are independent.
Later on, Hilbert discovered that the connection
is symmetric and found dependence between connection and metric tensor. One of the
reasons is in the simplicity of the lagrangian.

%\ifx\PrintBook\Defined
%Formally chapter \RefChapter{General Relativistic Field Equations}
%is the last chapter in the book. However from historyc aproach
%it reflects research which was the starting point of certain period of my life.
%Straight join of two lagrangians
%(of gravitational and quantum fields)
%is the heart of equations developed in this chapter.
%Equations
%\EqRef{Field}, \EqRef{Einstein},
%\EqRef{Cartan} and
%\EqRef{Maxwell} have complicated form.
%They are nonlinear over connection.
%However any attempt to solve these equations lead to case that
%this system breaks apart Einstein equation and field equation
%which are independent.
%It is possible that reason of the failure was inside of the method used to solve the problem.
%Recent developement of physics proved that join of
%general relativity and quantum mechanics demands more powerful methods.
%String theory and loop gravity
%represent main direction developed today.

%However inspite of failure analysis of these equations is very important.
%\fi

Since an errors of measurement are inescapable,
analysis of quantum field theory shows that either
symmetry of connection or dependence between connection and metric may be broken. 
This assumption leads to metric\hyph affine manifold
which is space with torsion and nonzero covariant derivative
of metric (section \RefSection{Metric-affine Manifold}).
\fi
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
\ePrints{4827-2437}
\ifx\Semafor\ValueOn

\section{Free Movement in Metric-Affine Manifold}
\fi
Independence of the metric tensor and the connection allows us to see
which object is responsible for different
phenomenon in geometry and therefore in physics.
Even we do not prove empirically existence of torsion and nonmetricity
we see here very interesting geometry.

The metric\hyph affine manifold appears in different physical applications.
It is very important to understand what kind of geometry of this space is,
how torsion influences on physical phenomena.
This is why small group of physicists continue to study gravitation
theory with torsion
\citeBib{Mielke,Obukhov,Sardanashvily,Gauge,Neeman}.

In particular we have two different definitions
of a geodesic curve in the Riemann manifold.
We consider a geodesic curve either as line of extreme length
(such line is called extreme),
or as line such that tangent vector
keep to be tangent to line during parallel transfer
(such line is called auto parallel).
Nonmetricity means that parallel transport
does not conserve a length of vector and an angle between
vectors. This leads to a difference between
definitions of auto parallel and extreme lines (\citeBib{torsion} and
section \RefSection{Line with extreme length})
and to a change in the expression of the Frenet transport.
The change of geometry influences the second Newton law which we study
in section \RefSection{Newton Laws: Scalar Potential}.
I show in theorems \RefTheorem{LengthTangentVector}
and \RefTheorem{First Newton law} 
that a free falling particle chooses an extreme line transporting
its momentum along the trajectory without change.

Pattern of the Newton second law depends on choice of potential.
In case of scalar potential
the Newton second law holds the relationship between force, mass and acceleration.
In case of vector potential
analysis of motion in a gravitational field shows that the field-strength tensor
depends on the derivative of the metric tensor.

Nonmetricity dramatically changes law
how orthogonal basis moves in space time.
However learning of parallel transport in space with nonmetricity
allows us to
introduce the Cartan transport
and the connection compatible with the metric tensor
(section \RefSection{Cartan Transport}). The Cartan transport
holds the basis orthonormal and this makes it valuable tool
in dynamics (section \RefSection{Newton Laws: Scalar Potential})
because the observer uses an orthonormal basis as his measurement tool.
The dynamics of a particle follows to the Cartan transport.
The question arises from this conclusion.

We can change the connection as we show in section \RefSection{Cartan Transport}.
%or we can change the metric tensor as is shown
%in  such way that the parallel transport conserves
%the metric tensor\,\footnote{I am not agree with conclussion in paper \citeBib{Hehl},
%however this paper shows way how to find the metric tensor compatible with connection}.
Why we need to learn manifolds with an arbitrary connection and the metric tensor?
The learning of the metric\hyph affine manifold shows why everything
works well in the Riemann manifold and what changes in a general case.
What kind of different physical phenomena
may result in different connections?
Physical constraints that appear in a model may lead to appearance of a nonmetricity
\citeBib{Gauge,Megged,gr-qc-9604027}.
Because the Cartan transport is the natural mechanism to conserve orthogonality,
we expect that we will interpret a deviation
of the test particle from the extreme line as
a result of an external to this particle
force\,\footnote{For instance if we extend the definition \EqRef{potential force} of a force
to a general case \EqRef{Newton} we can interpret a deviation of a charged particle
in electromagnetic field as result of the force
\[\ F^j=\frac e {cu^0} g^{ij} F_{li} u^l\]
The same way we can interpret a deviation of the auto parallel line as the force
\[F^i=-\frac {m c} {u^0} \Gamma(C)^i_{kl}u^ku^l\]
I remind that the Cartan symbol is the tensor}.
In this case the difference between two types of a transport
becomes measurable and meaningful. Otherwise another type
of a transport and nonmetricity are not observable and we can use
only the transport compatible with metric.

I see here one more opportunity. As follows from the paper \citeBib{Megged}
the torsion may depend on quantum properties of matter.
However the torsion is the part of the connection. This means that the connection may
also depend on quantum properties of matter. This may lead to breaking of
the Cartan transport. However this opportunity demands additional research.

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
The effects of torsion and a nonmetricity are cumulative.
\fi
\else

The effects of torsion are cumulative.
\fi
\ePrints{4827-2437}
\ifx\Semafor\ValueOff
They may be small but measurable. We can observe their effects not only in strong
fields like black hole or Big Bang but in regular conditions
as well.
Studying geometry and dynamics of point particle gives us a way to test this point of view.
There is mind to test this theory in condition when spin of quantum field is accumulated.
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
We can test a deviation from second Newton law or measure torsion by observing
the movement of two different particles.
\fi

To test if the spacetime has the torsion we
can test the opportunity to build a parallelogram in spacetime. 
We can get two particles or two photons
that start their movement from the same point
and using a mirror to force them
to move along opposite sides of the parallelogram.
We can start this test when we do not have quantum field and then repeat
the test in the presence of quantum field.
If particles meet in the same place
or we have the same interference then we have
torsion equal $0$ in this thread.
In particular, the torsion may influence the behavior of virtual particles.

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
To check if space time has nonmetricity, we
can measure the deviation of extreme line
from auto parallel line or
deviation of unit vector of speed from its parallel transport.
\fi
\fi
\fi

%\ifx\PrintBook\Defined
%\section{Symmetry}

%The torsion leads to a change in the Killing equation. We also need to add a similar equation
%for the connection.

%Asymmetry of connection arises not only from torsion. Theory of
%geometric object in vector space has natural
%generalization: the theory of reference frame in event space. Reference frame
%is powerful tool of measurement in general relativity.
%\fi

\ePrints{0407.092,0803.3276,GJSFRA.13.1.39}
\ifx\Semafor\ValueOn

\section{Tidal Acceleration}

Observations in Solar system and outside are very important. They give us an opportunity
to see where general relativity is right and to find out its limitation.
It is very important to be very careful with such observations.
NASA provided very interesting observation of Pioneer 10 and Pioneer 11
and managed complicated calculation of their accelerations. However, one interesting
question arises:
what kind of acceleration did we measure?

Pioneer 10 and Pioneer 11 performed free movement in solar system.
Therefore they move along their trajectory without acceleration.
However, it is well known that two bodies moving along close geodesics have relative
acceleration that we call tidal acceleration. Tidal acceleration in general relativity has form
\begin{equation}
\EqLabel{Tidal acceleration}
\frac{D^2\delta x^k}{ds^2}
=R^k_{lnk}\delta x^kv^nv^l
\end{equation}
where $v^l$ is the speed of body $1$ and $\delta x^k$ is the deviation of geodesic of body $2$
from geodesic of body $1$. We see from this expression that tidal acceleration
depends on movement of body $1$ and how the trajectory of body $2$ deviates from the trajectory of body $1$.
But this means that even for two bodies that are at the same distance from a central body we can measure
different acceleration relative an observer.

Section \RefSection{Tidal Equation} is dedicated to the problem
what kind of changes the tidal force experiences on
metric affine manifolds.

Finally the question arises. Can we use equation \EqRef{deviation_extreme}
to measure torsion? We get tidal acceleration from direct measurement. There is
a method to measure curvature (see for instance \citeBib{Wheeler}). However, even
if we know the acceleration and curvature we still have differential equation
to find torsion. However, this way may give direct answer to the question
of whether torsion exists or not.

Deviation from tidal acceleration \EqRef{Tidal acceleration}
predicted by general relativity may have different reason.
However we can find answer by combining different type of measurement.
\fi


==> Preface.0803.3276.Russian.tex <==
%auto-ignore

\ePrints{0803.3276,4827-2437}
\ifx\Semafor\ValueOn
\chapter{Введение}
\section{Об этой книге}
\labelSection{About This Book}

С тех пор, как Эйнштейн создал общую теорию относительности,
тесная связь между геометрией
и физикой стала реальностью
(\citeBib{Einstein: Geometry and Experience}).
В тоже время квантовая механика вводит новые концепции, которые
противоречат традиции, установленной на протяжении столетий.
Это означает, что нам нужны новые геометрические концепции, которые станут частью
языка квантовой механики.

Когда я познакомился с
общей теорией относительности и квантовой механикой, я почувствовал, что язык
квантовой механики не адекватен явлениям, которые она наблюдает.
Я имею в виду геометрию.
Эта книга начинается с изучения геометрического объекта, переходит к
системе отсчёта в физике, затем внезапно меняет направление
к изучению метрико\hyph аффинного многообразия.

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
Я посвятил главу \RefChapter{Space and Time in Physics}
небольшому сочинению, написанному мной, когда я был молод.\,\footnote{
К сожалению, некоторые ссылки потеряны. Я буду признателен, если кто-то узнает
\label{footnote: Space and Time in Physics}
знакомый текст и даст мне знать точную ссылку.}
В этом сочинении я пытался проанализировать природу определений пространства и времени.
\fi
\fi

\ePrints{0405.027,0803.3276,GJSFRA.13.1.39,4827-2437}
\ifx\Semafor\ValueOn
\section{Геометрический объект и принцип инвариантности}

\ePrints{0803.3276,4827-2437}
\ifx\Semafor\ValueOn
Разделы \RefSection{Basis in Vector Space}
и \RefSection{Geometric Object of Vector Space}
были написаны под большим влиянием книги \citeBib{Rashevsky}.
Изучение однородного пространства группы симметрии векторного пространства
ведёт нас к определению базиса этого пространства. Многообразие базисов - это множество
базисов изучаемого векторного пространства и является примером однородного пространства.
Как показано в \citeBib{Rashevsky}, это даёт возможность определить
концепцию инвариантности и геометрического объекта.

Мы определяем два типа преобразований многообразия базисов:
активные и пассивные преобразования. Различие между ними состоит в том,
что пассивное преобразование может быть выражено как преобразование
исходного пространства.

Это определение может быть распространено на произвольное многообразие. Однако в
этом случае мы обобщаем определение базиса и вводим систему
отсчёта. В случае пространства событий общей теорией относительности это приводит нас к
естественному определению системы отсчёта и преобразованию Лоренца.
Система отсчёта в пространтве событий - это непрерывное поле ортонормированных базисов.
\fi

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
Принцип инвариантности, рассмотренный в
теореме \xRef[0412.391]{theorem: invariance principle}
ограничен векторными пространствами и применим только
в рамках специальной теории относительности. Наша задача
описать конструкции, которые позволяют распространить
принцип инвариантности на общую теорию относительности.
\fi

Измерение пространственного интервала и временных отрезков
является одной из важных задач общей теории относительности.
Это физический процесс, который позволяет изучать
геометрию в определённой области пространства\Hyph времени.
С точки зрения геометрии, наблюдатель пользуется ортогональным базисом в касательной
плоскости как своим измерительным инструментом,
так как ортогональный базис приводит к простейшей локальной геометрии.
Двигаясь от точки к точке, наблюдатель переносит с собой
свой измерительный прибор.

Понятие геометрического объекта тесно связано с
физическими величинами, измеряемыми в пространстве\Hyph времени.
Принцип инвариантности позволяет выразить физические законы
независимо от выбора базиса. С другой стороны, если мы хотим
проверить полученное соотношение в опыте, мы должны зафиксировать
измерительный прибор. В нашем случае - это базис. Выбрав
базис, мы можем определить координаты геометрического
объекта, соответствующего изучаемой физической величине.
Следовательно мы можем определить измеряемое значение.

Каждая система отсчёта снабжена неголономными координатами.
\ePrints{4827-2437}
\ifx\Semafor\ValueOn
Роль неголономных координат в физических расчётах
рассмотрена в статье
\citeBib{GJSFRA.13.1.39}.
\else
Например, синхронизация системы отсчёта - это неголономная координата времени.
Простые расчёты показывают как синхронизация влияет на измерение времени в
окрестности Земли.
Измерение эффекта Допплера от звезды, вращающейся вокруг чёрной дыры, помогает
определить массу чёрной дыры.

Раздел
\RefSection{Lorentz Transformation in Orbital Direction}
показывает важность расчётов в ортогональном
базисе. Координаты, которыми мы пользуемся в пространстве событий,
- это просто метки
и расчёты, которые мы выполняем в координатах могут оказаться
не надёжными. Например, в статьях \citeBib{Tartaglia,Tomozawa}
авторы определяют координатную скорость света. Это ведёт к
неверному ответу и в результате этого к
различию скорости света в разных направлениях.
\fi
\fi

\ePrints{0405.027,0407.092,0803.3276,GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Моё внимание привлекла статья \citeBib{Ranada}. Чтобы объяснить аномальное ускорение Pioneer 10
и Pioneer 11 (\citeBib{Anderson02}), Антонио Ранада привлекает старую точку зрения Эйнштейна
о природе гравитационного поля и используют идею Эйнштейна о переменной скорости света.
Когда Эйнштейн начал изучать гравитационное поле, он старался
сохранить геометрию Минковского и, следовательно, предполагал, что масштаб
пространства и времени не меняются. В результате он был вынужден принять гипотезу, что скорость света может
меняться в гравитационном поле. Когда Гроссман познакомил Эйнштейна с римановой геометрией, Эйнштейн
понял, что начальная гипотеза была ошибочна и риманова геометрия лучше решит его задачу.
Эйнштейн никогда
не возвращался к идее о переменной скорости
света.

Действительно, три значения: масштаб пространства и времени и скорость света являются связанными в современной
теории и мы не можем изменить одну величину без изменения другой.
Присутствие гравитационного поля меняет это соотношение. Мы имеем два выбора. Мы сохраняем
исходно заданную геометрию (здесь, геометрию Минковского) и мы согласны, что скорость света
меняется от точки к точке. Риманова геометрия предлагает нам другой выбор. Геометрия становится
результатом измерения и измерительный инструмент может меняться от точки к точке. В этом случае
мы можем сохранить скорость света постоянной. Геометрия становится фоном, который зависит от
физических процессов. Физические законы становятся независимыми от фона.
\fi

\ePrints{0405.027,0803.3276}
\ifx\Semafor\ValueOn
Некоторые статьи посвящены теории переменной скорости света
\citeBib{Magueijo,Bassett}. Их теория основана на идее, что метрический тензор
может быть инвариантен относительно преобразования подобия. Эта идея не нова.
Как только Эйнштейн опубликовал общую теории относительности,
Вейль предложил свою идею сделать теорию инвариантной относительно
конформного преобразования. Тем не менее, Эйнштейн возражал
этой идее, так как она разрушала зависимость между расстоянием
и собственным временем. Мы можем найти детальный анализ в \citeBib{Straumann}.

Мы имеем тесную связь между скоростью света
и единицами длины и времени в специальной и общей теории относительности.
Когда мы развиваем новую теорию и обнаруживаем, что скорость света меняется,
мы должны спросить себя о причине. Сделали ли мы аккуратное измерение?
Имеем ли мы альтернативный путь для обмена информацией и синхронизации
системы отсчёта? Меняются ли преобразования между системами отсчёта
и образуют ли они группу?

В некоторых моделях фотон может иметь небольшую массу покоя \citeBib{Lammerzahl}.
В этом случае скорость света отлична от максимальной скорости и может
зависеть от направления. Недавний эксперимент \citeBib{0305117}
наложил ограничения на параметры этих моделей.
\fi

\ePrints{0405.028,0803.3276,GJSFRA.13.1.39,4827-2437}
\ifx\Semafor\ValueOn
\ePrints{4827-2437}
\ifx\Semafor\ValueOff
\section{Тензор кручения в общей теории относительности}

Тесная связь между метрическим тензором и связностью является
основой римановой геометрии.
В то же время, связность и метрика, как любой геометрический объект, являются объектом измерения.
Когда Гильберт выводил уравнение Эйнштейна, он определил лагранжиан, в котором
метрический тензор и связность независимы.
Позже Гильберт обнаружил, что связность
симметрична, и нашёл зависимость между связностью и метрическим тензором. Одна из причин
этого - простота лагранжиана.

%\ifx\PrintBook\Defined
%Глава \RefChapter{General Relativistic Field Equations}
%формально завершает книгу, хотя исторически она отображает
%исследование, с которого начался определённый этап моей жизни.
%В основу уравнений, выведенных в этой главе, было положено
%непосредственное объединение двух лагранжианов: гравитационного
%и квантового полей.
%Уравнения
%\EqRef{Field}, \EqRef{Einstein},
%\EqRef{Cartan} и
%\EqRef{Maxwell} имеют очень сложный вид.
%Они нелинейны по связности.
%Но любая попытка решить систему этих уравнений приводит к тому,
%что эта системв распадается на уравнение Эйнштейна и
%уравнение поля, которые независимы.
%Повидимому неудача изначально заложена в самом подходе к проблеме.
%Последующее развитие физики показало, что объединение общей теории
%относительности и квантовой механики требует более мощных методов.
%Основные направления на сегодняшний день можно разделить на теорию
%струн и петлевую теорию гравитации.

%Однако несмотря на неудачу, анализ полученных уравнений очень важен.
%\fi

Анализ квантовой теории поля показывает,что либо
симметрия связности, либо зависимость связности и метрики могут быть нарушены, 
поскольку неизбежны ошибки измерения.
Это допущение приводит к метрико\hyph аффинному многообразию,
которое является пространством с кручением и ненулевой ковариантной производной
метрического тензора (раздел \RefSection{Metric-affine Manifold}).
\fi
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
\ePrints{4827-2437}
\ifx\Semafor\ValueOn

\section{Свободное движение в метрико аффинном многообразии}
\fi
Независимость метрического тензора и связности позволяет нам видеть, какие
объекты ответственны за различные
явления в геометрии и, следовательно, в физике.
Даже несмотря на то, что мы не доказали эмпирически
существование кручения и неметричности, мы видим здесь очень интересную геометрию.

Метрико\hyph аффинное многообразие появляется в разных физических приложениях.
Очень важно понять какова геометрия этого пространства,
как кручение может влиять на физические процессы.
Именно поэтому небольшая группа физиков продолжает изучать теорию
гравитации с кручением
\citeBib{Mielke,Obukhov,Sardanashvily,Gauge,Neeman}.

В частности, мы имеем два различных определения
геодезической в римановом многообразие.
Мы можем рассматривать геодезическую либо как кривую экстремальной длины
(соответствующую кривую мы называем экстремальной),
либо как кривую, вдоль которой касательный вектор
переносится параллельно, оставаясь касательным к кривой
(соответствующую кривую мы называем автопараллельной).
Неметричность приводит к тому, что параллельный
перенос не сохраняет длину вектора и угол между
векторами. Это приводит к различию между
определениями автопараллельной и экстремальной кривых (\citeBib{torsion} и
раздел \RefSection{Line with extreme length})
и к изменению в выражении переноса Френе.
Изменение геометрии влияет на второй закон Ньютона, который
мы изучаем в разделе \RefSection{Newton Laws: Scalar Potential}.
Я показываю в теоремах \RefTheorem{LengthTangentVector}
и \RefTheorem{First Newton law},
что свободно падающая частица предпочитает экстремальную кривую, перенося
свой импульс вдоль траектории без изменения.

Форма второго закона Ньютона зависит от выбора формы потенциала.
В случае скалярного потенциала
второй закон Ньютона сохраняет соотношение между силой, массой и ускорением.
В случае векторного потенциала
анализ движения в гравитационном поле показывает, что тензор напряжённости поля
зависит от производной метрического тензора.

Неметричность значительно изменяет закон движения в пространстве
времени ортогонального базиса.
Однако изучение параллельного переноса в пространстве с неметричностью
позволяет нам
ввести перенос Картана
и связность, совместимую с метрическим тензором
(раздел \RefSection{Cartan Transport}). Перенос Картана
сохраняет базис ортонормированным и это делает его важным инструментом
в динамике (раздел \RefSection{Newton Laws: Scalar Potential}),
так как наблюдатель использует ортонормированный базис как инструмент измерения.
Динамика частицы основана на переносе Картана.
Тогда появляется вопрос.

Мы можем изменить связность как мы показали в разделе \RefSection{Cartan Transport}.
%or мы can change the metric tensor as is shown
%in  such way that the parallel transport conserves
%the metric tensor\,\footnote{I am not agree with conclussion in paper \citeBib{Hehl},
%however this paper shows way how to find the metric tensor compatible with connection}.
Почему мы должны изучать многообразия с произвольной связностью и метрическим тензором?
Изучение метрико\hyph аффинного многообразия показывает, почему всё
работает хорошо в римановом многообразии и что меняется в общем случае.
К какого рода различные физические явления
являются следствием различных связностей?
Физические ограничения, которые появляются в модели, могут вести к появлению неметричности
\citeBib{Gauge,Megged,gr-qc-9604027}.
Так как перенос Картана - естественный механизм сохранения ортогональности,
мы ожидаем, что мы будем интерпретировать отклонение
пробной частицы от экстремальной кривой как
результат силы, внешней по отношению к этой частице\,\footnote{Например,
если мы распространим определение \EqRef{potential force} силы
на общий случай \EqRef{Newton}, мы можем интерпретировать отклонение заряжённой
частицы в электромагнитном поле как результат силы
\[\ F^j=\frac e {cu^0} g^{ij} F_{li} u^l\]
Аналогично, мы можем интерпретировать отклонение автопараллельной кривой как силу
\[F^i=-\frac {m c} {u^0} \Gamma(C)^i_{kl}u^ku^l\]
Я напоминаю, что символ Картана - тензор}.
В этом случае различие между двумя типами переноса
становится измеримым и осмысленным. В противном случае другой тип
переноса и неметричность не наблюдаемы и мы можем пользоваться
только переносом, совместимым с метрикой.

Я вижу ещё одну возможность. Как следует из статьи \citeBib{Megged},
кручение может зависеть от квантовых свойств материи.
Тем не менее, кручение является частью связности. Следовательно, связность может
также зависеть от квантовых свойств материи. Это может привести к нарушению
переноса Картана. Однако эта возможность требует дополнительного исследования.

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
Кручение и неметричность имеют интегральные эффекты.
\fi
\else

Кручение имеет интегральные эффекты.
\fi
\ePrints{4827-2437}
\ifx\Semafor\ValueOff
Они могут быть малыми, но измеримыми. Мы можем наблюдать эти эффекты не только в сильных
полях, подобных чёрной дыре или большому взрыву, но также в обычных условиях.
Изучение геометрии и линамики точечной частицы даёт нам возможность
проверить эту точку зрения.
Есть смысл проверить эту теорию в условиях, когда спин квантового поля накоплен.
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
Мы можем проверить отклонение от второго закона Ньютона либо измерить кручение,
наблюдая движение двух различных частиц.
\fi

Чтобы проверить, имеет ли пространство\Hyph время кручение, мы
можем проверить возможность построить параллелограмм в пространстве\Hyph времени. 
Мы можем взять две частицы или два фотона,
которые начинают своё движение из одной и той же точки
и, пользуясь зеркалом, заставить их двигаться вдоль противоположных
сторон параллелограмма.
Мы можем начать этот эксперимент, когда квантового поля нет, и затем повторить
эксперимент в присутствии квантового поля.
Если частицы встретятся в одном и том же месте или мы имеем одинаковую
интерференцию, то мы имеем
кручение равное $0$ в этой среде.
В частности, кручение может действовать на поведение виртуальных частиц.

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
Чтобы проверить, имеет ли пространство\Hyph время неметричность, мы
можем измерить отклонение экстремальной кривой
от автопараллельной либо
отклонение единичного вектора скорости от его параллельного переноса.
\fi
\fi
\fi

%\ifx\PrintBook\Defined
%\section{Симметрия}

%The torsion leads to a change in the Killing equation. Мы also need to add a similar equation
%for the connection.

%Ассиметрия связности возникает не только за счёт кручения. Изучение теории
%геометрического объекта в векторном пространстве приводит к её естественному
%обобщению: теории системы отсчёта в пространстве событий. Система отсчёта
%является мощнейшим измерительным инструментом в общей теории относительности.
%\fi

\ePrints{0407.092,0803.3276,GJSFRA.13.1.39}
\ifx\Semafor\ValueOn

\section{Приливное ускорение}

Наблюдения в Солнечной системе и вне очень важны. Они дают нам возможность
видеть, где общая теория относительности права и найти её ограничения.
Очень важно быть осторожным с такими наблюдениями.
NASA выполнило очень интересные наблюдения Pioneer 10 и Pioneer 11
и выполнило сложные расчёты их ускорения. Однако, возникает один интересный
вопрос: какого типа ускорения мы меряли?

Pioneer 10 и Pioneer 11 совершают свободное движение в солнечной системе.
Следовательно, они движутся вдоль своей траектории без ускорения.
Однако, хорошо известно, что два тела, двигаясь вдоль близких геодезических, имеют относительное
ускорение, которое называется приливным ускорением. Приливное ускорение
в общей теории относительности имеет вид
\begin{equation}
\EqLabel{Tidal acceleration}
\frac{D^2\delta x^k}{ds^2}
=R^k_{lnk}\delta x^kv^nv^l
\end{equation}
где $v^l$ - скорость тела $1$ и $\delta x^k$ - отклонение геодезической тела $2$
от геодезической тела $1$. Мы видим из этого выражения, что приливное ускорение
зависит от движения тела $1$ и как траектория тела $2$ отклоняется от траектории тела $1$.
Но это значит, что даже для двух тел, которые находятся на одном и том же
расстоянии от центрального тела, мы можем измерить
разное ускорение относительно наблюдателя.

Раздел \RefSection{Tidal Equation} посвящён решению задачи,
какие изменения испытывает приливная сила на метрико\hyph аффинном многообразии.

Возникает вопрос: можем ли мы использовать уравнение \EqRef{deviation_extreme},
чтобы измерить кручение? Мы получим приливное ускорение из прямых измерений. Существует
метод измерять кривизну (см. например \citeBib{Wheeler}). Однако, даже
если мы знаем ускорение и кривизну, мы по\Hyph прежнему имеем дифференциальное уравнение,
чтобы найти кручение. Однако, этот путь может дать прямой ответ на вопрос
существует ли кручение.

Отклонение от приливного ускорения \EqRef{Tidal acceleration},
предсказанного общей теорией относительности может иметь различные причины.
Однако мы можем найти ответ, комбинируя разные методы измерения.
\fi


==> Refernce.Frame.Russian.tex <==
%auto-ignore
\input{Refernce.Frame.Eq}
\ifx\PrintBook\Defined
\chapter{Система отсчёта в пространстве событий}
\fi

\section{Система отсчёта на многообразии}
\labelSection{Reference Frame on Manifold}

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
Мы показали в разделе
\xRef[0412.391]{section: Basis in Vector Space},
что многообразие базисов векторного пространства можно отождествить
с группой симметрий этого пространства.
Нас не интересовали детали строения репера,
и изложенная теория может быть обобщена
и перенесена на произвольное многообразие.
В этом разделе мы  обобщаем определение базиса и определяем систему
отсчёта на многообразии.
В случае пространства событий общей теории относительности это ведёт нас к
\ePrints{4827-2437}
\ifx\Semafor\ValueOn
естественному определению
$O(3,1)$\Hyph системы отсчёта и преобразования Лоренца.\,\footnote{Смотри
определение преобразования Лоренца в разделе
\RefSection[GJSFRA.13.1.39]{Reference Frame in Event Space}.
}
\else
естественному определению системы отсчёта и преобразования Лоренца.
\fi
Мы предполагаем,
что касательное пространство к рассматриваемому многообразию
является векторным пространством $V$ конечной размерности $n$.
\else
Когда мы изучаем многообразие $V$, геометрия касательного пространства
является одним из важных факторов.
В этом разделе мы предполагаем
\begin{itemize}
\item все касательные пространства имеет одну и ту же геометрию;
\item касательное пространство
является векторным пространством $V$
конечной размерности $n$;
\item группой симметрии касательного пространства является группа Ли $G$.
\end{itemize}

Любой гомоморфизм векторного пространства отображает один базис в другой. 
Таким образом, мы можем распространить представление группы симметрии
на множество базисов.
Тем не менее, не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Базис, принадлежащий
выбранной орбите группы $G$, называется
\AddIndex{$G$\Hyph базисом}{G-basis}.
\fi

\begin{definition}
\labelDefinition{type G reference frame}
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Мы будем называть множество
\ShowEq{reference frame}
векторных полей
\ShowEq{vector field of reference frame}
\AddIndex{G\Hyph системой отсчёта}{G reference frame}
на многообразии $V$, если
для любого $x\in V$ множество
\ShowEq{reference frame at x}
является G\Hyph базисом в касательном пространстве $T_x$.
\else
Множество векторных полей
\ShowEq{e(i) 1n}
порождает
\AddIndex{G\Hyph систему отсчёта}{G reference frame}
\ShowEq{reference frame 1n}
на многообразии $V$, если
для любого $x\in V$ множество
\ShowEq{reference frame at x 1n}
является G\Hyph базисом\,\footnote{
Согласно разделу
\xRef[0412.391]{section: Basis in Vector Space}
мы можем отождествить базис $\Basis e(x)$ с элементом группы $G$.}
в касательном пространстве $T_x$.\,\footnote{
Существование на многообразии $G$\Hyph системы отсчёта
требует доказательства в каждом случае.}
Мы будем пользоваться обозначением
\ShowEq{show vector field of reference frame}
для векторных полей, порождающих
$G$\Hyph систему отсчёта $\Basis e$.
\fi
\qed
\end{definition}

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Векторное поле $a$ имеет разложение
\ShowEq{Vector field expansion, reference frame}
относительно системы отсчёта $\Basis e$.

Если мы не ограничим определение системы отсчёта группой симметрии,
то в каждой точке многообразия
мы можем выбрать систему отсчёта
\ShowEq{coordinate reference frame},
определённую векторными полями, касательными к линиям $x^i=const$.
Это поле базисов мы будем называть
\AddIndex{координатной системой отсчёта}{coordinate reference frame}.
Векторное поле $a$ имеет разложение
\ShowEq{Vector field expansion, coordinate reference frame}
относительно координатной системы отсчёта.
Тогда стандартные координаты системы отсчёта $\Basis e$ имеют вид
\ShowEq{standard coordinates of reference frame}
\ShowEq{reference frame expansion relative coordinate reference frame}
Так как векторы $e_{(i)}$ линейно независимы в каждой точке, матрица
$\|e^k_{(i)}\|$ имеет обратную матрицу $\|e_k^{(i)}\|$
\ShowEq{coordinate reference frame expansion relative reference frame}
\else
Мы также пользуемся записью
\ShowEq{reference frame, extensive definition}
для представления системы отсчёта на многообразии,
где мы задаём множество векторных полей
$e_{(k)}$ и двойственных им форм
\ShowEq{dual forms, reference frame}
таких, что в каждой точке
\ShowEq{dual forms and vector fields}
Равенство
\EqRef{dual forms and vector fields}
определяет формы $e^{(k)}$ однозначно.

В каждой точке многообразия
мы также рассмотрим
\AddIndex{координатную систему отсчёта}{coordinate reference frame}
\ShowEq{coordinate reference frame},
определённую векторными полями, касательными к линиям $x^i=const$.
Мы также пользуемся представлением
координатной системы отсчёта на многообразии в виде
\ShowEq{coordinate reference frame, extensive definition}
где мы задаём множество векторных полей
$\partial_i$ и двойственных им форм $dx^i$
таких, что в каждой точке
\ShowEq{dual forms and coordinate vector fields}
Эти системы отсчёта связаны отношением
\ShowEq{holonomic and anholonomic}
Из равенств
\EqRef{holonomic and anholonomic vector field},
\EqRef{holonomic and anholonomic forms},
\EqRef{dual forms and vector fields} следует
\ShowEq{frame and coframe}

\begin{theorem}
Системы отсчёта $\Basis e$ и $\Basis{\partial}$
связаны преобразованием
\ShowEq{transformation between reference frames}
где
\ShowEq{transformation between reference frames 4}
\end{theorem}
\begin{proof}
Векторное поле $a$ имеет разложение
относительно рассматриваемых систем отсчёта
\ShowEq{Vector field expansion relative reference frame}
где
\ShowEq{vector holonomic coordinates}
- \AddIndex{голономные координаты}{vector holonomic coordinates}
относительно координатной системы отсчёта $\Basis{\partial}$ и
\ShowEq{vector anholonomic coordinates}
- \AddIndex{неголономные координаты}{vector anholonomic coordinates}
относительно системы отсчёта $\Basis e$.

Мы получаем равенство
\EqRef{transformation between reference frames 1},
если рассматриваем координаты векторного поля $e_{(i)}$
относительно системы отсчёта $\Basis{\partial}$
и координаты векторного поля $\partial_k$
относительно системы отсчёта $\Basis e$.
Так как векторы $e_{(i)}$ линейно независимы в каждой точке, матрица
$\|e^k_{(i)}\|$ невырождена.
Так как векторы $\partial_k$ линейно независимы в каждой точке, матрица
$\|e_k^{(i)}\|$ невырождена.
Из равенств
\EqRef{transformation between reference frames 1}
следует, что
\ShowEq{transformation between reference frames 3}
Равенство
\EqRef{transformation between reference frames 4}
следует из равенства
\EqRef{transformation between reference frames 3}.
Из равенств
\EqRef{transformation between reference frames 1},
\EqRef{Vector field expansion relative reference frame}
следует, что
\ShowEq{transformation between reference frames 5}
Равенство
\ShowEq{transformation between reference frames 6}
следует из равенства
\EqRef{transformation between reference frames 5}.
Равенство
\ShowEq{dual forms and vector fields 1}
следует из равенств
\EqRef{dual forms and vector fields},
\EqRef{Vector field expansion relative reference frame}.
Равенство
\ShowEq{dual forms and coordinate vector fields 1}
следует из равенств
\EqRef{dual forms and coordinate vector fields},
\EqRef{Vector field expansion relative reference frame}.
Равенство
\EqRef{transformation between reference frames 2}
следует из равенств
\EqRef{transformation between reference frames 6},
\EqRef{dual forms and vector fields 1},
\EqRef{dual forms and coordinate vector fields 1}.
\end{proof}
\fi

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Мы также пользуемся более широким определением для
системы отсчёта на многообразии,
представленное в виде
\ShowEq{reference frame, extensive definition},
где мы задаём множество векторное полей
$e_{(k)}$ и двойственных им форм
\ShowEq{dual forms, reference frame}
таких, что
\ShowEq{dual forms and vector fields}
в каждой точке.
Формы $e^{(k)}$ определены однозначно из
\EqRef{dual forms and vector fields}.

Подобным образом мы можем определить
координатную систему отсчёта
\ShowEq{coordinate reference frame, extensive definition}.
Эти системы отсчёта связаны отношением
\ShowEq{holonomic and anholonomic}
Из равенств
\EqRef{holonomic and anholonomic vector field},
\EqRef{holonomic and anholonomic forms},
\EqRef{dual forms and vector fields} следует
\ShowEq{frame and coframe}

В частности, мы предположим, что мы имеем $GL(n)$-систему отсчёта 
$(\partial,dx)$, порождённый $n$ дифференцируемыми векторными полями
$\partial_i$ и 1-формами $dx^i$, которые определяют поля базисов $\partial$
и кобазисов $dx$, дуальных им.

Если задана функция $\varphi$ on $V$, то мы определяем \AddIndex{пфаффову производную}{pfaffian derivative}
\[d\varphi=\partial_i\varphi dx^i\]
\fi

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
\section{Система отсчёта в пространстве событий}
\labelSection{Reference Frame in Event Space}

Начиная с этого раздела, мы будем рассматривать ортогональную систему отсчёта
\ShowEq{reference frame in Vn}
в римановом пространстве с метрическим тензором $g_{ij}$.
Согласно определению, в каждой точке риманова пространства
векторные поля ортогональной системы отсчёта удовлетворяют соотношению
\[
g_{ij}e^i_{(k)}e^j_{(l)}=g_{(k)(l)}
\]
где $g_{(k)(l)}=0$, если $(k)\ne(l)$, и $g_{(k)(k)}=1$
или $g_{(k)(k)}=-1$ в зависимости от сигнатуры метрики.

Мы можем определить
\AddIndex{систему отсчёта в пространстве событий}
{reference frame in event space}
$V$ как $O(3,1)$\Hyph систему отсчёта.
Для нумерации векторов мы пользуемся индексом
$k=0, ..., 3$. Индекс $k=0$ соответствует времени подобному векторному полю.

\begin{remark}
\labelRemark{existence of a reference frame}
Мы можем доказать существование системы отсчёта, пользуясь
процедурой ортогонализации в каждой точке пространства
времени. Из той же процедуры мы видим, что координаты базиса
непрерывно зависят от точки.

Непрерывное поле времениподобных векторов каждого базиса определяет
конгруэнцию линий, касательных этому полю.
Мы будем говорить, что каждая из этих линий является мировой линией
наблюдателя или
\AddIndex{локальной системой отсчёта}{local reference frame}.
Следовательно, система отсчёта - это множество локальных систем отсчёта.
\qed
\end{remark}

Мы определяем \AddIndex{преобразование Лоренца}{Lorentz transformation}
как преобразование системы отсчёта
$$
{x'}^i = f^i (x^0, x^1, x^2, x^3)
$$
\begin{equation}
{e'}^i_{(k)} = a^i_j b^{(l)}_{(k)} e^j_{(l)}
\label{LorentzTransformation}
\end{equation}
где
$$
a^i_j = \frac {\partial x'^i} {\partial x'^j}
$$
$$
\delta_{(i)(l)} b^{(i)}_{(j)} b^{(l)}_{(k)} = \delta_{(j)(k)}
$$
Мы будем называть преобразование $a^i_j$ голономной частью и преобразование $b^{(l)}_{(k)}$
неголономной частью.
\fi

\section{Неголономные координаты}
\labelSection{Anholonomic Coordinates}

\ePrints{4827-2437}
\ifx\Semafor\ValueOff
Пусть $E(V, G,\pi)$ - главное расслоение,
где $V$ - дифференцируемое многообразие размерности $n$ и класса
не меньше, чем $2$. Мы также положим, что $G$ - группа симметрии касательной плоскости.

Мы определим форму связности на главном расслоении 
\begin{equation}
\omega^L=\lambda^L_Nda^N+\Gamma^L_idx^i\ \ \ \omega=\lambda_Nda^N+\Gamma dx
\EqLabel{G connection form}
\end{equation}
Мы называем функции $\Gamma_i$ компонентами связности.

Если слой является группой $GL(n)$, то связность имеет вид
\ShowEq{GLn connection form}
\[\Gamma^A_i=\Gamma^a_{bi}\]

Векторное поле $a$ имеет два вида координат: \AddIndex{голономные координаты}{vector holonomic coordinates}
\ShowEq{vector holonomic coordinates}
относительно координатной системы отсчёта
и \AddIndex{неголономные координаты}{vector anholonomic coordinates}
\ShowEq{vector anholonomic coordinates}
относительно системы отсчёта. Эти два вида координат так же следуют отношению
\begin{equation}
a^i(x)=e^i_{(i)}(x)a^{(i)}(x)
\EqLabel{parallel transfer, 3}
\end{equation}
в любой точке $x$.

Мы можем изучать параллельный перенос векторных полей,
пользуясь любой формой координат.
Так как \eqref{LorentzTransformation} - линейное преобразование,
мы ожидаем, что параллельный перенос в
неголономных координатах имеет такое же представление,
как в голономных координатах.
Таким образом мы запишем
\ShowEq{parallel transfer of vector}
Необходимо установить связь между
\AddIndex{голономными координатами связности}{holonomic coordinates of connection}
\ShowEq{holonomic coordinates of connection}
и \AddIndex{неголономными координатами связности}{anholonomic coordinates of connection}
\ShowEq{anholonomic coordinates of connection}
\ShowEq{parallel transfer of vector, 1}
Предполагая \EqRef{parallel transfer, 1},
\EqRef{parallel transfer, 2} и \EqRef{parallel transfer, 3}, мы получим
\ShowEq{parallel transfer, 4}
Из \EqRef{parallel transfer, 4} следует, что 
\begin{align*}
\Gamma^{(i)}_{(k)(p)}e^{(k)}_i(x)e^{(p)}_p(x)a^i(x)dx^p
&=a^{(i)}(x)-e^{(i)}_i(x+dx)\left(a^i(x)-\Gamma^i_{kp}a^k(x)dx^p\right)\\
&=a^i(x)e^{(i)}_i(x)-e^{(i)}_i(x+dx)\left(a^i(x)-\Gamma^i_{kp}a^k(x)dx^p\right)\\
&=a^i(x)\left(e^{(i)}_i(x)-e^{(i)}_i(x+dx)\right)
+e^{(i)}_j(x)\Gamma^j_{ip}a^i(x)dx^p\\
&=e^{(i)}_j(x)\Gamma^j_{ip}a^i(x)dx^p
-a^i(x)\frac{\partial e^{(i)}_i(x)}{\partial x^p}dx^p\\
&=\left(e^{(i)}_j(x)\Gamma^j_{ip}
-\frac{\partial e^{(i)}_i(x)}{\partial x^p}\right)a^i(x)dx^p
\end{align*}
Так как $a^i(x)$ и $dx^p$ произвольны, мы имеем 
\[
\Gamma^{(i)}_{(k)(p)}e^{(k)}_i(x)e^{(p)}_p(x)
=e^{(i)}_j(x)\Gamma^j_{ip}
-\frac{\partial e^{(i)}_i(x)}{\partial x^p}
\]
\begin{equation}
\Gamma^{(i)}_{(k)(p)}
=e^i_{(k)}e^p_{(p)}e^{(i)}_j\Gamma^j_{ip}
-e^i_{(k)}e^p_{(p)}\frac{\partial e^{(i)}_i}{\partial x^p}
\EqLabel{parallel transfer, 5}
\end{equation}
Мы определим символический оператор
\begin{equation}
\frac{\partial}{\partial x^{(p)}}
=e^p_{(p)}\frac{\partial}{\partial x^p}
\EqLabel{anholonomic derivative}
\end{equation}
Из \EqRef{frame and coframe} следует
\ShowEq{parallel transfer, 6}
Равенства
\ShowEq{de(k)i=...dek(i)}
\ShowEq{dek(i)=...de(k)i}
являются следствием равенства
\EqRef{parallel transfer, 6}.
Подставим \EqRef{anholonomic derivative} и
\EqRef{de(k)i=...dek(i)} в \EqRef{parallel transfer, 5}
\begin{equation}
\Gamma^{(i)}_{(k)(p)}=
e^i_{(k)}e^p_{(p)}e^{(i)}_j\Gamma^j_{ip}
-e^{(i)}_i\frac{\partial e^i_{(k)}}{\partial x^{(p)}}
\EqLabel{Gamma1}
\end{equation}

Равенство \EqRef{Gamma1} показывает некоторое сходство между голономными и неголономными координатами.
Мы определим символ
\ShowEq{partial(k)}
для производной вдоль векторных полей $e_{(k)}$
$$\partial_{(k)}=e^i_{(k)}\partial_i$$
Тогда \EqRef{Gamma1} принимает форму
$$
\Gamma^{(k)}_{(l)(p)}=
e^i_{(l)}e^r_{(p)}e^{(k)}_j\Gamma^j_{ir}
-e^i_{(l)}\partial_{(p)} e^{(k)}_i
$$

Следовательно, когда мы переходим от голономных координат к неголономным, преобразование связности
подобно преобразованию при переходе от одной координатной системы к другой.
Это приводит нас к модели неголономных координат.

Векторные поля $e_{(k)}$ порождают кривые, определённые дифференциальными уравнениями
$$
e^j_{(l)} \frac{\partial t} {\partial x^j} = \delta^{(k)}_{(l)}
$$
или символической системой 
\begin{equation}
\frac{\partial t} {\partial x^{(l)}} = \delta^{(k)}_{(l)}
\label{DefForX}
\end{equation}
Имея в виду символическую систему \eqref{DefForX}, мы обозначим
функционал $t$ посредством
\ShowEq{x(k)}
и будем называть его
\AddIndex{неголономной координатой}{anholonomic coordinate}.
Мы будем называть обычные координаты голономными.

Отсюда мы можем найти производную и получить
\ShowEq{Derivative For X}
Необходимое и достаточное условие полной интегрируемости
системы дифференциальных уравнений \EqRef{Derivative For X} - это равенство
\ShowEq{cikl=0}
где мы вводим \AddIndex{объект неголономности}{anholonomity object}
\ShowEq{anholonomity object 0}
\ShowEq{Anholonomity Object}
\ShowEq{Anholonomity Object kl=>(k)(l)}

\begin{theorem}
Любая система отсчёта имеет $n$ векторных полей
\DrawEq{partial_(k)}1
которые имеют коммутатор
\ShowEq{commutator vector fields, reference frame}
\end{theorem}

\begin{proof}
Равенство
\ShowEq{commutator vector fields, reference frame, 1}
является следствием равенства
\eqRef{partial_(k)}1.
Так как
\ShowEq{dij-dji=0}
то равенство
\ShowEq{commutator vector fields, reference frame, 2}
является следствием равенств
\EqRef{dek(i)=...de(k)i},
\eqRef{partial_(k)}1,
\EqRef{commutator vector fields, reference frame, 1}.
Равенство
\EqRef{commutator vector fields, reference frame}
является следствием равенств
\EqRef{Anholonomity Object},
\EqRef{Anholonomity Object kl=>(k)(l)},
\EqRef{commutator vector fields, reference frame, 2}.
\end{proof}

По той же причине мы определяем форму
\ShowEq{dx(k)=}
и внешний дифференциал этой формы имеет вид
\ShowEq{anholonomity}

Следовательно, когда $c^{(i)}_{(k)(l)} \not =0$, дифференциал $dx^{(k)}$ не является точным дифференциалом
и система дифференциальных уравнений
\EqRef{Derivative For X}
вообще говоря не может быть интегрируемой.
Тем не менее, мы можем построить реальный объект, который
моделирует решение. Мы можем изучать, как функция $x^{(i)}$ изменяется
вдоль разных кривых.
Мы будем называть такие координаты
\AddIndex{неголономными координатами на многообразии}
{anholonomic coordinates on manifold}.

\begin{remark}
\labelRemark{anholonomic coordinates, model}
Функция $x^{(i)}$ является натуральным параметром вдоль кривой потока
векторных полей $\Vector e_{(i)}$.
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Координата времени вдоль локальной системы отсчёта
является собственным временем наблюдателя.
Так как система отсчёта состоит из локальных систем отсчёта,
мы ожидаем, что их собственные времена
синхронизированы.

Мы определяем \AddIndex{синхронизацию системы отсчёта}{synchronization of reference frame}
как неголономную координату времени.

Так как синхронизация - это неголономная координата, это порождает
новые физические явления,
которые мы должны иметь в виду, когда работаем
с сильными гравитационными полями или выполняем
точные измерения. Я опишу одно из этих явлений в разделах
\RefSection{Anholonomic Coordinates in Central Body Gravitational Field} -
\RefSection{Doppler Shift in Friedman Space}.
\else
Пример такой функции мы рассмотрим в разделе
\RefSection{Synchronization of Reference Frame}.
Собственное время определено вдоль мировой линии локальной системы
отсчёта. Как мы видели в замечании
\ref{remark: existence of a reference frame}
всё пространство пронизано мировыми линиями локальных систем.
Чтобы собственное время локальных систем могло быть
временем системы отсчёта,
мы ожидаем, что собственное время непрерывно изменяется
от точки к точке.
\fi
Для синхронизации часов локальных систем отсчёта
мы пользуемся классической процедурой обмена световыми сигналами.

На первый взгляд возникает ощущение, что нельзя синхронизировать часы,
чего мы не наблюдаем на практике.
Мы допускаем, что синхронизация возможна до тех пор,
пока мы определяем время вдоль незамкнутых кривых.
Синхронизация нарушается, когда мы пытаемся синхронизировать часы
вдоль замкнутой кривой.
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff

С точки зрения математики
– это проблема интегрирования дифференциальной формы.
\fi
А именно, изменение функции вдоль петли имеет вид
\begin{equation}
\begin{split}
\Delta x^{(i)}
&= \oint dx^{(i)}\\
&=\int\int c^{(i)}_{(k)(l)}dx^{(k)}\wedge dx^{(l)}\\
&=\int\int c^{(i)}_{(k)(l)} e^{(k)}_k e^{(l)}_l dx^k\wedge dx^l
\end{split}
\EqLabel{change of coordinate along a loop}
\end{equation}

Это означает неоднозначность определения неголономной координаты.
\qed
\end{remark}

Начиная с этого места, мы не будем делать различия между голономными и неголономными координатами.
Мы так же будем обозначать $b^{(l)}_{(k)}$ как ${a^{-1}}^{(l)}_{(k)}$ в преобразовании Лоренца
\eqref{LorentzTransformation}.

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
Хотя форма $dx^{(k)}$ не является точным дифференциалом, нетрудно убедиться,
что форма $d^2x^{(k)}$ является внешним дифференциалом формы $dx^{(k)}$.
Следовательно,
\begin{equation}
\EqLabel{exterior derivative 3}
d^3x^{(k)}=0
\end{equation}

Мы можем представить внешний дифференциал формы, записанной в неголономных
координатах, в виде
\begin{align*}
&d(a_{(i_1)...(i_n)}dx^{(i_1)}\wedge ...\wedge dx^{(i_n)})\\
=&a_{(i_1)...(i_n),p}dx^p\wedge dx^{(i_1)}\wedge ...\wedge dx^{(i_n)}\\
-&a_{(i_1)...(i_n)}ddx^{(i_1)}\wedge ...\wedge dx^{(i_n)}-...
-(-1)^{n-1}a_{(i_1)...(i_n)}dx^{(i_1)}\wedge ...\wedge ddx^{(i_n)}\\
=&a_{(i_1)...(i_n),(p)}e_p^{(p)}e^p_{(r)}dx^{(r)}\wedge dx^{(i_1)}\wedge ...\wedge dx^{(i_n)}\\
-&a_{(i_1)...(i_n)}c^{(i_1)}_{(p)(r)}dx^{(p)}\wedge dx^{(r)}\wedge ...\wedge dx^{(i_n)}-...\\
-&(-1)^{n-1}a_{(i_1)...(i_n)}dx^{(i_1)}\wedge ...\wedge c^{(i_n)}_{(p)(r)}dx^{(p)}\wedge dx^{(r)}\\
=&(a_{(i_1)...(i_n),(p)}
-a_{(r)...(i_n)}c^{(r)}_{(p)(i_1)}-...
-a_{(i_1)...(r)} c^{(r)}_{(p)(i_n)})
dx^{(p)}\wedge dx^{(i_1)}\wedge ...\wedge dx^{(i_n)}
\end{align*}
В случае формы $d^3x^{(k)}$ мы получим равенство
\begin{equation}
\EqLabel{exterior derivative, anholonomic form}
\begin{array}{l}
d(c^{(k)}_{(i)(j)}dx^{(i)}\wedge dx^{(j)})\\
=(c^{(k)}_{(i)(j),(p)}
-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
-c^{(k)}_{(i)(r)} c^{(r)}_{(p)(j)})
dx^{(p)}\wedge dx^{(i)}\wedge dx^{(j)}  
\end{array}
\end{equation}
Из равенств \EqRef{exterior derivative 3}
и \EqRef{exterior derivative, anholonomic form}
следует
\begin{equation}
\EqLabel{exterior derivative, anholonomic form, 1}
(c^{(k)}_{(i)(j),(p)}
-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
-c^{(k)}_{(i)(r)} c^{(r)}_{(p)(j)})
dx^{(p)}\wedge dx^{(i)}\wedge dx^{(j)}=0  
\end{equation}
Нетрудно убедиться, что
\begin{equation}
\EqLabel{exterior derivative, anholonomic form, 2}
\begin{array}{l}
(-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
-c^{(k)}_{(i)(r)} c^{(r)}_{(p)(j)})
dx^{(i)}\wedge dx^{(j)}\\
=(-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
+c^{(k)}_{(r)(i)} c^{(r)}_{(p)(j)})
dx^{(i)}\wedge dx^{(j)}\\
=-2c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
dx^{(i)}\wedge dx^{(j)}
\end{array}
\end{equation}
Подставив \EqRef{exterior derivative, anholonomic form, 2}
в \EqRef{exterior derivative, anholonomic form, 1}, получим
\begin{equation}
\EqLabel{exterior derivative, anholonomic form, 3}
(c^{(k)}_{(i)(j),(p)}
-2c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)})
dx^{(p)}\wedge dx^{(i)}\wedge dx^{(j)}=  0
\end{equation}
Из \EqRef{exterior derivative, anholonomic form, 3} следует
\begin{equation}
\EqLabel{exterior derivative, anholonomic form, 4}
\begin{array}{l}
c^{(k)}_{(i)(j),(p)}+c^{(k)}_{(j)(p),(i)}+c^{(k)}_{(p)(i),(j)}\\
=2c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
+2c^{(k)}_{(r)(p)}c^{(r)}_{(i)(j)}
+2c^{(k)}_{(r)(i)}c^{(r)}_{(j)(p)}
\end{array}
\end{equation}
\fi
\else
Мы определим форму связности в пространстве событий 
\ShowEq{GLn connection form}
Параллельный перенос векторных полей не зависит от выбора координат
и равенство
\EqRef{transformation between reference frames 6}
должно быть инвариантно относительно параллельного переноса.
Из этого требования
согласно расчётам в разделе
\RefSection[GJSFRA.13.1.39]{Anholonomic Coordinates}
следует, что мы можем рассматривать форму $e^{(k)}$
как дифференциал координаты $x^{(k)}$
\ShowEq{dx(k)=}
и векторное поле $e_{(k)}$ как операцию дифференцирования
по координате $x^{(k)}$
\DrawEq{partial_(k)}{}
В этом случае мы рассматриваем матрицу преобразования,
отображающего систему отсчёта $\Basis{\partial}$
в систему отсчёта $\Basis e$ как матрицу Якоби
преобразования координат $x^i$ в координаты $x^{(k)}$
\ShowEq{Derivative For X}
Дифференциал формы $dx^{(i)}$ имеет вид
\ShowEq{d2x(i)}
где
\ShowEq{anholonomity object}
\AddIndex{объект неголономности}{anholonomity object}
\ShowEq{Anholonomity Object}
Следовательно, необходимое и достаточное условие полной интегрируемости
системы дифференциальных уравнений
\EqRef{Derivative For X} - это равенство
\ShowEq{cikl=0}
Вообще говоря, система дифференциальных уравнений
\EqRef{Derivative For X}
не является вполне интегрируемой.
Отображение
\ShowEq{x(k)}
называется
\AddIndex{неголономной координатой}{anholonomic coordinate}.
Координата $x^i$ называется голономной.

Хотя неголономные координаты нельзя построить в конечной области,
мы можем однозначно определить их вдоль незамкнутой кривой.\,\footnote{Я
описал построение неголономной системы координат в разделе
\RefSection[GJSFRA.13.1.39]{Anholonomic Coordinates}.
}
Мы также рассматриваем неголономную координату $x^{(0)}$
как синхронизацию системы отсчёта.
Начиная с этого места, мы не будем делать различия между голономными и неголономными координатами.
\fi

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOn
Мы определим форму кривизны для связности \EqRef{G connection form}
\[\Omega=d\omega+[\omega,\omega]\]
\[\Omega^D=d\omega^D+C^D_{AB}\omega^A\wedge \omega^B=R^D_{ij}dx^i\wedge dx^j\]
где мы определяем объект кривизны
\[R^D_{ij}=\partial_i\Gamma^D_j-\partial_j\Gamma^D_i+C^D_{AB}\Gamma^A_i\Gamma^B_j+\Gamma^D_k c^k_{ij}\]

Форма кривизны для связности \EqRef{GLn connection form} is
\begin{equation}
\Omega^a_c = d \omega^a_c + \omega^a_b \wedge \omega^b_c
\EqLabel{Curvature}
\end{equation}
где мы определим объект кривизны
\begin{equation}
R^D_{ij}=R^a_{bij}=\partial_i\Gamma^a_{bj}-\partial_j\Gamma^a_{bi}
+\Gamma^a_{ci}\Gamma^c_{bj}-\Gamma^a_{cj}\Gamma^c_{bi}+\Gamma^a_{bk} c^k_{ij}
\EqLabel{GLn curvature}
\end{equation}
Мы определим тензор Ричи
\[R_{bj}=R^a_{baj}=\partial_a\Gamma^a_{bj}-\partial_j\Gamma^a_{ba}
+\Gamma^a_{ca}\Gamma^c_{bj}-\Gamma^a_{cj}\Gamma^c_{ba}+\Gamma^a_{bk} c^k_{aj}\]
\fi

\ePrints{4827-2437,0803.3276}
\ifx\Semafor\ValueOn

\section{Метрико-аффинное многообразие}
\labelSection{Metric-affine Manifold}

При выводе уравнений гравитационного поля
(\citeBib{Landau}, \S 93,
\citeBib{Gravitation MTW 2}, \S 21.2),
предполагается, что метрический тензор
$g^{ij}$ и связность $\Gamma^k_{ij}$ независимы.
Однако мы предполагаем симметричность
метрического тензора и связности.
При выводе уравнений гравитационного поля
мы получаем связь
\ShowEq{g;k=0}
В квантовой механике
измерение компонент
метрического тензора и связности
содержит ошибку.
Если мы предположим, что связность не симметрична, то уравнение
\EqRef{g;k=0}
может оказаться неверным.

Так как ковариантная производная метрического тензора
может быть отлична от 0,
мы вводим \AddIndex{неметричность}{nonmetricity}
\ShowEq{nonmetricity}
Перенесём производную $g$ и кручение в левую часть.
\ShowEq{Connection1}
Меняя порядок индексов, мы запишем ещё два уравнения
\ShowEq{Connection2}
\ShowEq{Connection3}
Если мы вычтем равенство \EqRef{Connection1} из суммы равенств
\EqRef{Connection2} и \EqRef{Connection1}, то мы получим
\ShowEq{Connection4}
Окончательно мы получаем
\ShowEq{Connection5}

В случае связности \EqRef{GLn connection form}
мы определим \AddIndex{форму кручения}{torsion form}
\begin{equation}
T^a = d^2 x^a + \omega^a_b \wedge dx^b
\EqLabel{Torsion}
\end{equation}
Из \EqRef{GLn connection form} следует
\begin{equation}
\omega^a_b \wedge dx^b=(\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
\EqLabel{wedge connection}
\end{equation}
Подставляя \EqRef{wedge connection} и
\ePrints{4827-2437}
\ifx\Semafor\ValueOn
\EqRef{d2x(i)}
\else
\EqRef{anholonomity}
\fi
в \EqRef{Torsion}
мы получим
\begin{equation}
T^a=T^a_{cb}dx^c\wedge dx^b =
-c^a_{cb}dx^c\wedge dx^b + (\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
\EqLabel{Torsion 1}
\end{equation}
где мы определили \AddIndex{тензор кручения}{torsion tensor}
\begin{equation}
T^a_{cb} =
\Gamma^a_{bc}-\Gamma^a_{cb}-c^a_{cb}
\EqLabel{Torsion coordinates}
\end{equation}

Форма кривизны для связности \EqRef{GLn connection form} is
\begin{equation}
\Omega^a_c = d \omega^a_c + \omega^a_b \wedge \omega^b_c
\EqLabel{Curvature}
\end{equation}
где мы определим объект кривизны
\begin{equation}
R^a_{bij}=\partial_i\Gamma^a_{bj}-\partial_j\Gamma^a_{bi}
+\Gamma^a_{ci}\Gamma^c_{bj}-\Gamma^a_{cj}\Gamma^c_{bi}+\Gamma^a_{bk} c^k_{ij}
\EqLabel{GLn curvature}
\end{equation}
Мы определим тензор Ричи
\[R_{bj}=R^a_{baj}=\partial_a\Gamma^a_{bj}-\partial_j\Gamma^a_{ba}
+\Gamma^a_{ca}\Gamma^c_{bj}-\Gamma^a_{cj}\Gamma^c_{ba}+\Gamma^a_{bk} c^k_{aj}\]

Коммутатор вторых производных имеет вид
\begin{equation}
\EqLabel{commutator second derivative of vector}
\xi^a_{;cb}-\xi^a_{;bc}
=R^a_{d bc}\xi^d
-T^p_{bc}\xi^a_{;p}
\end{equation}

Так как производная метрического тензора не равна 0, мы не можем поднимать или опускать индекс
тензора внутри производной как мы это делаем в обычном римановом пространстве.
Теперь эта операция принимает следующий вид
\[a^i_{;k} = g^{ij} a_{j;k} + g^{ij}_{;k} a_j\]
Это равенство для метрического тензора принимает следующий вид
\[g^{ab}_{;k} = - g^{ai} g^{bj} g_{ij;k}\]

\begin{definition}
\labelDefinition{metric-affine manifold}
Мы будем называть риманово пространство с кручением
и неметричностью
\AddIndex{метрико\Hyph аффинным многообразием}{metric-affine manifold} \citeBib{Mielke}.
\qed  
\end{definition}

Если мы изучаем подмногообразие $V_n$ многообразия $V_{n+m}$, мы видим, что имерсия порождает
связность $\Gamma^\alpha_{\beta\gamma}$, которая связана со связностью в многообразии соотношением
\[
\Gamma^\alpha_{\beta\gamma} e^l_\alpha =
\Gamma^l_{mk} e^m_\beta e^k_\gamma + \frac {\partial e^l_\beta} {\partial u^\gamma}
\]
Следовательно, не существует непрерывного вложения
пространства с кручением в риманово пространство.
\fi

\ifx\texFuture\Defined
\section{Covariant exterior Derivative}

exterior derivative of form \EqRef{holonomic and anholonomic forms}
is different from 0. At first sight it looks unusual. However
form \EqRef{holonomic and anholonomic forms} is not
exact differential.

мы define covariant exterior derivative of form $t = t_a \theta^a$ as
\[
Dt = t_{a;b} \theta^b \land \theta^a
+ t_a c^a_{bc} \theta^b \land \theta^c
\]

When мы look at such equation мы ask if $d^2=0$ still is legal.

\section{Moving Basis}

мы meet another interesting situation when мы study moving of frame along
manifold. If мы introduce derivative for each vector of frame as
$$
\frac {De^i_{(k)}} {dx^l}
= e^i_{(k),l} + \Gamma^i_{pl} e^p_{(k)}
$$
then мы get transformation for moving frame
$$
\frac {De^i_{(k)}} {dx^l}
= A^{(p)}_{(k)l} e^i_{(p)}
$$
\[
A_{(p)(k)l} + A_{(k)(p)l} = - g_{(p)(k);l}
\]
In particular,
\[A_{(k)(k)l}= - \frac 1 2 g_{(k)(k);l}\]
мы observed the same type of transformation when мы analyzed Frenet transfer.

Therefore, if $g_{pk;l} = 0$, then мы get orthogonal transformation of frame.
However this is not so in case of nonzero derivative.
\fi


==> Representation.Russian.tex <==
%auto-ignore
\input{Representation.Eq}
\ifx\PrintBook\undefined

\section{Введение}

Эта статья была написана под большим влиянием книги \citeBib{Rashevsky}.
Изучение однородного пространства группы симметрий векторного пространства
ведёт нас к определению базиса этого пространства
и многообразия базисов.
Мы вводим два типа преобразований многообразия базисов:
активные и пассивные преобразования. Различие между ними состоит в том,
что активное преобразование может быть выражено как преобразование
исходного пространства.
Как показано в \citeBib{Rashevsky}, пассивное преобразование
даёт возможность определить
понятия инвариантности и геометрического объекта.

Мы имеем
две противоположные точки зрения на геометрический объект.
С одной стороны мы фиксируем координаты геометрического объекта
относительно заданного базиса и указываем закон преобразования
координат при замене базиса. В то же время мы рассматриваем
всю совокупность координат геометрического объекта
относительно различных базисов как единое целое. Это
даёт нам возможность
изучения геометрического объекта, не используя координаты.
\else
\chapter{Представление группы}
\labelChapter{Representation of Group}
\fi
\section{Представление группы}
\labelSection{Representation of Group}

\begin{definition}
\labelDefinition{nonsingular transformation} 
Мы будем называть отображение
\[
t:M\rightarrow M
\]
\AddIndex{невырожденным преобразованием}{nonsingular transformation},
если существует обратное отображение.
\qed
\end{definition}

\begin{definition}
Пусть
\ShowEq{product of transformations}
произведение преобразований $k$ и $l$.
Преобразование называется
\AddIndex{левосторонним преобразованием}{left-side transformation}
или оно действует слева
\[
u'=t u
\]
если
\ShowEq{left-side transformation}
Мы будем обозначать
\ShowEq{set of left-side nonsingular transformations}
множество левосторонних невырожденных преобразований множества $M$.
\qed
\end{definition}

\begin{definition}
Пусть
\ShowEq{product of transformations}
произведение преобразований $k$ и $l$.
Преобразование называется
\AddIndex{правосторонним преобразованием}{right-side transformation}
или оно действует справа
\[
u'= ut
\]
если
\ShowEq{right-side transformation}
Мы будем обозначать
\ShowEq{set of right-side nonsingular transformations}
множество правосторонних невырожденных преобразований множества $M$.
\qed
\end{definition}

Мы будем обозначать
\ShowEq{identical transformation}
тождественное преобразование.

\begin{definition}
\labelDefinition{left-side representation of group} 
Пусть $l(M)$ - группа
и $\delta$ - единица группы $l(M)$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\[
f:G\rightarrow l(M)
\]
\AddIndex{левосторонним представлением}
{left-side representation} группы\,\footnote{
Теория представления групп является частным случаем теории
представления универсальной алгебры
\citeBib{1908.04418}.
}
$G$ в множестве $M$, если отображение $f$ удовлетворяет условиям
\begin{equation}
f(ab)u=f(a)(f(b)u)
\EqLabel{left-side representation of group}
\end{equation}
\qed
\end{definition}

\begin{definition}
\labelDefinition{right-side representation of group} 
Пусть $r(M)$ - группа
и $\delta$ - единица группы $r(M)$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\[
f:G\rightarrow r(M)
\]
\AddIndex{правосторонним представлением}
{right-side representation} группы
$G$ в множестве $M$, если отображение $f$ удовлетворяет условиям
\begin{equation}
uf(ab)=(uf(a))f(b)
\EqLabel{right-side representation of group}
\end{equation}
\qed
\end{definition}

Любое утверждение, справедливое для левостороннего представления группы,
будет справедливо для правостороннего представления.
Поэтому мы будем пользоваться общим термином
\AddIndex{представление группы}{representation of group}
и будем пользоваться обозначениями для левостороннего
представления в тех случаях, когда это не вызывает недоразумения.

\begin{theorem}
\labelTheorem{inverse transformation}
Для любого $g\in G$
\begin{equation}
\EqLabel{inverse transformation}
f(g^{-1})=f(g)^{-1}
\end{equation}
\end{theorem}
\begin{proof}
На основании \EqRef{left-side representation of group} и
\begin{equation}
f(e)=\delta
\EqLabel{right-side identical transformation}
\end{equation}
мы можем записать
\[
u=\delta u=f(gg^{-1})u=f(g)(f(g^{-1})u)
\]
Это завершает доказательство.
\end{proof}

\begin{example}
Пусть $G$ - группа.
Групповая операция определяет два различных представления на множестве $G$:
\AddIndex{левый сдвиг}{left shift, group}, который мы определяем равенством
\ShowEq{left shift =}
\ShowEq{left shift}
и \AddIndex{правый сдвиг}{right shift, group}, который мы определяем равенством
\ShowEq{right shift =}
\ShowEq{right shift}
\qed
\end{example}

\begin{theorem}
Пусть представление
\[
u'=f(a)u
\]
является левосторонним представлением. Тогда представление
\ShowEq{right-side representation h}
является правосторонним представлением.
\end{theorem}
\begin{proof}
Утверждение следует из цепочки равенств
\ShowEq{right-side representation h 1}
\end{proof}

\begin{definition}
Пусть $f$ - левостороннее представление группы $G$ в множестве $M$.
Для любого $v\in M$ мы определим
\AddIndex{орбиту представления группы}
{orbit of representation of group} $G$ как множество
\ShowEq{orbit of left representation of group}
\ShowEq{show orbit of left representation of group}
\qed
\end{definition}

\begin{definition}
Пусть $f$ - правостороннее представление группы $G$ в множестве $M$.
Для любого $v\in M$ мы определим
\AddIndex{орбиту представления группы}
{orbit of representation of group} $G$ как множество
\ShowEq{orbit of right representation of group}
\ShowEq{show orbit of right representation of group}
\qed
\end{definition}

Так как $f(e)=\delta$, то
\ShowEq{u in orbit of v}vv.

\begin{theorem}
\labelTheorem{proper definition of orbit}
Если
\ShowEq{orbit, proposition}
то
\ShowEq{orbit u=orbit v}
\end{theorem}
\begin{proof}
Из \EqRef{orbit, proposition} следует
существование $a\in G$ такого, что
\begin{equation}
v=f(a)u
\EqLabel{orbit, 1}
\end{equation}
Если
\ShowEq{u in orbit of v}wv,
то существует $b\in G$ такой, что
\begin{equation}
w=f(b)v
\EqLabel{orbit, 2}
\end{equation}
Подставив \EqRef{orbit, 1} в \EqRef{orbit, 2},
мы получим
\begin{equation}
w=f(b)(f(a)u)
\EqLabel{orbit, 3}
\end{equation}
На основании \EqRef{left-side representation of group}
из \EqRef{orbit, 3} следует,
что
\ShowEq{u in orbit of v}wu.
Таким образом,
\DrawEq[vu]{orbit v in orbit u}{vu}

На основании \EqRef{inverse transformation}
из \EqRef{orbit, 1} следует,
что
\begin{equation}
u=f(a)^{-1}v=f(a^{-1})v
\EqLabel{orbit, 4}
\end{equation}
Равенство \EqRef{orbit, 4} означает, что
\ShowEq{u in orbit of v}uv{}
и, следовательно,
\DrawEq[uv]{orbit v in orbit u}{uv}
Утверждение
\EqRef{orbit u=orbit v}
следует из утверждений
\eqRef{orbit v in orbit u}{vu},
\eqRef{orbit v in orbit u}{uv}.
\end{proof}

\begin{theorem}
\labelTheorem{direct product of representations}
Если определены представление $f_1$ группы $G$ в множестве $M_1$
и представление $f_2$ группы $G$ в множестве $M_2$,
то мы можем определить
\AddIndex{прямое произведение представлений
$f_1$ и $f_2$ группы}
{direct product of representations of group}
\begin{align*}
f&=f_1\otimes f_2:G\rightarrow M_1\otimes M_2\\
f(g)&=(f_1(g),f_2(g))
\end{align*}
\end{theorem}
\begin{proof}
Чтобы показать, что $f$ является представлением,
достаточно показать, что $f$ удовлетворяет определению
\RefDefinition{left-side representation of group}.
\[f(e)=(f_1(e),f_2(e))=(\delta_1,\delta_2)=\delta\]
\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
\end{align*}
\end{proof}

\section{Однотранзитивное представление}

\begin{definition}
Мы будем называть
\AddIndex{ядром неэффективности представления группы}
{kernel of inefficiency of representation of group} $G$
множество \[K_f=\{g\in G:f(g)=\delta\}\]
Если $K_f=\{e\}$, мы будем называть представление группы $G$
\AddIndex{эффективным}{effective representation of group}.
\qed
\end{definition}

\begin{theorem}
Ядро неэффективности - это подгруппа группы $G$.
\end{theorem}
\begin{proof}
Допустим
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\[f(a_1a_2)u=f(a_1)(f(a_2)u)=u\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
\end{proof}

Если действие не эффективно, мы можем перейти к эффективному,
заменив группой $G_1=G|K_f$,
пользуясь факторизацией по ядру неэффективности.
Это означает, что мы можем изучать только эффективное действие.

\begin{definition}
Мы будем называть представление группы
\AddIndex{транзитивным}{transitive representation of group},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)b\]
Мы будем называть представление группы
\AddIndex{однотранзитивным}{single transitive representation of group},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in V$
существует одно и только одно $g\in G$ такое, что $a=f(g)b$
\end{theorem}

\begin{definition}
Мы будем называть пространство $V$
\AddIndex{однородным пространством}{homogeneous space} группы $G$,
если мы имеем однотранзитивное представление группы $G$ на $V$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{single transitive representation of group}
Если мы определим однотранзитивное представление $f$ группы $G$ на многообразии $A$,
то мы можем однозначно определить координаты на $A$, пользуясь координатами на группе $G$.

Если $f$ - ковариантное представление, то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $G$.
Если $f$ = контравариантное представление, то $f(a)$ эквивалентно правому сдвигу $R(a)$ на группе $G$.
\end{theorem}
\begin{proof}
Мы выберем точку $v\in A$
и определим координаты точки $w\in A$
как координаты преобразования $a$ такого, что $w=f(a) v$.
Координаты, определённые таким образом, однозначны
с точностью до выбора начальной точки $v\in A$,
так как действие эффективно.

Если $f$ - ковариантное представление, мы будем пользоваться записью
\[f(a)v=av\]
Так как запись
\[f(a)(f(b)v)=a(bv)=(ab)v=f(ab)v\]
совместима с групповой структурой, мы видим, что ковариантное представление $f$ эквивалентно левому сдвигу.

Если $f$ - контравариантное представление, мы будем пользоваться записью
\[f(a)v=va\]
Так как запись
\[f(a)(f(b)v)=(vb)a=v(ba)=f(ba)v\]
совместима с групповой структурой, мы видим, что контравариантное представление $f$ эквивалентно правому сдвигу.
\end{proof}

\begin{theorem}%
\labelTheorem{shifts on group commuting}
Левый и правый сдвиги на группе $G$ перестановочны.
\end{theorem}
\begin{proof}
Это следствие ассоциативности группы $G$
\[(L(a) R(b))c = a(cb)=(ac)b=(R(b) L(a))c\]
\end{proof}

\begin{theorem}%
\labelTheorem{two representations of group}
Если мы определили однотранзитивное представление $f$ на многообразии $A$,
то мы можем однозначно определить однотранзитивное представление $h$
такое, что диаграмма
\[
\xymatrix{
M\ar[rr]^{h(a)}\ar[d]^{f(b)} & & M\ar[d]^{f(b)}\\
M\ar[rr]_{h(a)}& &M
}
\]
коммутативна для любых $a$, $b\in G$.\,\footnote{Теорема
\RefTheorem{two representations of group}
на самом деле очень интересна. Тем не менее её
смысл становится более ясным, когда мы приложим эту теорему к многообразию базисов,
смотри раздел \RefSection{Basis in Vector Space}.}
\end{theorem}
\begin{proof}
Мы будем пользоваться групповыми координатами для точек $v\in A$.
Для простоты мы предположим, что $f$ - ковариантное представление.
Тогда согласно теореме \RefTheorem{single transitive representation of group}
мы можем записать левый сдвиг $L(a)$ вместо преобразования $f(a)$.

Пусть точки $v_0, v\in A$. Тогда мы можем найти
одно и только одно $a\in G$ такое, что
\[v=v_0 a=R(a) v_0\]
Мы предположим
\[h(a)=R(a)\]
Существует $b\in G$ такое, что
\[w_0=f(b)v_0=L(b) v_0\ \ \ \ w=f(b)v=L(b) v\]
Согласно теореме \RefTheorem{shifts on group commuting} диаграмма
\begin{equation}
\xymatrix{
v_0\ar[rr]^{h(a)=R(a)}\ar[d]^{f(b)=L(b)} & & v\ar[d]^{f(b)=L(b)}\\
w_0\ar[rr]_{h(a)=R(a)}& &w
}
\label{Diagram: two representations of group}
\end{equation}
коммутативна.

Изменяя $b$ мы получим, что $w_0$ - это произвольная точка, принадлежащая $A$.

Мы видим из диаграммы, что, если $v_0=v$, то $w_0=w$ и следовательно $h(e)=\delta$.
С другой стороны, если $v_0\neq v$, то $w_0\neq w$ потому, что представление $f$ однотранзитивно.
Следовательно представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $w_0$ мы можем найти $a$
такое, что $w=h(a)w_0$. Следовательно представление однотранзитивно.

В общем случае, представление $f$ не коммутативно и следовательно
представление $h$ отлично от представления $f$.
Таким же образом мы можем создать представление $f$, пользуясь представлением $h$.
\end{proof}

\begin{remark}
\labelRemark{one representation of group}
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если группа $G$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на многообразии $A$,
то мы можем определить два перестановочных представления на многообразии $A$.
Только левый или правый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму \eqref{Diagram: two representations of group}
и предположить $h(a)v_0=L(a)v_0=v$ вместо $h(a)v_0=R(a)v_0=v$ и
проанализировать, какое выражение $h(a)$ имеет в
точке $w_0$. Диаграмма
\[\xymatrix{
v_0\ar[rr]^{h(a)=L(a)}\ar[d]^{f(b)=L(b)} & & v\ar[d]^{f(b)=L(b)}\\
w_0\ar[rr]_{h(a)}& &w
}\]
эквивалентна диаграмме
\[\xymatrix{
v_0\ar[rr]^{h(a)=L(a)} & & v\ar[d]^{f(b)=L(b)}\\
w_0\ar[rr]_{h(a)}\ar[u]_{f^{-1}(b)=L(b^{-1})}& &w
}\]
и мы имеем $w=bv=bav_0=bab^{-1}w_0$. Следовательно
\[h(a)w_0=(bab^{-1})w_0\] Мы видим, что представление $h$
зависит от его аргумента.\qed  
%There is interesting question. Если I имею преобразование $L(a)$ in точке $b$
%what is $c$ такое, что $L(a) b = R_c b$. Мы можем find it из равенства
%$ab=bc$, so $c=b^{-1}ab$, следовательно
%\[L(a) b = R_{b^{-1}ab} b\]?????
\end{remark}

\ePrints{0803.3276}
\ifx\Semafor\ValueOff
\section{Линейное представление}

Если на множестве $M$ определена дополнительная структура,
мы предъявляем к представлению группы дополнительные требования.

Если на множестве $M$ определено понятие непрерывности,
то мы полагаем, что преобразование
\[
u'=f(a)u
\]
непрерывно по $u$
и, следовательно,
\[\left|\frac { \partial u'} {\partial u}\right|\neq 0\]

Если $M$ - группа, то большое значение имеют
представления левых и правых сдвигов.

\begin{definition}
Пусть $M$ - векторное пространство $V$ над полем $F$.
Мы будем называть представление группы $G$ в векторном пространстве $V$
\AddIndex{линейным представлением}
{linear representation of group},
если $f(a)$ - линейное отображение пространства $V$ для любого $a\in G$.
\qed
\end{definition}

\begin{remark}
\labelRemark{row and column vectors, vector space}

Допустим, преобразование $f(a)$ является линейным
однородным преобразованием.
$f_\gamma^\beta(a)$ являются элементами матрицы
преобразования. Мы обычно полагаем, что нижний индекс
перечисляет строки в матрице и верхний индекс перечисляет столбцы.

Согласно закону умножения матриц мы можем
представить координаты вектора как строку матрицы.
Мы будем называть такой вектор
\AddIndex{вектор\hyph строкой}{row vector}.
Мы можем так же рассматривать вектор, координаты которого
формируют столбец матрицы и будем называть
такой вектор \AddIndex{вектор\hyph столбцом}{column vector}.

Левостороннее линейное представление в пространстве вектор\hyph столбцов
\[
u'=f(a)u\ \ \ \ u'_\alpha=f_\alpha^\beta(a)u_\beta\ \ \ \ a\in G
\]
является ковариантным представлением
\[
u''_\gamma=f_\gamma^\beta(ba) u_\beta
=f_\gamma^\alpha(b)(f_\alpha^\beta(a) u_\beta)
=(f_\gamma^\alpha(b)f_\alpha^\beta(a)) u_\beta
\]

Левостороннее линейное представление в пространстве вектор\hyph строк
\[
u'=f(a)u\ \ \ \ u'^\alpha=f^\alpha_\beta(a)u^\beta\ \ \ \ a\in G
\]
является контравариантным представлением
\[
u''^\gamma=f^\gamma_\beta(ba) u^\beta
=f^\gamma_\alpha(b)(f^\alpha_\beta(a) u^\beta)
=(f^\alpha_\beta(a)f^\gamma_\alpha(b)) u^\beta
\]

Правостороннее линейное представление в пространстве вектор\hyph столбцов
\[
u'=uf(a)\ \ \ \ u'_\alpha=u_\beta f_\alpha^\beta(a)\ \ \ \ a\in G
\]
является контравариантным представлением
\[
u''_\gamma=u_\beta f_\gamma^\beta(ab)
=(u_\beta f_\alpha^\beta(a))f_\gamma^\alpha(b)
=u_\beta(f_\gamma^\alpha(b)f_\alpha^\beta(a)) 
\]

Правостороннее линейное представление в пространстве вектор\hyph строк
\[
u'=uf(a)\ \ \ \ u'^\alpha=u^\beta f^\alpha_\beta(a)\ \ \ \ a\in G
\]
является ковариантным представлением
\[
u''^\gamma=u^\beta f^\gamma_\beta(ab)
=(u^\beta f^\alpha_\beta(a))f^\gamma_\alpha(b)
=u^\beta(f^\alpha_\beta(a)f^\gamma_\alpha(b)) 
\]
\qed
\end{remark}

\begin{remark}
\labelRemark{covariant and contravariant representations}
При изучении линейного представления
мы явно будем пользоваться тензорной записью.
Мы можем пользоваться только верхним индексом и записью $u^\cdot{}_\alpha^.$ вместо
$u_\alpha$. Тогда мы можем записать преобразование этого объекта в виде
\[u'{}^\cdot{}_\alpha^.=f^\cdot{}_\alpha^.{}_\cdot{}^\beta_. u^\cdot{}_\beta^.\]
Таким образом мы можем спрятать различие между ковариантным и
контравариантным представлениями. Эта сходство идёт
сколь угодно далеко.
\qed
\end{remark}
\fi


==> Space.Time.Russian.tex <==
%auto-ignore
\def\texSpaceTime{}

				\chapter{Пространство и время в физике}
			\labelChapter{Space and Time in Physics}

			\section{Геометрия и физика}
			\labelSection{Geometry and Physics}
\epigraph{
Несомненно, что разум кажется нам слабым, когда
мы думаем о стоящих перед ним задачах; особенно слабым
он кажется, когда мы противопоставляем его безумству и страстям человечества,
которые, надо признать, почти полностью руководят судьбами человеческими
как в малом, так и в большом. Но
творения интелекта переживают шумную суету поколений и
на протяжении веков озаряют мир светом и теплом.}
{\citeBib{Einstein: Isaak Newton}, стр. 78}
Геометрические представления не являются творениями свободного ума,
а наоборот, представляют продукт практической деятельности человека.
По мере развития познания менялись представления о пространстве
и времени.\footref{footnote: Space and Time in Physics}

\CiteQuotation{Закон не может быть точным хотя бы потому, что понятия,
с помощью которых мы его формулируем, могут развиваться и в будущем
оказаться недостаточными. На дне любого тезиса и любого доказательства
остаются следы догмата непогрешимости.}{\citeBib{Einstein: On Science}, стр. 143}

Возникнув из конкретных потребностей практики человека,
математика развивалась по сложному и противоречивому пути познания.
С одной стороны, это наиболее абстрактная область науки.
Математик совершено свободно оперирует с абстрактными понятиями, изучает их свойства,
обобщает, создаёт новые понятия, ещё более удаляясь от реальной практики.
И тем более удивительны успехи прикладной математики.
Её успехи всегда потрясали человека, особенно в XX веке,
когда такие абстрактные разделы математики как теория групп,
функциональный анализ, дифференциальная геометрия
стали языком современной физики.
Соприкосновение математики с любой другой областью науки приводит к взаимному обогащению обеих.

\CiteQuotation{Из всех наук математика пользуется особым особым уважением, потому что
её теоремы абсолютно верны и неоспоримы, тогда как законы других наук в известной степени
спорны и всегда существует опасность их опровержения новыми открытиями. Однако исследователю,
работающему в какой-либо другой области науки, не приходится завидовать математику,
так как положения математики покоятся не на реальных объектах, а исключительно на объектах
нашего воображения.
В самом деле, нет ничего удивительного в том, что можно прийти к логически согласованным
выводам, если сначала пришли к соглашению относительно основных положений (аксиом), а
также относительно тех приёмов, при помощи
которых из этих основных положений выводятся другие теоремы. В то же время это глубокое уважение
к математике имеет и другое основание, а именно: математика является тем, что даёт точным
наукам известную меру уверенности; без математики они её не могли бы достичь.
//
В связи с этим возникает вопрос, который волновал исследователей всех времён.
Почему возникло такое превосходное соответствие математики с реальными предметами,
если сама она является произведением только человеческой мысли, 
не связанонй ни с каким опытом? Может ли человеческий разум без всякого опыта, путём только
одного размышления понять свойства реальных вещей.}
{\citeBib{Einstein: Geometry and Experience}}

Математика имеет эмпирические корни - алгебра связана с необходимостью расчётов,
геометрия порождена необходимостью измерений на поверхности земли,
логика является абстрактным выражением причино-следственной связи, анализ изучает движение.
Именно поэтому не случайно, что на определённых этапах развития познания
становится возможным описать реальный процесс с помощью математических моделей
разной степени сложности. Так шаг за шагом утверждения теоретической математики
становятся аппаратом прикладной математики, математика становится эмпирической наукой.

\CiteQuotation{Свидетельствами эмпирического происхождения геометрии остались в ее
системе только основные понятия ... и так называемые аксиомы.
Число этих логически неприводимых основных понятий и аксиом стремились свести к минимуму.
Стремление извлечь всю геометрию из смутной области эмпирического незаметно привело
к ошибочному заключению, которое можно уподобить превращению героев древности в богов.
Мало-помалу привыкли к взгляду на основные понятия как на "очевидные",
т.е. как на предметы и качества представления, присущие человеческому духу;
согласно этому взгляду, основным понятиям геометрии соответствуют предметы интуиции,
и отрицание той или иной аксиомы геометрии никоим образом не может быть осуществлено
непротиворечиво. Но тогда самая возможность приложения этих основных понятий и аксиом к
объектам действительности становится той самой задачей, из которой возникло кантовское
понимание пространства.
//
Второй мотив для отказа геометрии от ее эмпирической основы дала физика.
Согласно ставшему гораздо более утонченным взгляду физики на природу твердых тел и света,
в природе не существует таких обьектов, которые бы по своим свойствам точно соответствовали
основным понятиям эвклидовой геометрии. Твердое тело не может считаться абсолютно неизменяемым,
а луч света точно не воспроизводит ни прямую линию, ни даже вообще какой либо образ одного
измерения. По возрению современной науки геометрия, взятая в отдельности, не соответствует ...
никаким опытам; она должна быть приложена к объяснению их совместно с механикой, оптикой и т.д.
Так как, сверх того, геометрия должна предшествовать физике, поскольку законы последней не
могут быть выражены без помощи геометрии, то геометрия и должна казаться наукой, логически
предшествующей всякому опыту и всякой опытной проверке.}
{\citeBib{Einstein: Noneuclidean Geometry and Physics}, стр. 179}

\CiteQuotation{... Если теоремы математики прилагаются к отражению реального мира,
они не точны; они точны до тех пор, пока они не ссылаются на действительность.}
{\citeBib{Einstein: Geometry and Experience}}

\CiteQuotation{... С этой точки зрения вопрос о применимости или неприменимости эвклидовой
геометрии приобретает ясный смысл. Эвклидова геометрия, как и геометрия вообще, сохраняет
характер математической науки, так как вывод ее теорем из аксиом по-прежнему остается чисто
логической задачей, но в то же время она становится и физической наукой, так как ее аксиомы
содержат в себе утверждения относительно обьектов природы, справедливость которых может быть
доказана только опытом.}{\citeBib{Einstein: Noneuclidean Geometry and Physics}, стр. 181}

\CiteQuotation{Форма предмета не есть нечто внешнее по отношению к нему, она принадлежит
ему и определяется им самим. Поэтому формы существования материального мира - это общая
структура, определяемая его коренными свойствами, а не что-то такое, во что мир как бы
вложен ... Рациональная теория пространства и времени необходимо выводит свойства
последних как свойства такой общей структуры из самих свойств материи. Таков был источник
геометрии - она отражала прежде всего общее свойство отношений твердых тел, определяемых в
первую очередь возможностью их движения.}{\citeBib{Cite: 104}, p 117}

\CiteQuotation{... Математика вообще и геометрия в частности обязаны своим происхождением
необходимости узнать что-либо о поведении реально существующих предметов.
На это указывает даже само слово "геометрия", означающее "измерение земли".
Измерение же земли имеет дело с возможными расположениями тел в природе ... Из
системы понятий аксиоматической геометрии нельзя получить никаких суждений о
таких реально существующих предметах, которые мы называем практически твердыми телами.
Чтобы такого рода суждения были возможны, мы должны лишить геометрию ее формально-логического
характера, сопоставив пустой схеме понятий аксиоматической геометрии реальные обьекты
нашего опыта. Для этой цели достаточно прибавить только такое утверждение:
//
твердые тела ведут себя в смысле различных возможностей взаимного
расположения, как тела эвклидовой геометрии трех измерений; таким образом, теоремы
эвклидовой геометрии содержат в себе утверждения, определяющие поведение практически твердых тел.
//
Дополненнная таким утверждением геометрия становится, очевидно,
естественной наукой ... Ее утверждения покоятся существенным образом на выводах из опыта,
а не только на логических заключениях. Будем в дальнейшем называть дополненную таким
образом геометрию "практической геометрией" ... Вопрос о том, является ли практическая
геометрия эвклидовой или нет, приобретает совершенно ясный смысл; ответ на него может дать
только опыт. Всякие измерения длины в физике точно так же, как и геодезические или
астрономические измерения, в этом смысле составляют предмет практической геометрии,
если при этом исходить из того опытного закона, что свет распространяется по прямой линии,
и именно по прямой в смысле практической геометрии.}
{\citeBib{Einstein: Geometry and Experience}}

Приведенные рассуждения показывают, что математика не является особой областью познания,
развивающейся независимо от познавательно\Hyph преобразующей практики человека. На самом деле,
исходными посылками для математики служит практика, и в конечном итоге математика является
незаменимым аппаратом в практической деятельности человека.

			\section{Пространство-время}
			\labelSection{Spacetime}
\epigraph
{... Пространство и время - не простые формы явлений, а объективно\hyph реальные формы бытия.
В мире нет ничего, кроме движущейся материи, и движущаяся материя не может двигаться иначе,
как в пространстве и во времени... Изменчивость человеческих представлений о пространстве и
времени так же мало опровергают объективную реальность того и другого, как изменчивость научных
знаний о строении и формах движения материи не опровергают объективной реальности внешнего мира.}
{Lenin, 110, с. 181, 182}
\epigraph
{... Не вещи предполагают существование пространства и времени,
а наоборот, пространство и время предполагают наличность вещей, ибо пространство,
или протяженность, предполагает наличность чего-то, что протяженно, и время - движение:
ведь время - лишь понятие, производное от движения, - предполагает наличность чего-то,
что движется. Всё - пространственно и временно.}
{Феербах, 111, с. 50}

Прежде чем перейти к изучению взаимодействия геометрии и ОТО,
необходимо дать чёткое определение основных понятий. Основное понятие геометрии -
это пространство; пространство, наполненое физическим содержанием, называют пространством событий.

\CiteQuotation{... Прежде понятий, относящихся к пространству, должно существовать понятие
"материальный объект". Это логически первичное понятие. В этом легко убедиться,
анализируя пространственные понятия, например, "рядом", "касание" и т. д.,
другими словами, отыскивая их эквиваленты в опыте.}{109, с. 235}

\CiteQuotation{Физическое понятие времени отвечает понятию, присущему интуитивному мышлению.
Но такое понятие восходит к порядку вовремени ощущений индивидуума, и этот порядок мы должны
принимать как нечто первично данное. Некто ощущает ... чувственное ощущение в данный момент,
соединенное с воспоминанием о (прежних) чувственных ощущениях. Это и есть причина того,
что чувственные ощущения, по-видимому, образуют временные ряды ощущений, основанные на
оценках "раньше" и "позже". Эти ряды могут повторяться, и тогда они могут быть опознаны.
Они могут также повторяться неточно, с заменой некоторого числа событий други ми, причем
характер повторения для нас не утрачивается. Таким образом, мы приходим к представлению
времени в виде некоего одномерного каркаса, который можно заполнить ощущениями разными
способами. Одни и теже ряды ощущений отвечают тем же субъективным интервалам времени.
//
Переход от этого "субъективного" времени  ...  к понятию времени
донаучного мышления связывается с возникновением идеи о существовании реального мира,
независимого от субъекта. В этом смысле (объективное) событие ставится в соответствие с
субъективным ощущением. В таком же смысле "субъективное" время ощущения сопоставляется с
"временем" соответствующего "объективного" события. В противоположность ощущениям внешние
события и их порядок во времени претендует на справедливость для всех субъектов.
//
... При более подробном рассмотрении идеи объективного мира внешних
событий оказалось необходимым установить более сложную зависимость между событиями и
ощущениями. Впервые это было сделано с помощью инстинктивных правил мышления, в которых
особенно важную роль играет понятие пространства. Процесс усложнения понятий ведет в конечном
счете к естественным наукам.}{109, с. 242, 243}

\CiteQuotation{Форма предмета есть ... не что иное, как совокупность отношений его частей.
Поэтому речь должна идти о тех материальных связях элементов мира, которые в своей
совокупности и определяют пространство\Hyph время.
//
Простейший элемент мира - это то, что называется событием.
Оно представляет собой "точечное" явление вроде мгновенной вспышки точечной лампы или,
пользуясь наглядными понятиями о пространстве-времени, явление, протяжением которого в
пространстве и во времени можно пренебречь... Событие аналогично точке в геометрии... Всякое
явление, всякий процесс представляется как некоторая связная совокупность событий.
//
Отвлекаясь от всех свойств события, кроме того, что оно существует,
мы представляем его как ... "мировую точку". Пространство\Hyph время и есть множество всех
мировых точек.}{\citeBib{Cite: 104}, с. 133, 134}

Однако подобное определение неполно, оно не учитывает, что
\CiteQuote{каждое событие ... воздействует на некоторые другие события и
само подвержено воздействиям других событий. Вообще воздействие и есть движение,
связывающее одно событие с другим через ряд промежуточных событий... В понятиях
физики воздействие можно определить как передачу импульса и энергии.}{\citeBib{Cite: 104}, с. 134}

Таким образом, геометрия пространства-времени неотделима от физических процессов,
протекающих в самом пространстве-времени. 

\CiteQuotation{Пространство-время есть множество всех событий в мире, отвлеченных
от всех его свойств, кроме тех, которые определяются отношениями воздействия одних
событий на другие.
//
Пространственно-временная структура мира есть не что иное
как его причинно\Hyph следственная структура, взятая лишь в соответствующей
абстракции.}{\citeBib{Cite: 104}, с. 135}

Следующий вопрос, который необходимо рассмотреть, - это вопрос о физическом содержании
понятия координат. Чтобы понять всю важность этого вопроса, вспомним как ввёл Эйнштейн
единное время в теории относительности.
Прежде всего, каждый наблюдатель снабжён собственными часами. Но для того, чтобы время,
показываемое каждым наблюдателем, было координатой в пространстве событий, необходима
синхронизация часов. Однако процесс синхронизации основан на физических явлениях.

\CiteQuotation{Если в точке $A$ пространства помещены часы, то наблюдатель,
находящийся в $A$, может устанавлить время событий в непосредственной близости от $A$
путем наблюдения одновременных с этими событиииями показаний стрелок часов.
Если в другой точке $B$ пространства также имеются часы (мы добавим: "точно такие же часы,
как в точке $A$"), то в непосредственной близости от $B$ тоже возможна временная оценка событий
находящимся в $B$ наблюдателем. Однако невозможно без дальнейших предположений сравнивать во
времени какое-либо событие в $A$ с событием в $B$; мы определили пока только
"$A$-время" и "$B$-время",
но не общее для $A$ и $B$ "время". Последнее можно установить, вводя определение, что "время",
необходимое для прохождения света из $A$ в $B$, равно "времени", требуемому для прохождения света
из $B$ в $A$. Пусть в момент $t_A$ по "$A$-времени" луч света выходит из $A$ в $B$,
отражается в момент
$t_B$ по "$B$-времени" от $B$ к $A$ и возвращается назад в $A$ в момент $t'_A$ по "$A$-времени".
Часы в $A$ и $B$ будут идти, согласно определению, синхронно, если
\[t_B - t_A = t'_A - t_B\]
Мы сделаем допущение, что это определение синхронности можно дать непротиворечивым
образом и притом для сколь угодно многих точек и что, таким образом, справедливы
следующие утверждения:
//
1) если часы в $B$ идут синхронно с часами в $A$,
то часы в $A$ идут синхронно с часами в $B$;
//
2) если часы в $A$ идут синхронно как с часами в $B$,
так и с часами в $C$, то часы в $B$ и $C$ также идут синхронно относительно друг
друга.}{\citeBib{Einstein: Electrodynamics of Moving Bodies}, стр. 9, 10}

Аналогичные построения, основанные на измерении расстояний между наблюдателями
(что также можно выполнить с помощью световых сигналов) приводят
к понятию пространственных координат.

В ОТО проблема координат оказывается сложнее, но суть её остаётся следующей:
координаты являются концентрированным выражением взаимодействия различных
наблюдателей в пространстве событий.

			\section{Принцип ковариантности}
			\labelSection{Covariance Principle}
\epigraph
{Сущность времени и пространства есть движение, потому что оно всеобще;
понять его значит высказать его сущность в форме понятия.}
   {Гегель, "Лекции по истории философии".}
\epigraph
{Движение есть сущность времени и пространства. Два основных понятия выражают эту сущность:
(бесконечная) непрерывность и "пунктуальность" (= отрицание непрерывности, прерывность).
Движение есть единство непрепрерывности (времени и пространства. Движение  есть противоречие,
есть единство противоречий.}
   {111, с. 231, Lenin, Philosophic notebooks}
Определив содержание понятия пространства, мы можем перейти к рассмотрению принципов,
положенных в основу ОТО. Основным принципом ОТО является принцип общековариантности.
Вторым, не менее важным принципом в современной формулировке ОТО, является принцип
эквивалентности. Оба эти принципа тесно взаимосвязаны.
Опираясь на принцип Маха, Эйнштейн формулирует основные принципы.

\CiteQuotation{Пусть $K$ - галилеева координатная система, т. е. такая,
относительно которой (по крайней мере в рассматриваемой четырехмерной области)
некоторая масса, достаточно удаленная от других, движется прямолинейно и равномерно.
Пусть $K'$ - вторая координатная система, которая относительно $K$ движется равномерно
ускоренно. Тогда достаточно изолированная от других масса совершает относительно
$K'$ ускоренное движение, причем ни ускорение, ни направление этого ускорения не
зависят от химического состава и физического состояния этой массы.
//
Может ли наблюдатель, покоящийся относительно координатной системы $K'$,
отсюда заключить, что он находится в "действительно" ускоренной координатной
системе? Ответ на этот вопрос должен быть отрицательным, ибо только что указанное
поведение масс, свободно движущихся относительно $K'$, может быть столь же хорошо
объяснено следующим образом. Координатная система $K'$ не имеет ускорения, но в
рассматриваемой пространственно-временной области имеется гравитационное поле,
вызывающее ускоренное движение тел относительно
системы $K'$.}{\citeBib{Einstein: Foundations of general relativity}, стр. 456}

Однако Эйнштейн сделал в этой работе две методологические ошибки.
Изложив основные принципы ОТО, он пишет%

\CiteQuotation{Из этих соображений видно, что построение общей теории относительности
должно одновременнно привести и к теории тяготенмя, ибо гравитационное поле можно
"создать" простым изменением координатной
системы.}{\citeBib{Einstein: Foundations of general relativity}, с. 457}

Во-первых. Тесная связь основных принципов не означает их тождество.
Принцип эквивалентности оказался исторически первым и самым простым принципом,
сформулированным в общековариантной форме. В дальнейшем Эйнштейн понял,
что теорию относительности нельзя свести к теории гравитационного поля. Всю свою
оставшуюся жизнь он посвятил развитию принципа общековариантности.

Во-вторых. Как следствие отождествления системы отсчёта и системы координат,
Эйнштейн ошибочно отождествлял преобразование Лоренца с общим координатным
преобразованием. Самая грубая ошибка состояла в том, что Эйнштейн полагал, что с
помощью преобразований Лоренца можно породить гравитационное поле в инерциальной
системе отсчёта, если его там не было. Но это противоречит принципу общековариантности.
На самом деле здесь имеет место переход к неинерциальной системе отсчёта, выраженный
в появлении неголономности координат, используемых наблюдателем.

\CiteQuotation{... Нельзя любое поле тяжести заменить состоянием движения системы
без гравитационного поля, точно также как нельзя преобразовать все точки произвольно
движущейся среды к покою посредством релятивистского преобразования.}{107, с. 166}

Однако изолированный наблюдатель не знает, какими координатами он пользуется.
С другой стороны, и в неинерциальной системе отсчёта, и в гравитационном поле
свободные тела движутся по траекториям, не зависящим от их массы.

\CiteQuotation{Принцип эквивалентности - это утверждение о полной тождественности
всех физических процессов и явлений в однородном поле тяготения и в соответствующей
равномерно ускоренной системе отсчета, причем в общем случае речь идет о достаточно
малых пространственно-временных областях. Из принципа эквивалентности следует равенство
инертной массы и тяжелой массы, так как в противном случае уже механические движения в
ускоренной системе отсчета и в поле тяжести протекали бы неодинаково.}{Ginzburg, 105, с. 339}

Проведенный мною недавно анализ показывает, что принцип эквивалентности
не является утверждением о равенстве двух разных типов массы.
Основа принципа эквивалентности состоит в том, что ни одно явление
не может отличить одну систему отсчёта от другой и законы физики не зависят от того,
какую систему отсчёта мы используем.
Изучение электромагнитных полей показывает, что масса менее важна в общей теории относительности,
чем мы полагали раньше. Не масса, а тензор энергии импульса порождает гравитационное поле.
Свет не имеет массы, но имеет импульс.
Эйнштейн, исправив наиболее грубые ошибки, формулировал основные принципы следующим образом:
\CiteQuote{Пусть $K$ - инерциальная система без поля тяжести, $K'$ - система
координат, равномерно ускоренная относительно $K$. Тогда поведение материальных точек по
отношению к системе $K'$ будет таким же, как если бы $K'$ была инерциальной системой,
в которой существует однородное поле тяготения. Таким образом, в свете известных
из опыта свойств поля тяжести определение инерциальной системы оказывается несостоятельным.
Напрашивается мысль о том, что каждая, любым образом движущаяся система отсчета, с точки
зрения формулировки законов природы, равноценна любой другой и что, следовательно, для
областей конечной протяженности вообще не существует физически выделенных (привилегированых)
состояний движения (общий принцип относительности). Последовательное проведение этой идеи
требует еще более глубокого видоизменения геометрико-кинематических основ теории, чем
специальная теория относительности... Обобщая, приходим к следующему результату: поле
тяготения и метрика представляют собой лишь различные формы проявления одного и того же
физического поля.}{\citeBib{Einstein: Main problems of general relativity}, стр. 124}

Современная формулировка принципа общековариантности не зависит от принципа эквивалентности.
Суть состоит в том, что преобразования Лоренца образуют чётко определённую группу,
а физические величины являются инвариантными конструкциями относительно этой группы.

Необходимо отметить, что различные ошибочные толкования утверждений ОТО, высказываний Эйнштейна
(особенно ранних) обедняют содержание ОТО.
Так, отождествляя оба принципа, Фок утверждал, что
ОТО правильнее было бы назвать теорией тяготения. Другие авторы считают, что тот или иной
принцип, подобно принципу Маха, сыграл роль повивальной бабки и сейчас не является
фундаментальным принципом теории.
Нечёткость определения преобразований Лоренца у Эйнштейна породила различные поиски.
Пытаясь систематизировать обширный материал, многие исследователи ошибочно упрощали
проблему, выделяя привилегированные системы отсчёта, что противоречит принципу общековариантности.

\CiteQuotation{Существенное достижение общей теории относительности заключается в том,
что она избавила физику от необходимости вводить "инерциальную систему". Это понятие
неудовлетворительно по той причине, что оно без какого-либо обоснования выделяет из
всех мысленно возможных систем координат некоторые системы. Затем делается
предположение, что законы физики выполняются только для таких инерциальных
систем... Таким образом, в системе физики пространство как таковое наделяется ролью,
выделяющей его из всех прочих элементов физического описания. Оно играет определяющую
роль во всех процессах, не испытывая их обратного воздействия. Хотя подобная теория
является логически возможной, но, с другой стороны, она выглядит не совсем
удовлетворительной. Ньютон вполне сознавал этот недостаток, но он столь же ясно понимал,
что иного пути для физики в то время не было. Среди физиков позднейшего времени особое
внимание на это обстоятельство обратил Эрнст Мах.}{106, с. 854, 855}

Систематизируя ошибочные представления, Гинзбург пишет 

\CiteQuotation{... Название "общая теория относительности" вполне закономерно и нет оснований
от него отказываться, не говоря уже о том, что замена этого названия представляется практически
невозможной в силу установившейся традиции.
//
К сожалению, вопросы терминологии и словоупотребления столь тесно
переплетаются с существенными проблемами, что нередко мешают обсуждению этих
проблем, ... заставляют спорить о словах... Вопрос о названии теории ... столь
явно терминологический, что не может породить расхождений по сути дела. Но этого
нельзя сказать о проблеме существования в ОТО привилегированых систем отсчета... Для
достаточно малых областей пространства-времени в ОТО, конечно, существует привилегированая
система отсчета - ... имеется в виду свободно падающая локально инерциальная система
отсчета ..., в которой нет сил тяготения и справедлива частная теория относительности.
Но такие системы ... не совпадают с инерциальными системами классической механики...
//
Для областей конечной протяженности в общем случае мы не видим никакого
аналога инерциальных систем, никаких систем, столь же "привилегированых". Но здесь
то и возникает возможность терминологических разногласий. Исследование конкретных
физических задач связано с каким-то упрощением, приближением, с идеализацией
ситуации ... Но совершенно очевиден частный характер такой привилегированности, сугубо
отличный от той привилегированности, которой наделяла инерциальные системы классическая
механика.}{105, p 343 - 345}

			\section{Пространство-время и квантовая механика}
			\labelSection{Spacetime and Quantum}
\epigraph
{Каждый человек заключён в темницу своих идей, и каждый в юности должен взорвать её, чтобы
попытаться сравнить свои идеи с реальностью. Но через несколько веков другой человек, быть
может, отвергнет его идеи. С художником в его неповторимости такого произойти не может.
Так происходит только в поисках истины, и это вовсе не печально.}
   {\citeBib{Einstein: On Science}, стр. 144}

Как уже отмечалось выше, геометрические представления тесно связаны с физическими.
Поэтому в макрофизике, где все тела имеют чётко определённую форму и движутся по чётко
определённым траекториям, геометрия (во всём многообразии представлений и теорий) описывает
жёстко и однозначно определённые конструкции. Не составляет исключения и общая теория относительности.

В частности, элементарное событие - это явление длительности, которой можно пренебречь,
в области пространства, размерами которой можно пренебречь.
Точка в пространстве, траектория движения, форма тела становятся абстракциями,
не имеющими реальных физических аналогов. В большинстве случаев длительностью или размером
пренебрегать нельзя. Исчезновение существующей в макрофизике грани между частицами и волнами
привело к размыванию чётких геометрических форм. Тем самым геометрические представления
становятся в противоречие с физическими.

Совместный анализ уравнений квантовой механики и теории относительности приводит
к парадоксальному результату: необходимо квантовать метрический тензор. Соответствующий
геометрический аппарат ещё не разработан, однако несложные построения позволяют сказать
кое-что определённое о геометрической структуре пространства общерелятивистской квантовой механики.

Для того, чтобы понять суть новых геометрических представлений рассмотрим наглядный
геометрический пример.
Предположим, что в результате решения задачи мы получили на многообразии размерности $2$
две метрические формы, описывающие сферы радиусов $R$ и $r$. Таким образом, в любой точке
многообразия наблюдатель будет одновременно находиться на обеих сферах.
Предположим, что мы находимся на северном полюсе. Тогда мы получим, что обе сферы касаются
друг друга в северном полюсе. Будем двигаться теперь на юг. Но возникает вопрос: по какой
из двух сфер мы будем двигаться? Предположим, что мы будем двигаться по большой сфере.
Тогда мы перестанем касаться малой сферы. А это противоречит постановке задачи. Следовательно,
при движении по большой сфере мы как бы увлекаем за собой малую сферу. Аналогично, двигаясь
по малой сфере, мы увлекаем за собой большую сферу.

Эта картина, безусловно, не зависит ни от размерности многообразия, ни от числа и
значения метрических форм. Мы теперь можем подвести некоторые итоги.

- Квантование метрического тензора приводит к расслоению основного многообразия
(согласно значению метрического тензора).

- Квантование метрического тензора выталкивает движущийся объект из основного многообразия
в многообразие касательных плоскостей. Этот процесс намечался ещё в ОТО: система измерительных
приборов наблюдателя находится в касательных плоскостях. При движении наблюдателя основное
многообразие движется без скольжения вдоль плоскостей, всё время касаясь их.

- Параллельный перенос вдоль заданной кривой неоднозначен и, по-видимому, операция необратимая.
Геодезическая перестаёт быть кривой в привычном понимании и распадается на множество кривых,
движение по которым происходит с той или иной вероятностью. Это приводит к неоднозначному
заданию измерительной системы, которой пользуется наблюдатель.

Далее следует terra incognita математических и физических результатов. Недалеко то время,
когда мы станем свидетелями новых революционных преобразований в геометрии, физике, философии.

\CiteQuotation{Прежде чем переходить к вопросу о завершении общей теории относительности,
я должен высказаться о занимаемой мною позиции по отношению к той физической теории,
которая мз всех физических теорий нашего времени достигла наибольших успехов. Я имею в
виду статистическую квантовую механику... Это единственная современная теория, дающая стройное
объяснение тому, что мы знаем относительно квантового характера микромеханических процессов.
Эта теория, с одной стороны, и теория относительности, с другой, обе в известном смысле
считаются верными, хотя слияние этих теорий не удалось до сих пор, несмотря на все усилия.
С этим, должно быть, и связано то, что среди современных физиков-теоретиков имеются
совершенно различные мнения о том, как будет выглядеть теоретический фундамент будущей
физики. Будет ли это теория поля?}{\citeBib{Einstein: Autobiographical Notes}, стр. 288, 289}

\CiteQuotation{Б. Теория поля еще не вполне определяется системой уравнений поля.
Надо ли признавать наличие сингулярностей? Следует ли постулировать граничные условия?
//
В. Можно лм думать, что теория поля позволит понять атомистическую и
квантовую структуру реальности?.. Я полагаю, что по этому поводу в настоящее время никому не
известно ничего достоверного, поскольлу мы не знаем, каким образом и в какой степенм
исключение сингулярностей сокращает множество решений. У нас вообще нет никакого метода
для систематического полученмя решений, свободных от сингулярностей... В настоящее время
преобладает мнение, что теорию поля сначала необходимо перевести "квантованием" в
статистическую теорию вероятностей... Я вижу в этом лишь попытку описывать линейными
методами соотношения существенно нелинейного характера.
//
Г. Можно убедительно доказать, что реальность вообще не может быть
представлена непрерывным полем. Из квантовых явленмй, по-видимому, следует, что конечная
система с конечной энергией может полностью описываться конечным набором чисел (квантовых
чисел). Это, кажется, нельзя совместить с теорией континуума и требует для описания
реальности чисто алгебраической теории. Однако сейчас никто не знает, как найти основу
для такой теории.}{106, p 872, 873}

Прежде чем мы найдём новую геометрию, мы должны изучить,
что может произойти, если мы объединим идеи общей теории относительности и
квантовой механики.


==> Stmt.Gravity.Russian.tex <==
%auto-ignore
\input{Stmt.Gravity.Eq}

\AddEq[2]{note: sum of vectors 1}
{
Сумма векторов
%TabPage
\noindent
\begin{tabular}{@{}lcr}
\ShowEq{Vector v}{#1}
&
и
&
\ShowEq{Vector w}{#2}
\end{tabular}
определена правилом треугольника
\ShowEq{Vector v+w}{#1}{#2}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
Из правила параллелограмма
следует коммутативность сложения.
\end{minipage}
&
\begin{minipage}{160pt}
\ShowEq{Vector v+w=w+v}{#1}{#2}
\end{minipage}
\end{tabular}
}

\AddEq[2]{note: sum of vectors 2}
{
Ниже мы рассмотрим модель аффинного пространства
в метрико\hyph аффинном многообразии.
\ePrints{0803.3276,0405.027}
\ifx\Semafor\ValueOff
Когда мы рассматриваем связность $\Gamma^k_{ij}$ в римановом пространстве,
мы накладываем на связность ограничение,\,\footnote{
Смотри определение аффинной связности в римановом пространстве
на странице
\citeBib{Rashevsky}\Hyph 443.
}
что тензор кручения
\ShowEq{T=G-G}
обращается в $0$ (симметрия связности)
и скалярное произведение векторов при параллельном переносе не меняется.
Если на дифференцируемом многообразии определены
метрический тензор и произвольная связность,
то это многообразие называется
\AddIndex{метрико\Hyph аффинным многообразием}{metric-affine manifold}.\,\footnote{
Смотри также определение
\RefDefinition[\RefGravity]{metric-affine manifold}.
}
В частности, связность в метрико\Hyph аффинном многообразии имеет кручение.
\fi

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
\setlength{\parindent}{5mm}
В римановом пространстве, мы пользуемся геодезическими
вместо прямых.
Поэтому вектор $#1$ мы можем представить
с помощью отрезка $AB$ геодезической $L_{#1}$
при условии, что
вектор $#1$ касается геодезической $L_{#1}$ в точке $A$
и длина отрезка $AB$ равна длине вектора $#1$.
\end{minipage}
&
\ShowEq{Vector v Riemann}{#1}
\end{tabular}

\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{210pt}
\setlength{\parindent}{5mm}
Это определение позволяет отождествить вектор $#1$
и отрезок $AB$ геодезической $L_{#1}$.
\end{minipage}
&
\end{tabular}

\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{200pt}
\setlength{\parindent}{5mm}
Для заданных векторов $#1$ и $#2$ в касательной плоскости к точке $A$,
мы будем полагать $\rho>0$ - длина вектора $#1$
и $\sigma>0$ - длина вектора $#2$.
\ePrints{323966352,0921-2370}
\ifx\Semafor\ValueOff
Пусть $V$ - единичный вектор, колинеарный вектору $#1$
\ShowEq{V rho=v}
Пусть $W$ - единичный вектор, колинеарный вектору $#2$
\ShowEq{W sigma=w}
\fi
%\ShowEq{triangle ABC}
\end{minipage}
&
\ShowEq{Vector w Riemann}{#2}
\end{tabular}
}

\AddEq{note: sum of vectors 3}
{
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{240pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_v$ через точку $A$, используя вектор $v$
как касательный вектор к $L_v$ в точке $A$.
Пусть $\tau$ - канонический параметр на $L_v$ и
\ShowEq{dx/dt=A}{\tau}V
Мы перенесём вектор $w$ вдоль геодезической $L_v$ из точки $A$
в точку $B$, определённую значением параметра $\tau=\rho$.
Мы обозначим результат $w'$.
\end{minipage}
&
\ShowEq{Vector v+w= 1 Riemann}vw
\end{tabular}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_{w'}$ через точку $B$, используя вектор $W'$
как касательный вектор к $L_{w'}$ в точке $B$.
Пусть $\varphi'$ - канонический параметр на $L_{w'}$ и 
\ShowEq{dx/dt=A}{\varphi'}{W'}
Мы определим точку $C$ на геодезической $L_{w'}$
значением параметра $\varphi'=\sigma$
\end{minipage}
&
\ShowEq{Vector v+w= Riemann}vw
\end{tabular}

Я полагаю, что длина векторов $v$ и $w$ мала.
Тогда существует единственная геодезическая $L_u$
из точки $A$ в точку $C$.
Я буду отождествлять отрезок $AC$ геодезической $L_u$
и вектор $v+w$.
}

\AddEq{note: sum of vectors 4}
{
Аналогичным образом я строю треугольник $ADE$,
чтобы определить вектор $w+v$.

\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_w$ через точку $A$, используя вектор $w$
как касательный вектор к $L_w$ в точке $A$.
Пусть $\varphi$ - канонический параметр на $L_w$ и
\ShowEq{dx/dt=A}{\varphi}W
Мы перенесём вектор $v$ вдоль геодезической $L_w$ из точки $A$
в точку $D$, определённую значением параметра $\varphi=\sigma$.
Мы обозначим результат $v'$.
\end{minipage}
&
\ShowEq{Vector w+v= 1}
\end{tabular}

%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Мы проведём геодезическую $L_{v'}$ через точку $D$, используя вектор $v'$
как касательный вектор к $L_{v'}$ в точке $D$.
Пусть $\tau'$ - канонический параметр на $L_{v'}$ и 
\ShowEq{dx/dt=A}{\tau'}{V'}
Мы определим точку $E$ на геодезической $L_{v'}$
значением параметра $\tau'=\rho$
\end{minipage}
&
\ShowEq{Vector w+v=}
\end{tabular}

Существует единственная геодезическая $L_u$
из точки $A$ в точку $E$.
Я буду отождествлять отрезок $AE$ геодезической $L_u$
и вектор $w+v$.
}

\AddEq{note: sum of vectors 5}
{
%TabPage
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
Формально линии $AB$ и $DE$ так же, как линии $AD$ и $BC$, параллельны.
Длины отрезков $AB$ и $DE$ равны так же, как длины
отрезков $AD$ и $BC$ равны. Мы называем такую фигуру
\AddIndex{параллелограммом}{parallelogram}, построенным на векторах
$v$ и $w$ с вершиной в точке $A$.
\end{minipage}
&
\ShowEq{Vector v+w=w+v Metric-affine}vw
\end{tabular}
}

\DefLemma{increase of coordinate along geodesic}
{
Пусть $L_v$ - геодезическая через точку $A$ и вектор $v$
- касательный вектор к $L_v$ в точке $A$.
Приращение координаты $x^k$ вдоль геодезической $L_v$ имеет вид
\ShowEq{increase of coordinate along geodesic}
где $\tau$ - канонический параметр и мы вычисляем производные и компоненты
$\Gamma^k_{mn}$ в начальной точке. 
}

\DefProof{increase of coordinate along geodesic}
{
Система дифференциальных уравнений геодезической $L_v$
имеет вид
\ShowEq{differential equation of geodesic}
Мы можем записать решение
системы дифференциальных уравнений
\EqRef{differential equation of geodesic}
в виде ряда Тейлора
\ShowEq{increase of coordinate along geodesic 1}
Равенство
\EqRef{increase of coordinate along geodesic}
является следствием равенства
\EqRef{increase of coordinate along geodesic 1}.
}

\DefTheorem{parallelogram is not closed old}
{
Предположим $CBADE$ - параллелограм с вершиной в точке
$A$; тогда построенная фигура не будет замкнута \citeBib{torsion}.
Величина различия координат
точек $C$ и $E$ равна поверхностному интегралу кручения
над этим параллелограммом\,\footnote{Доказательство этого утверждения я нашёл в \citeBib{Shilov}}
\ShowEq{CE = surface integral of the torsion}
}

\AddEq{theorem: parallelogram is not closed}
{
\noindent
\begin{tabular}{@{}lr}
\begin{minipage}{160pt}
\setlength{\parindent}{5mm}
\begin{theorem}
\labelTheorem{parallelogram is not closed}
Предположим $CBADE$ - параллелограм с вершиной в точке
$A$; тогда построенная фигура не будет замкнута \citeBib{torsion}.
Величина различия координат
точек $C$ и $E$ равна поверхностному интегралу кручения
над этим параллелограммом
\ShowEq{CE = surface integral of the torsion}
\end{theorem}
\end{minipage}
&
\ShowEq{Vector v+w=w+v Metric-affine}vw
\end{tabular}
}

\DefProof{parallelogram is not closed}
{
Согласно лемме
\RefLemma{increase of coordinate along geodesic},
приращение координаты $x^k$ вдоль геодезической $L_v$
имеет следующий вид\,\footnote{
Доказательство этого утверждения я нашёл в \citeBib{Shilov}}
\ShowEq{CE = surface integral of the torsion}
\ShowEq{Delta AB=}
и приращение координаты $x^k$ вдоль геодезической $L_{b'}$
имеет следующий вид
\ShowEq{Delta BC=}
Здесь
\ShowEq{W'k=Wk-...}
результат параллельного переноса вектора $w$ из $A$ в $B$ и
\ShowEq{G(B)=G(A)+...}
с точностью до малой первого порядка. Подставляя
\EqRef{W'k=Wk-...},
\EqRef{G(B)=G(A)+...}
в
\EqRef{Delta BC=},
мы получим
\ShowEq{Delta BC= 1}
Общее приращение координаты $x^K$ вдоль пути $ABC$ имеет вид
\ShowEq{Delta ABC=}
Аналогично общее приращение координаты $x^K$ вдоль пути $ADE$ имеет вид
\ShowEq{Delta ADE=}
Из
\EqRef{Delta ABC=}
и
\EqRef{Delta ADE=}
следует, что
\ShowEq{Delta ADE-ABC=}
и мы получаем интегральную сумму для выражения
\[
\Delta_{ADE}x^k-\Delta_{ABC}x^k
=\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn})dx^m \wedge dx^n
\]

\ePrints{0803.3276,FAlgebra,0405.027}
\ifx\Semafor\ValueOn
Однако недостаточно найти разность
\[\Delta_{ADE}x^k-\Delta_{ABC}x^k\]
чтобы найти разность координат точек $C$ и $E$.
Координаты могут быть неголономными и мы должны учесть, что
координаты вдоль замкнутого пути изменяются \EqRef{change of coordinate along a loop}
\[\Delta x^k=\oint_{ECBADE}dx^k=-\iint_\Sigma c^k_{mn}dx^m \wedge dx^n \]
где $c$ - объект неголономности.

Окончательно разность координат точек $C$ и $E$ имеет вид
\[\Delta_{CE}x^k=\Delta_{ADE}x^k-\Delta_{ABC}x^k+\Delta x^k=
\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn}-c^k_{mn})dx^m \wedge dx^n\]
Используя \EqRef{Torsion coordinates}, мы доказали утверждение.
\fi
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теоремы
\RefTheorem{action of ring of rational integers in Abelian group}
и определения
\RefDefinition{module over commutative ring}
следует, что абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefEq
{
\begin{definition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\qed
\end{definition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в алгебре
\ShowEq{AoxA}A{}
определено согласно правилу
\DrawEq{product in algebra AA}{}
Представление
\ShowEq{h:AoxA->L(A)}
$D$\Hyph алгебры
\ShowEq{AoxA}A{}
в модуле
\ShowEq{L(A;B)}DAA,
определённое равенством
\ShowEq{representation AA in LA}
позволяет отождествить тензор
\ShowEq{d in AxoA}
с линейным отображением
\ShowEq{product in algebra AA 2},
где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}
имеет вид
\ShowEq{a ox b c=}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{direct sum of D modules}
{
Копроизведение в категории $D$\Hyph модулей называется
\AddIndex{прямой суммой}{direct sum}.\,\footnote{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой $D$\Hyph модулей $A$ и $B$.
}

\AddEq{theorem: definition of module over commutative ring}
{
\begin{theorem}
\labelTheorem{definition of module}
Элементы $D$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закону ассоциативности}{associative law}
\DrawEq{associative law, module}2
\item 
\labelItem{distributive law, module}
\AddIndex{закону дистрибутивности}{distributive law}
\ShowEq{distributive law, module}
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, D-module}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
\end{theorem}
}

\AddEq{definition: module over algebra}
{
\begin{definition}
\labelDefinition{\SideWS module over algebra}
Эффективное \SideRu востороннее представление
\DrawEq{\SideWS A->*V}{def}
ассоциативной $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{\SideRu вым модулем}{\SideWS module} над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{\SideRu вым $A$\Hyph модулем}{\SideWS A module}
или
\AddIndex{$\SideA$\Hyph модулем}{\SideA-module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\qed
\end{definition}
}

\DefDefinition{left vector space over algebra}
{
Пусть $A$ - алгебра с делением.
Эффективное левостороннее представление
\DrawEq{left A->*V}{}
%ассоциативной $D$\Hyph алгебры $A$
абелевой группы $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{левым векторным пространством}{left vector space}
над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{левым $A$\Hyph векторным пространством}{left A vector space}
или
\AddIndex{$A*$\Hyph векторным пространством}{A*-vector space}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
}

\DefDefinition{right vector space over algebra}
{
Пусть $A$ - алгебра с делением.
Эффективное правостороннее представление
\DrawEq{right A->*V}{}
%ассоциативной $D$\Hyph алгебры $A$
абелевой группы $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{правым векторным пространством}{right vector space}
над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{правым $A$\Hyph векторным пространством}{right A vector space}
или
\AddIndex{$*A$\Hyph векторным пространством}{*A-vector space}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
}

\AddEq{theorem: module over algebra}
{
\begin{theorem}
\labelTheorem{\SideWS module over algebra}
Следующая диаграмма представлений описывает \SideRu\To $\Base$\Hyph модуль $V$
\ShowEq{diagram of representations, \SideWS module}
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
\end{theorem}
}

\DefProof{module over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\def\Temp{}
\ifx\SideNS\Temp
\RefDefinition{module over commutative ring}
и теоремы
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefDefinition{\SideWS module over algebra}
%и следствия
%\RefCorollary{Free Algebra over Ring}.
и теоремы
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{lemma}
\labelLemma{structure of D algebra is generated by product}
{\it
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
}
\end{lemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\RefDefinition{linear map from A1 to A2, commutative module},
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{representation of D module in D module determines the product}
{\it
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
}
\end{lemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лем
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\AddEq{theorem: A module -> algebra is associative}
{
\begin{theorem}
\labelTheorem{\SideWS A module -> algebra is associative}
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
\end{theorem}
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\AddEq{theorem: definition of A module}
{
\begin{theorem}
\labelTheorem{definition of \SideWS module}
Пусть $V$ является \SideRu\What $\Base$\Hyph модулем.
Для любого вектора $v\in V$,
вектор, порождённый диаграммой представлений
\EqRef{diagram of representations, \SideWS module},
имеет следующий вид
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\ShowEq{\SideWS module, a+n:V->V}
порождает\,\footnote{
Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.
}
\algebrad $\Base_{(1)}$
где сложение определено равенством
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
и произведение определено равенством
\DrawEq{(a+n)(b+m)=}{\SideWS module}
\algebraD $\Base_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\algebrab $\Base$.
\begin{table}[h]
%\caption{Active and Passive Representations}
%\label{table:Passive and Active Representations}
\begin{tabular}{|l|l|l|}
\hline
Если \algebrac $\Base$ имеет единицу, то
\ShowEq{A1=A unital extension}
Если \algebrac $\Base$ является идеалом $\CBase$, то
\ShowEq{A1=D unital extension}
В противном случае
\ShowEq{A1=A+D unital extension}
\end{tabular}
\end{table}
\item
\algebraD $\Base$ является \SideRu\What идеалом \algebrab $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
Множество преобразований
\EqRef{\SideWS module, (a+n)v=av+nv}
порождает \SideRu\HSide представление \algebrab $\Base_{(1)}$ в абелевой группе $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
\end{theorem}
}

\AddEq{theorem: definition of A module, property}
{
\begin{theorem}
\labelTheorem{definition of \SideWS module, property}
Элементы \SideRu\From $\Base$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\ShowEq{distributive law, \SideWS module}
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{p,q in \Base 1, v,w in V}
\end{theorem}
}

\AddEq{proof: definition of A module}
{%
{\sc Доказательство теорем
\RefTheorem{definition of \SideWS module},
\RefTheorem{definition of \SideWS module, property}.}
Пусть $v\in V$.

\begin{lemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Пусть 
\ShowEq{module, d in D}
\ShowEq{module, a in A}
Отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
}
\end{lemma}

{\sc Доказательство.}
Утверждения
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{\SideWS module over algebra}.
Так как $V$ является абелевой группой, то
\ShowEq{\SideWS module, dv+av in V}
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\EqRef{\SideWS module, a+n:V->V}.
Поскольку преобразование $\DTransf(\DArg)$
и \SideRu\HSide преобразование $\ATransf(a)$
являются эндоморфизмами абелевой группы $V$,
то отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
\hfill\(\odot\)

Пусть $\Base_{(1)}$ - множество отображений
\EqRef{\SideWS module, a+n:V->V}.
Равенство
\EqRef{distributive law, \SideWS module, 1}
является следствием леммы
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\EqRef{distributive law, \SideWS module, 2}.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\EqRef{distributive law, \SideWS module, 2}.
Равенство
\ShowEq{distributive law, \CBase, \SideWS module, 2}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\ShowEq{distributive law, \Base, \SideWS module, 2}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \algebrab $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{\SideWS module}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Так как произведение в $D$\Hyph алгебре $A$ может быть неассоциативным,
то опираясь на теорему
\RefTheorem{definition of \SideWS module, property},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
\qed
}

\AddEq{definition: submodule}
{
\begin{definition}
\labelDefinition{submodule, \SideWS module}
Подпредставление $D$\Hyph \SideRu вого модуля $V$ называется
\AddIndex{подмодулем}{submodule}
\SideRu вого $D$\Hyph модуля $V$.
\qed
\end{definition}
}

\AddEq{theorem: submodule}
{
\begin{theorem}
\labelTheorem{submodule, \SideWS module}
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu вого $\Base$\Hyph модуля $V$.
Если векторы
\ShowEq{set vi}
принадлежат подмодулю $V'$ \SideRu вого $\Base$\Hyph модуля $V$,
то линейная комбинация векторов
\ShowEq{set vi}
принадлежат подмодулю $V'$.
\end{theorem}
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определений
\RefDefinition{\SideWS linear combination of vectors},
\RefDefinition{submodule, \SideWS module}.
}

\AddEq{theorem: set of vectors generated by set of vectors}
{
\begin{theorem}
\labelTheorem{set of vectors generated by set of vectors, \SideWS module}
Пусть $V$ - \SideRu\To $\Base$\Hyph модуль.
Множество векторов, порождённое множеством векторов
\ShowEq{vi V},
имеет вид\,\footnote{
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}
\ShowEq{w=sum vi, \SideWS module}
\end{theorem}
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
Согласно теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
мы должны доказать следующие утверждения:
\ShowEq{vectors generated by set of vectors}

\begin{itemize}
\item
Для произвольного
\ShowEq{vk in v}
положим
\ShowEq{ci=dik}{\Base_{(1)}}
Тогда
\ShowEq{vk=sum vi, \SideWS module}
Утверждение
\RefItem{\SideWS module, vk in Jv}
следует из
\EqRef{w=sum vi, \SideWS module},
\EqRef{vk=sum vi, \SideWS module}.
\item
Утверждение
\RefItem{\SideWS module, cvk in Jv}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{definition of \SideWS module}
и утверждения
\RefItem{\SideWS module, vk in Jv}.
\item
Так как $V$ является абелевой группой,
то утверждение
\RefItem{\SideWS module, sum cvk in Jv}
следует из утверждения
\RefItem{\SideWS module, cvk in Jv}
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
и теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.
\else
и теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{structure of Abelian group}.
\fi
\item
Пусть
\ShowEq{w12 in Jv}wv
Так как $V$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\DrawEq{w1+w2 in V}{\SideNS}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{gi12}w
такие, что
\DrawEq[w]{w12= \SideNS}{module}
где множества
\DrawEq[w]{|ci12 ne 0|}{\SideWS module}
конечны.
Так как $V$ является абелевой группой,
то из равенства
\eqRef{w12= \SideNS}{module}
следует, что
\DrawEq[w]{w1+w2= \SideNS}{module}
Равенство
\DrawEq[w]{w1+w2= 1 \SideNS}{module}
является следствием равенств
\EqRef{distributive law, \SideWS module, 2},
\eqRef{w1+w2= \SideNS}{module}.
Из равенства
\eqRef{|ci12 ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}w
конечно.
\item
Пусть
\ShowEq{w in Jv}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{(1)}$\Hyph числа $a$,
\ShowEq{aw in Xk \SideWS module}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{set au vi}w
такие, что
\ShowEq{w= \SideWS module}
где
\DrawEq{|wi ne 0|}{\SideWS module}
Из равенства
\EqRef{w= \SideWS module}
следует, что
\ShowEq{aw= \SideWS module}
Из утверждения
\eqRef{|wi ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |awi ne 0|}
конечно.
\end{itemize}
Из равенств
\eqRef{w1+w2 in V}{\SideNS},
\eqRef{w1+w2= 1 \SideNS}{module},
\EqRef{aw in Xk \SideWS module},
\EqRef{aw= \SideWS module}
следует, что
\ShowEq{Xk+1 in Jv}
}

\AddEq{definition: linear combination of vectors}
{
\begin{definition}
\labelDefinition{\SideWS linear combination of vectors}
Пусть
\ShowEq{vi V}{}
- множество векторов.
\ShowEq{\SideWS linear combination}%
Выражение
\ShowEq{A linear combination =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{vi}
Вектор
\ShowEq{w=wi vi\SideNS}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{vi}
\qed
\end{definition}
}

\AddEq{definition: generating set of module}
{
\begin{definition}
\labelDefinition{generating set of \SideWS module}
$J(v)$
называется
\AddIndex{подмодулем, порождённым множеством}
{submodule generated by set} $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $D$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
\qed
\end{definition}
}

\AddEq{remark: generating set of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\AddEq{remark: basis of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\AddEq{definition: basis of module}
{
\begin{definition}
\labelDefinition{basis of \SideWS module}
Если множество $X\subset V$ является множеством образующих
\SideRu\From $D$\Hyph модуля $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $D$\Hyph модуля $V$.
Если существует минимальное множество $X$, порождающее
\SideRu\To $D$\Hyph модуль $V$, то такое множество $X$ называется
\AddIndex{базисом}{basis} \SideRu\From $D$\Hyph модуля $V$.
\qed
\end{definition}
}

\AddEq{theorem: linearly depends on rest of vectors}
{
\begin{theorem}
\labelTheorem{linearly depends on rest of vectors, \SideWS module}
Пусть $\Base$ - \Algebra.
Если уравнение
\ShowEq{\SideWS wi vi=0}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0},
то вектор $v_{\gij}$
линейно зависит от остальных векторов $v$.
\end{theorem}
}

\AddEq{proof: linearly depends on rest of vectors}
{
\begin{proof}
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}v
и определения
\RefDefinition{\SideWS linear combination of vectors}.
\end{proof}
}

\AddEq{remark: 0=0vi}
{
Очевидно, что для любого множества векторов $v_{\gii}$,
\ShowEq{\SideWS 0=0vi}
}

\AddEq{remark: scalars and vectors as matrix}
{
Представим множество $\Base_{(1)}$\Hyph чисел
\ShowEq{set au vi}w
в виде матрицы
\ShowEq{column vector w=wi}w
Представим множество векторов
\ShowEq{set vi}
в виде матрицы
\ShowEq{row vector w=wi}vn
Тогда мы можем записать линейную комбинацию векторов
\ShowEq{w=wi vi\SideNS}
в виде
\ShowEq{w=w cr v}
}

\AddEq{definition: linearly independent vectors}
{
\begin{definition}
\labelDefinition{\SideWS linearly independent vectors}
Множество векторов\,\footnote{
Я следую определению в
\citeBib{Serge Lang}, страница 100.}
\ShowEq{set vi}
\SideRu\From $\Base$\Hyph модуля $V$
\AddIndex{линейно независимо}{linearly independent set},
если $w=0$ следует из уравнения
\ShowEq{\SideWS wi vi=0}
В противном случае, множество векторов
\ShowEq{set vi}
\AddIndex{линейно зависимо}{linearly dependent set}.
\qed
\end{definition}
}

\AddEq{theorem: basis of module}
{
\begin{theorem}
\labelTheorem{basis of \SideWS module}
Множество векторов
\ShowEq{basis for module over algebra}
является базисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e_{\gii}$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
\end{theorem}
}

\DefProof{basis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определению
\RefDefinition{\SideWS linear combination of vectors},
множество $\Basis e$ порождает \SideRu\To $\Base$\Hyph модуль $V$
(определение
\RefDefinition{generating set of \SideWS module}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRu\To $\Base$\Hyph модуль $V$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество $\Basis e$ является базисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\AddEq{theorem: division algebra, basis}
{
\begin{theorem}
\labelTheorem{division algebra, \SideWS basis}
Пусть $\Base$ - \Algebra.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы $e_{\gii}$ линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{theorem}
}

\DefProof{division algebra, basis}
{
Пусть множество векторов
\ShowEq{ei, i in I}
линейно зависимо. Тогда в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}.
Согласно теореме
\RefTheorem{linearly depends on rest of vectors, \SideWS module},
вектор $e_{\gij}$
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество векторов
\ShowEq{ei, i in I}
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{ei, i in I}
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{ei, i in I},
то множество векторов $v$,
\ShowEq{ei, i in I}
не является линейно независимым.
}

\AddEq{convention: we use separate color for index of element}
{
\begin{convention}
\labelConvention{we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
}

\AddEq{convention: unit of algebra in basis}
{
\begin{convention}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.
\qed
\end{convention}
}

\DefDefinition{linear map from D1 A1 to D2 A2, module}
{
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
$D_1$\Hyph модуля $A_1$
в $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}

\ifx\texFuture\Defined
\AddEq{linear map from D1 A1 to D2 A2, module}
{
\begin{definition}
\labelDefinition{linear map from D1 A1 to D2 A2, \SideNS module}
{\it
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
\SideRu\From $D_1$\Hyph модуля $A_1$
в \SideRu\To $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu\From $D_1$\Hyph модуля $A_1$ в \SideRu\To $D_2$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}
\qed
\end{definition}
}
\fi

\DefDefinition{linear map from A1 to A2, commutative module}
{
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
}

\DefEq
{
\begin{theorem}
\labelTheorem{set of A->B is D module}
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
\end{theorem}
}
{theorem: set of A->B is D module}
%\DefEq

\DefDefinition{coordinates of vector 2016}
{
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Матрица $\Base$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\fi
}

\AddEq{definition: coordinates of vector}
{
\begin{definition}
\labelDefinition{coordinates of vector, \SideWS module}
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base_{(1)}$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
Матрица $\Base_{(1)}$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\qed
\end{definition}
}

\AddEq{theorem: linear dependence between vectors of basis}
{
\begin{theorem}
\labelTheorem{linear dependence between vectors of basis, \SideWS module}
Пусть $\Base$ - \algebra.
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$.
Пусть
\DrawEq[w]{c*e=0, \SideWS module}{1}
линейная зависимость векторов базиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{(1)}$\Hyph число
\ShowEq{wi i in I}
не имеет обратного элемента
в \algebraa $\Base_{(1)}$.
\item
Множество $\Base'$ матриц
\ShowEq{w=wi i in I}
порождает \SideRu\To $\Base$\Hyph модуль.
\end{enumerate}
\end{theorem}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{w=wi i in I}
такая, что равенство
\eqRef{c*e=0, \SideWS module}{1}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Если мы положим, что $\Base_{(1)}$\Hyph число $c^{\gij}$
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}e
является следствием равенства
\eqRef{c*e=0, \SideWS module}{1}.
Следовательно вектор $e_{\gij}$
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является базисом.
Следовательно, наше предположение неверно,
и $\Base_{(1)}$\Hyph число $c^{\gij}$ не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[b]{c*e=0, \SideWS module}{}
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\AddEq{theorem: coordinates of vector with linear dependence}
{
\begin{theorem}
\labelTheorem{coordinates of vector with linear dependence, \SideWS module}
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет базис $\Basis e$ такой, что в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{2}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{w=wi i in I}
определяет координаты вектора $0\in V$ относительно базиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно базиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
\end{theorem}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{c*e=0, \SideWS module}{2}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно базиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{c*e=0, \SideWS module}{2},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.
}

\AddEq{definition: free module over ring}
{
\begin{definition}
\labelDefinition{free \SideWS module}
\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRu\To $\Base$\Hyph модуль}{free module},\,\footnote{
Я следую
определению в \citeBib{Serge Lang}, страница 103.}
если \SideRu\To $\Base$\Hyph модуль $V$ имеет базис
и векторы базиса линейно независимы.
\qed
\end{definition}
}

\AddEq{theorem: coordinates of vector of free module}
{
\begin{theorem}
\labelTheorem{coordinates of vector of free \SideWS module}
Координаты вектора $v\in V$ относительно базиса $\Basis e$
свободного \SideRu\From $\Base$\Hyph модуля $V$
определены однозначно.
\end{theorem}
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\RefTheorem{coordinates of vector with linear dependence, \SideWS module}
и определений
\RefDefinition{\SideWS linearly independent vectors},
\RefDefinition{free \SideWS module}.
}

\DefTheorem{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnote{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}
левого \BoxB{A}модуля
\ShowEq{L(A;B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f:A->B}fAA
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\end{enumerate}
}

\DefTheorem{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnote{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}
\ShowEq{L(A;B)}DAB.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\ShowEq{A->B}AD.
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A;B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A;B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\DefTheorem{direct sum of n D modules}
{
Прямая сумма $D$\Hyph модулей
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}
}

\DefTheorem{foa=fi ai}
{
Пусть
\ShowEq{A1n}An{}
- $D$\Hyph модули и
\ShowEq{A1o+.n}An
Представим $A$\Hyph число
\ShowEq{A1o+.n}an
как вектор столбец
\ShowEq{a=(a1.n)}an
Представим линейное отображение
\ShowEq{f:A->B}fAB
как вектор строку
\ShowEq{f=(f1.n)}
Тогда значение отображения $f$ в $A$\Hyph числе $a$
можно представить как произведение матриц
\ShowEq{foa=fi ai}
}

\DefTheorem{foa=fi a}
{
Пусть
\ShowEq{A1n}Bm{}
- $D$\Hyph модули и
\ShowEq{A1o+.n}Bm
Представим $B$\Hyph число
\ShowEq{A1o+.n}bm
как вектор столбец
\ShowEq{a=(a1.n)}bm
Тогда линейное отображение
\ShowEq{f:A->B}fAB
имеет представление как вектор столбец отображений
\ShowEq{a=(a1.n)}fm
таким образом, что если
$b=f\circ a$,
то
\DrawEq{foa=fi a}{}
}

\DefTheorem{map of direct sum of modules}
{
Пусть
\ShowEq{A1n}An,
\ShowEq{A1n}Bm{}
- $D$\Hyph модули и
\ShowEq{A1o+.n}An
\ShowEq{A1o+.n}Bm
Представим $A$\Hyph число
\ShowEq{A1o+.n}an
как вектор столбец
\ShowEq{a=(a1.n)}an
Представим $B$\Hyph число
\ShowEq{A1o+.n}bm
как вектор столбец
\ShowEq{a=(a1.n)}bm
Тогда линейное отображение $f$
имеет представление как матрица отображений
\ShowEq{matrix of maps}
таким образом, что если
$b=f\circ a$,
то
\ShowEq{b=f rco a}
Отображение
\ShowEq{fij:->}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $f^i_j$
с помощью \BoxB{B^i}чисел.
}

\DefTheorem{direct sum of D modules}
{
Пусть
\ShowEq{set Bi}A
- семейство $D$\Hyph модулей.
Тогда представление
\ShowEq{D->*o+A}
кольца $D$
в прямой сумме абелевых групп
\ShowEq{o+Ai}
является прямой суммой $D$\Hyph модулей
\ShowEq{o+Ai}
}

\AddEq{text: Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\AddEq{theorem: linear map of A module, coordinates}
{
\begin{theorem}
\labelTheorem{linear map of \SideWS A module, coordinates \Base\DF\Base\DT}
\ShowEq{Let e be basis}{\Base_\DF}iI{}{D_1}{\Base_\DF}
\ShowEq{Let e be basis}{\Base_\DT}jJ{}{D_2}{\Base_\DT}
\ShowEq{Let e be basis}{\Module_1}kK{\SideRu\Which}{\Base_\DF}{\Module_1}
\ShowEq{Let e be basis}{\Module_2}lL{\SideRu\Which}{\Base_\DT}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}{\Vector g}{\Vector f}
имеет представление
\DrawEq[g]{r2:A1->A2, \DFDT module}{1 \SideWS g}
\ShowEq{linear map in \SideWS A module}
\DrawEq{linear map in A module}{\SideNS}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
\end{theorem}
}

\DefProof{linear map of A module, coordinates}
{
Равенство
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS g}
является следствием теоремы
\RefTheorem{linear map of D1 D2 module, coordinates}.

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map in A module}{\SideNS}
является следствием теоремы
\RefTheorem{map of direct sum of modules}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}
алгебры $\AOn$
в модуле $\LAnA$,
определённое равенством
\DrawEq{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\ShowEq{product in algebra An 2}
где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\AddEq{remark: notation for linear map}
{
Если отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D_1$\Hyph алгебры $A_1$ в $D_2$\Hyph алгебру $A_2$,
то я пользуюсь обозначением
\ShowEq{f circ a =}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{theorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{theorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefEq
{
\begin{proof}
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
\end{proof}
}
{proof: conjugation transformation}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{theorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
\end{proof}
}
{proof: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A;B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{theorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{h generated by f, associative algebra}
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(D;A_1;A_2)$.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\ShowEq{f:A->B}f{A_1}{A_2}
имеет вид
\ShowEq{h generated by f, associative algebra}
\end{theorem}
}
{theorem: h generated by f, associative algebra}
%\DefEq

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A;B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{theorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{theorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A;B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map of complex field}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\ShowEq{f:A->B}fCC
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a01=}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefTheorem{linear map of complex field}
{
Линейное отображение
\ShowEq{f in LRC y=fx}
поля комплексных чисел имеет вид
\ShowEq{linear map of algebra C, structure, 1}
\ShowEq{linear map of algebra C, structure, 2}
где $C$\Hyph числа
\ShowEq{a... C}
определены равенством
\ShowEq{a01=}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{polylinear map of algebras}
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$ ($A_1=...=A_n=A$)
в $D$\Hyph алгебру
$S$.
}

\DefEq
{
\begin{theorem}
\labelTheorem{sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of linear maps, D module}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{sum of polylinear maps, module}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of polylinear maps, module}
%\DefEq

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\AddEq{definition: linear map A module}
{
\begin{definition}
\labelDefinition{linear map \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set linear maps, \SideWS A12 module}
множество линейных отображений
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{definition}
}

\AddEq{definition: homomorphism A module}
{
\begin{definition}
\labelDefinition{homomorphism \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for homomorphism}1
в диаграмму представлений
\ShowEq{A module diagram for homomorphism}2
называется
\AddIndex{гомоморфизмом}{homomorphism}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set homomorphisms, \SideWS A12 module}
множество гомоморфизмов
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{definition}
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A;B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefEq
{
\begin{definition}
\labelDefinition{linear map from A1 to A2, module}
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.
\qed
\end{definition}
}
{definition: linear map from A1 to A2, module}
%\DefEq

\AddEq{theorem: linear map of module}
{
\begin{theorem}
\labelTheorem{linear map, \Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}hf
\SideRu\From $\Base_{\DF}$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_{\DT}$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnote{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map, \Base\DF \Module\VF->\Base\DT \Module\VT, \SideWS module}
рассматривается как определение.}
\ShowEq{property linear map \MapE}
\end{theorem}
}

\DefProof{linear map, DA1->DA2, module}
{
Из определений
\RefDefinition[\RefRepresentation]{reduced morphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module}
следует, что
отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D }).
Равенство
\eqRef{f(da)=h... module}{\DFDT \SideWS module}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{polylinear map of algebras}
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{polylinear map of algebras}
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\RefDefinition{linear map from A1 to A2, commutative module},
\RefDefinition{polylinear map of modules}
и теоремы
\RefTheorem{linear map, DA1->DA2, module}.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\RefDefinition{module over commutative ring}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A;B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A;B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\AddEq{theorem: linear map of A module}
{
\begin{theorem}
\labelTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}gf
\SideRu\From $\Base_\DF$\Hyph модуля $\Module_\VF$
в \SideRu\To $\Base_\DT$\Hyph модуль $\Module_\VT$
удовлетворяет равенствам\,\footnote{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
рассматривается как определение.}
\ShowEq{property linear map \MapE}
\end{theorem}
}

\DefProof{linear map of module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map from D1 A1 to D2 A2, module}
следует, что
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
и отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
Равенство
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module}
является следствием равенства
%\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{definition}.
}

\DefProof{linear map of A module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map \SideWS A module}
следует, что
\begin{itemize}
\item
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module});
\item
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{g \DFDT \SideWS module}).
\item
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{f(a+b)=...}{f \DFDT \SideWS module}).
\end{itemize}
Равенства
\eqRef{f(da)=h...}{g \DFDT \SideWS module},
\eqRef{f(da)=h...}{f \DFDT \SideWS module}
являются следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{definition}.
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\AddEq[1]{theorem: maps of conjugation antilinear}
{
\begin{theorem}
\labelTheorem{#1 maps of conjugation antilinear}
Отображения сопряжения
\ShowEq{I... O}
\DoVerb являются антилинейными гомоморфизмами.
\end{theorem}
}

\DefProof{H maps of conjugation antilinear}
{
Произведение $H$\Hyph чисел
\ShowEq{H number Ea}a
и
\ShowEq{H number Ea}b
имеет вид
\DrawEq[ab]{H product aEx}{ab}
\ShowEq{H items maps of conjugation antilinear}
}

\DefProof{O maps of conjugation antilinear}
{
Произведение $O$\Hyph чисел
\ShowEq{O number Ea}a
и
\ShowEq{O number Ea}b
имеет вид
\DrawEq[ab]{O product aEx}{ab}
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{theorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{theorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{theorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{theorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{theorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{theorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{theorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{theorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{theorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A;B)}R{#1}{#1}{}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{theorem}
}

\AddEq [6]{Let e be basis}
{
Пусть
\ShowEq{basis e of module}{#1}{#2}{#3}
базис в #4 $#5$\Hyph модуле $#6$.
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в свободном #3 $#4$\Hyph модуле $#5$.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}1{}
\DrawEq [#1{1}]{va=ae1, \SideWS module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS module}
относительно базиса
\ShowEq{basis e}2{}
\DrawEq [#9{2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}2.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}1{}
и
\ShowEq{basis e}2.
}

\AddEq{theorem: linear map of module, coordinates}
{
\begin{theorem}
\labelTheorem{linear map of \SideWS \DFDT module, coordinates}
\ShowEq{Let e be basis}1iI{}{\Base_{\DF}}{\Module_1}
\ShowEq{Let e be basis}2jJ{}{\Base_{\DT}}{\Module_2}
Тогда линейное отображение
\ShowEq{show linear map \MapE}h{\Vector f}
имеет представление
\DrawEq[f]{r2:A1->A2, \DFDT module}{1 \SideWS f}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowEq{coordinates of the linear map}a{\Module}fhiI{D_2}{}b
\end{itemize}
\end{theorem}
}

\DefProof{linear map of module, coordinates}
{
Так кaк
\ShowEq{show linear map \MapE}h{\Vector f}
линейное отображение, то равенство
\ShowEq{\DFDT vb=h(e1)a \SideNS}
является следствием равенств
\eqRef{f(da)=h... \SideWS module}{\DFDT \SideWS module},
\eqRef{va=ae1, \SideWS module}{a \DFDT\SideWS module},
\eqRef{vb=f(va)}{a \DFDT\SideWS module}.
$\Module_2$\Hyph число
\ShowEq{f(e1) \SideNS}
имеет разложение
\DrawEq{f(e1)= \SideNS}{\DFDT}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{\DFDT vb=h(e1)a \SideNS}
и \eqRef{f(e1)= \SideNS}{\DFDT}, мы получаем
\ShowEq{\DFDT vb=a f e \SideNS}
\eqRef{r2:A1->A2, \DFDT module}{1 \SideWS f}
следует из сравнения
\eqRef{va=ae1, \SideWS module}{b \DFDT\SideWS module}
и \EqRef{\DFDT vb=a f e \SideNS} и
теоремы \RefTheorem{coordinates of vector of free \SideWS module}.
}

\DefDefinition{algebra over ring}
{
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnote{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.} в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinition{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefEq
{
\begin{definition}
\labelDefinition{center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14}
\ShowEq{center of algebra}
\qed
\end{definition}
}
{definition: center of algebra}
%\DefEq

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {B}{0}%
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления группы}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate representation}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
   {O}{0}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate representation}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Tidal.Russian.tex <==
%auto-ignore
\input{Tidal.Eq}

\section{Приливное уравнение}
\labelSection{Tidal Equation}

Положим, что
рассматриваемые тела совершают произвольное, а не геодезическое движение.

Мы предположим, что оба наблюдателя начинают своё путешествие из одной и той же
точки\,\footnote{Я следую \citeBib{Wheeler}, страница 33} и их скорость
удовлетворяет дифференциальным уравнениям
\ShowEq{Trajectory}
где $I=1,2$ - номер наблюдателя и $ds_I$ - инфинитезимальная дуга на геодезической $I$.
Наблюдатель $I$ следует геодезической связности
\EqRef{conection overline =},
когда $a_I=0$.
Мы положим так же, что $ds_1=ds_2=ds$.

\AddIndex{Отклонение траекторий}{deviation of trajectories}
\ShowEq{deviation of trajectories}
- это вектор, соединяющий наблюдателей.
Кривые бесконечно мало близки в окрестности начальной точки
\[x^i_2(s_2)=x^i_1(s_1)+\delta x^i(s_1)\]
\[v^i_2(s_2)=v^i_1(s_1)+\delta v^i(s_1)\]

Производная вектора $\delta x^i$ имеет вид
\[\frac{d\delta x^i}{ds}=\frac{d(x^i_2-x^i_1)}{ds}=v_2^i-v_1^i=\delta v^i\]
\AddIndex{Скорость отклонения}{speed of deviation}
$\delta x^i$ - это ковариантная производная
\ShowEq{speed of deviation}
\ShowEq{a speed of deviation}
Из \EqRef{a speed of deviation} следует, что
\ShowEq{deviation_extreme_5}
Наконец мы готовы оценить вторую
ковариантную производную вектора $\delta x^i$
\ShowEq{deviation_extreme_6 0}
\ShowEq{deviation_extreme_6}
\begin{theorem}
\labelTheorem{deviation_extreme}
Приливное ускорение
\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
связности \EqRef{conection overline =}
\fi
имеет вид
\ShowEq{deviation_extreme}
\end{theorem}
\begin{proof}
Траектория наблюдателя $1$ удовлетворяет уравнению
\ShowEq{deviation_extreme_1}
\ShowEq{deviation_extreme_2}
В тоже время траектория наблюдателя $2$ удовлетворяет уравнению
\ShowEq{deviation_extreme_3 1}
Мы можем переписать это уравнение с точностью до порядка $1$
\ShowEq{deviation_extreme_3 2}
Используя \EqRef{deviation_extreme_1}, мы получим
\ShowEq{deviation_extreme_3 3}
\ShowEq{deviation_extreme_3}
Мы подставим \EqRef{deviation_extreme_5}, \EqRef{deviation_extreme_2},
и \EqRef{deviation_extreme_3} в \EqRef{deviation_extreme_6}
\ShowEq{deviation_extreme_7}
\ShowEq{deviation_extreme_8}
Слагаемые, подчёркнутые символом $1$, представляют кривизну,
и слагаемые, подчёркнутые символом $2$ представляют
ковариантную производную кручения.
\EqRef{deviation_extreme} следует из \EqRef{deviation_extreme_8}.
\end{proof}

\begin{remark}
Тело $2$ может быть удалено от тела $1$. Тогда мы
можем воспользоваться процедурой (так же как в \citeBib{Anderson02}),
основанной на параллельном переносе.
С этой целью мы перенесём вектор скорости наблюдателя $2$ в начальную точку
наблюдателя $1$ и затем оценим приливное ускорение. Эта процедура работает в случае не
сильного гравитационного поля.
\qed
\end{remark}

\ePrints{GJSFRA.13.1.39}
\ifx\Semafor\ValueOff
\begin{remark}
Если в центральном поле наблюдатель $1$ имеет орбитальную скорость $V_\phi$, наблюдатель $2$ движется в
радиальном направлении, и оба наблюдателя следуют геодезической, то приливное ускорение имеет вид
\ShowEq{tidal acceleration in central field}
\qed
\end{remark}

\begin{remark}
Если наблюдатель $2$ следует геодезической в центральном поле, но наблюдатель $1$ зафиксировал свою
позицию на расстоянии $r$, то
\[a^1=\Gamma^1_{kl}v^kv^l
=\frac{r_g}{2r^2c^2}\]
Ускорение следует закону обратных квадратов, как следует из \EqRef{deviation_extreme}.
\qed
\end{remark}

\begin{remark}
У теоремы \RefTheorem{deviation_extreme} есть один особый случай. Если
наблюдатель $1$ движется вдоль экстремальной кривой, мы можем
пользоваться связностью Картана. В этом случае
$a_1^i=0$. Если наблюдатель $2$ движется вдоль геодезической, то
\begin{equation}
\EqLabel{remark deviation_extreme Nongeodesic 1}
a_2^i=-\Gamma(C)^i_{kl}v_2^kv_2^k=-\Gamma(C)^i_{kl}(v_1^kv_1^k+2v_1^l\delta v^k)
\end{equation}
Если мы подставим \EqRef{deviation_extreme_5}
в \EqRef{remark deviation_extreme Nongeodesic 1}, то мы получим
\ShowEq{remark deviation_extreme Nongeodesic 3}
В этом случае \EqRef{deviation_extreme} принимает вид
\ShowEq{remark deviation_extreme Nongeodesic 2}
В случае начальных условий
\begin{align*}
\delta x^k&=0\\\frac{D\delta x^k}{ds}&=0
\end{align*}
\EqRef{remark deviation_extreme Nongeodesic 2} является
оценкой ускорения \EqRef[0405.028]{Newton}.
\qed
\end{remark}
\fi

\section{Приливное ускорение и производная Ли}

\EqRef{deviation_extreme} напоминает выражение производной Ли
\EqRef[0405.028]{Lie derivative of connection, def}.
Чтобы увидеть это сходство, мы должны записать уравнение \EqRef{deviation_extreme}
другим способом.

По определению
\ShowEq{Lie 0}
\ShowEq{Lie 1}
Так как $\frac{\overline{D}a^k}{ds}$ - вектор, мы можем легко найти вторую производную
\ShowEq{Lie 2}
На последнем шаге мы используем \EqRef{Lie 1}, когда $a^k=v^k$.
Когда $v^p$ - касательный вектор траектории наблюдателя $1$, из
\EqRef{Trajectory} следует, что
\ShowEq{Lie 3}
и из \EqRef{Lie 2} и \EqRef{Lie 3} следует, что
\ShowEq{Lie 4}
\begin{theorem}
\labelTheorem{Lie deviation_extreme}
Скорость отклонения двух траекторий \EqRef{Trajectory} удовлетворяет уравнению
\ShowEq{Lie and deviation_extreme}
\end{theorem}
\begin{proof}
Мы подставим \EqRef{Lie 1} и \EqRef{Lie 4} в \EqRef{deviation_extreme}.
\ShowEq{Lie 6}
\ShowEq{Lie 5}
\EqRef{Lie and deviation_extreme} следует из \EqRef{Lie 5}
и \EqRef[0405.028]{Lie derivative of connection, def}.
\end{proof}

На первый взгляд можно предположить, что скорость отклонения
геодезической является вектором Киллинга второго типа. Это возможно, хотя
уравнение
\ShowEq{Lie deviation geodesic 1}
не следует из уравнения
\ShowEq{Lie deviation geodesic}
Однако уравнение \EqRef{Lie deviation geodesic} показывает тесную
связь между глубокой симметрией пространства\Hyph времени и гравитационным полем.

